Simulating Cooperative Prosocial Behavior with Multi-Agent LLMs: Evidence and Mechanisms for AI Agents to Inform Policy Decisions

Human prosocial cooperation is essential for our collective health, education, and welfare. However, designing social systems to maintain or incentivize prosocial behavior is challenging because people can act selfishly to maximize personal gain. This complex and unpredictable aspect of human behavior makes it difficult for policymakers to foresee the implications of their designs. Recently, multi-agent LLM systems have shown remarkable capabilities in simulating human-like behavior, and replicating some human lab experiments. This paper studies how well multi-agent systems can simulate prosocial human behavior, such as that seen in the public goods game (PGG), and whether multi-agent systems can exhibit ``unbounded actions'' seen outside the lab in real world scenarios. We find that multi-agent LLM systems successfully replicate human behavior from lab experiments of the public goods game with three experimental treatments - priming, transparency, and varying endowments. Beyond replicating existing experiments, we find that multi-agent LLM systems can replicate the expected human behavior when combining experimental treatments, even if no previous study combined those specific treatments. Lastly, we find that multi-agent systems can exhibit a rich set of unbounded actions that people do in the real world outside of the lab -- such as collaborating and even cheating. In sum, these studies are steps towards a future where LLMs can be used to inform policy decisions that encourage people to act in a prosocial manner.

==> 3_setup.tex <==
% 3 sections; 1. lab experiments, 2. combinations, and 3. evaluation/results

\section{Experimental Setup}

\color{red}wrote this whole section (esp eval) using the word "treatment" either need to define it or (preferably) change it\color{black}

With the goal of better understanding the ability of multi-agent LLM systems to model prosocial human behavior, we simulate three different types of experiments: (1) simulations which aim to directly capture the effect of a treatment observed in a previous lab experiment with human subjects; (2) simulations which combine treatments/effects from multiple previous lab experiments with human subjects; and (3) select "out-of-the-lab" real-world scenarios we use as case studies.

For all experiments, we use OpenAI's GPT. Specifically, we use GPT4 (model gpt-4o-mini), which has been shown to have the ability to interpret inherently human concepts such as equity and also scores  well on a variety of standardized tests, ranging from the Bar Exam to the GRE \cite{openai2023gpt4}.

\subsection{Research Questions}

We specifically address the following three research questions:

\bigskip

\begin{itemize}[itemindent=2.5em]
  \item[\underline{\textbf{RQ1}}] Can multi-agent LLM system simulations replicate behaviors observed in PGG lab experiments with human subjects?
\begin{itemize} [leftmargin=0.5in]
\item[\underline{a.}] Does priming LLM agents via game name replicate the effect of priming humans via game name?
\item[\underline{b.}] Does introducing transparency in contribution between LLM agents replicate the effect of introducing transparency in contribution between humans?
\item[\underline{c.}] Does varying the endowments of LLM agents replicate the effect of varying endowments of humans?
\end{itemize}
\end{itemize}

\bigskip
\color{blue}

\begin{itemize}[itemindent=2.5em]
  \item[\underline{\textbf{RQ1}}] \textit{Can multi-agent LLM system simulations replicate behaviors observed in PGG lab experiments with human subjects?} We answer this research question via three experiments comparing results from simulations with LLM-agents to results from lab experiments with human subjects:
  
  \begin{itemize} [leftmargin=0.5in]
    \item[\underline{1.}] Priming via Game Name
    \item[\underline{2.}] Introducing Transparency of Contributions
    \item[\underline{3.}] Varying Endowments
  \end{itemize}
\end{itemize}

\color{black}

\bigskip

\begin{itemize}[itemindent=2.5em]

  \item[\underline{\textbf{RQ2.}}] Can multi-agent LLM system simulations replicate human behavior extrapolated from combining the behaviors observed in multiple lab experiments with human subjects?
\begin{itemize}[leftmargin=0.5in]
    \item[\underline{a.}] Does priming LLM agents with sentences known to increase/decrease generosity in humans have that effect in simulations of the PGG?
\item[\underline{b.}] Does the effect of priming LLM agents via game name in multi-round PGGs fade over time, like priming has been observed to fade over time in other experiments with human subjects?
\end{itemize}
\end{itemize}

  \bigskip
\color{blue}
\begin{itemize}[itemindent=2.5em]

  \item[\underline{\textbf{RQ2.}}] \textit{Can multi-agent LLM system simulations replicate human behavior extrapolated from combining the behaviors observed in multiple lab experiments with human subjects?} We answer this research question via two experiments combining treatments and expected effects from multiple lab experiments with human subjects:
  \begin{itemize}[leftmargin=0.5in]
    \item[\underline{1.}] Using a priming methodology from other cooperation games in the PGG
    \item[\underline{2.}] Measuring the change in effect of priming over time, using results of priming over time from a different competition game
  \end{itemize}
\end{itemize}
\color{black}

\bigskip

\begin{itemize}
  \item[\underline{\textbf{RQ3.}}] What are required mechanisms for simulations to
inform policy-makers regarding real-world situations to test policies that encourage human collaboration?
\end{itemize}

\bigskip

\color{blue}

\begin{itemize}
  \item[\underline{\textbf{RQ3.}}] \textit{What are required mechanisms for simulations to
inform policy-makers regarding real-world situations to test policies that encourage human collaboration?} We answer this research question via three real-world case studies towards identifying necessary mechanisms:
\begin{itemize}[leftmargin=0.5in]
    \item[\underline{1.}] A classroom setting with varying late-assignment policies
    \item[\underline{2.}] A store parking lot where shoppers need to return shopping carts to designated areas
    \item[\underline{3.}] Graffitti?
  \end{itemize}
\end{itemize}

\color{black}

\bigskip

We expect generally positive results for the first two research questions, given other work has shown the ability of LLMs to replicate lab experiments that are both published and unpublished \cite{hewitt2024predicting}, but still verify this in the context of the PGG towards specifically understanding the abilities of multi-agent LLM systems to simulate prosocial behavior. \color{red}The third research question is more open-ended - we use case studies of two real-world scenarios towards identifying two mechanisms required for simulations to show expected outcomes, a process which can be continued to be used by policy makers. As policy makers consider the specific scenarios which they need to simulate, they may realize and implement new mechanisms required to enable their simulation.\color{black}

\subsection{Multi-Agent-LLM System}

For our experiments, we adapt a previous introduced agent architecture for simulating social emergent behavior \cite{park2023generativeagentsinteractivesimulacra}. In this architecture, the administrator provides each agent with a name, public and private biographies, instructions (called directives), and an initial plan, which consists of a description, stop condition, and a location. The architecture also allows for the creation of rooms, between which agents are able to move. 

\subsubsection{System Setup for Public Goods Game Experiments}

In PGG experiments, there is an agent named and directed to act as the moderator. The remaining agents (varies from three to four depending upon the experiment) are given arbitrary alphabetical names (Alice, Bob, Casey, and David). Each agent's initial endowment is specified in their public biography, which all other agents can see. If there is a priming condition, it is included in the private biography as to expose the desired agent to the priming without leakage to other agents. Communication is not inherently turn-taking in the architecture; so we have to specify the order and method of contribution to player agents via their directives and initial plan. We initialize two separate rooms - the Game Room and the Moderation Room. Player agents are by default in the game room, then travel to the moderation room to tell the moderator their contribution once the player specified as being before them returns to game room from the moderation room after making their contribution. The moderator remains in the moderation room other than to announce payoffs after all players have made contributions. To realize transparency, we simply remove the moderation room, and have all agents make their contributions publicly in the game room. For the experiment with multiple rounds, we use nearly the same instruction set, other than specifying to the moderator and player agents via directives to repeat the same process for multiple rounds.

The thoughts and actions of each player (and the moderator) are displayed in separate output logs, each representing one of the agents involved in the simulation. In each of the output logs, the agent waits for the condition required (the return of the player before them), then acts on the plan of moving to the moderation room and making a contribution by speaking with the moderator. The moderator stores each contribution to memory in order to later announce payoffs. We extract the contribution amount of each agent using a script on each agent's output logs, identifying the section in which the agent speaks in the moderation room and taking the monetary amount in that sentence. We also manually verified these contribution amounts to ensure accuracy.

\subsubsection{System Setup for Real-World Case Studies}

\color{red}We use two real-world settings as case studies to identify mechanisms needed to enable informative simulations. For these case studies, we run several simulations with slightly varying conditions to generally understand the ways in which agents act, and then use that to create a mechanism which enables a behavior we identify as missing from a combination of general knowledge and informative studies.

The first is a classroom setting, where we specifically focus the impact of various late policies (no penalty, full penalty, and penalty by days late) on student communicative and collaborative behaviors. We define a professor agent (named the Professor) and three student agents with arbitrary names (Alice, Bob, and Casey). The professor agent is given instructions to announce a late policy to the class, and then begin assigning assignments. In student agents public biography, they are given one of three "personalities" - an overachiever, a hard-worker, and a balanced individual. In the private biographies of the agents, we add various perturbations to student lives that would reasonably affect their ability to turn in assignments on time, such as having a midterm in another class, having special difficulty with a particular assignment, or having a busy week in general. We do not need to implement a rigid turn-taking guideline, however we do generally add a framework within which agents act - the professor agent announces assignments on a fixed frequency in the classroom, between which student agents "work" on assignments and consider how many days late they will need to submit it based on the other factors in their lives.

Second, we simulate shoppers in a parking lot who can either return or not return their shopping cart. We define five shopper agents with arbitrary names (Alice, Bob, Casey, David, and Emery). We add various perturbations to shopper lives that affect their ability to return their shopping cart \cite{scientificamerican2020shoppingcarts} in their private biographies. Shopper agents by default have blank public biographies; but if perturbations added to the shopper's private biography would reasonably be extrapolated other people in real life (such as having a child), we also include it in the shopper's public biography. Shopper agents are not given directives, but have an initial plan to decide whether or not to return their shopping cart, and then to act on it. We also try changing the environment by adding agents who are employees of the store tasked with taking the shopping carts from the parking lot back into the store. These agents are given the name "Employee," have public biographies which indicate that they are a store employee, have an initial plan (and related directives) to move carts, and otherwise have all other fields left blank.\color{black}

\subsection{Evaluation}

\subsubsection{Replicating Observed Outcomes from Past Public Goods Game Experiments}

For experiments of the first type, we run simulations of the PGG using treatments from published lab experiments with human subjects, checking whether the effect of said treatments on multi-agents LLMs in simulation in similar to that of on humans. The treatments and effects we replicate from previous lab experiments are listed in Table ~\ref{labexperiments}.

\begin{center}
\begin{table}[H]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{10pt}
\begin{tabular}{|>{\columncolor{gray!20}\centering\arraybackslash}m{0.5cm}|p{6cm}|p{6cm}|} 
 \hline
 \rowcolor{gray!20} \textbf{Exp.} & \multicolumn{1}{c|}{\textbf{Treatment}} & \multicolumn{1}{c|}{\textbf{Expected Result}} \\ [0.5ex] 
 \hline\hline
 \textbf{1} & \textbf{Priming via Game Name:} Participants are presented the PGG as a game called either the "Taxation Game" or "Teamwork Game." & Participants presented the game as the "Taxation Game" contribute less than participants presented the "Teamwork Game." \cite{Eriksson_Strimling_2014} \\ 
 \hline
 \textbf{2} & \textbf{Transparency of Contribution:} Participants know what others contribute to the public pool (under standard conditions, contributions are made privately with respect to other players). & Participants make larger contributions when participants are aware of each other's contributions compared to when contributions are made privately without other's knowledge. \cite{transparencytwo}\\
 \hline
 \textbf{3} & \textbf{Variations in Endowment:} Participants start the PGG with different endowment amounts. & "Rich" participants contribute more when other participants are also "rich." \cite{HARGREAVESHEAP20164}  \\
 \hline
\end{tabular}
\caption{\label{labexperiments}Table of treatments and expected results (effects) from previous lab experiments of the PGG with human subjects. Actual experiments that are drawn from are cited in the second column.}
\end{table}
\end{center}




For these experiments, we simulate one-shot PGGs with three or four players, measuring whether the impact the treatments have on player contributions is similar to what has been observed in experiments with human subjects (i.e., the expected result listed). For the first experiment, we run ten simulations of the PGG with four players, two under each priming condition, and compare the average contribution amount of players from either group. For the second experiment, we also run ten simulations of the PGG with four players: five simulations with transparency of contributions and five without. We compare the average contribution amount of players in either of the two conditions. In the first and second experiments, players are all endowed with \$20. For the third experiment, we run twenty simulations with three players: fifteen simulations where all players have the same initial endowment (five where that endowment is \$20, five where it is \$50, and five where it is \$80) and five simulations where players have different initial endowments (namely, \$20, \$50, and \$80). We compare the average contributions of players with each of the three endowments in the fixed and the varied endowment conditions (i.e., we compare how much a player with \$X contributes in the condition where everyone has \$X vs. the varied condition). In all three experiments, 1.6 times the amount of the public pool is split evenly amongst the players as their payoff - players are made aware of this to inform the way in which they act, but the simulations are of one-shot PGGs.

\subsubsection{Verifying Outcomes from Combinations of Past Lab Experiments}

We also design two additional experiments based on a combination of treatments and effects from multiple lab experiments with human subjects. The first takes a priming methodology and effect from experiments with human subjects of different cooperative games than the PGG to see if the effect holds for the PGG. The second uses a priming methodology used on the one-shot PGG and measures if it has the same effect over multiple rounds similar to the way in which priming affects different economic games than the PGG. The treatments and effects in the combined experiments we design are listed in Table ~\ref{combinedexperiments}.

\begin{center}
\begin{table}[H]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{10pt}
\begin{tabular}{|>{\columncolor{gray!20}\centering\arraybackslash}m{0.5cm}|p{6cm}|p{6cm}|} 
 \hline
 \rowcolor{gray!20} \textbf{Exp.} & \multicolumn{1}{c|}{\textbf{Treatment}} & \multicolumn{1}{c|}{\textbf{Expected Result}} \\ [0.5ex] 
 \hline\hline
 \textbf{1} & \textbf{Priming via Sentences:} Participants are presented with 5 sentences alluding to either "unity" or "proportionality" concepts. & Participants presented with sentences alluding to "unity" contribute more than participants primed with "proportionality". \cite{6d947858-4a17-3462-9053-fc55b58ffee1, moralsmatter} \\ 
 \hline
 \textbf{2} & \textbf{Priming via Game Name over Multiple Rounds:} Participants are presented the PGG as a game called either the "Taxation Game" or "Teamwork Game" and play for five rounds. & The effect of priming should fade over time; although there should still be a disparity between participants in either group's initial contributions, it should lessen over time. \cite{Eriksson_Strimling_2014, JIMENEZJIMENEZ201594} \\
 \hline
\end{tabular}
\caption{\label{combinedexperiments}Table of treatments and expected results (effects) from combining previous lab experiments with human subjects. Actual experiments that are drawn from are cited in the second column.}
\end{table}
\end{center}

For both experiments, all players are endowed with \$20. For the first experiment, we run ten simulations a one-shot PGG with four players, two under each priming condition ("unity" and "proportionality"), and compare the average contribution amount of players from either group. We prime each player by exposing them to five sentences alluding to each concept, taken from the lab experiment \cite{moralsmatter}. In this experiment, 1.6 times the amount of the public pool is split evenly amongst the players as their payoff - players are made aware of this to inform the way in which they act, but the simulations are of one-shot PGGs. For the second experiment, we run ten simulations of a PGG with five rounds and four players, two under each priming condition ("Taxation" and "Teamwork"). In this experiment, payoffs are computed the same as in the previous experiment (namely, 1.6 times the amount of the public pool split evenly amongst the players). Since there are multiple rounds, the payoff and amount not contributed are summed to determine each players endowment for the next round. Within each priming condition, we compare the average contribution in the first round compared to the fifth round. We also compare the contributions between priming conditions, checking that there was an initial disparity that ultimately begins to fade.

\color{red}

\subsubsection{Real-World Case Studies}

SEE RESULTS, THERE'S A BIG BULLET POINT LIST OF EVAL / RESULTS COMBINED I'M TRYING TO FIGURE OUT HOW TO SEPARATE. 

TALK ABOUT HOW THESE CONNECT TO PROSOCIAL SITUATIONS HERE?

\color{black}

==> 4_results.tex <==
\section{Results}

Based on the results from our experiments, we answer our research questions.

\subsection{\underline{RQ1}: Can multi-agent LLM system simulations replicate behaviors observed in PGG lab experiments with human subjects?}

Towards answering this question, we simulate treatments from three different lab experiments with human subjects: (1) priming via game name, (2) transparency of contributions, and (3) variations in endowment. In the first two experiments, LLM-agents replicate the direction of effects with statistical significance, but overestimates the magnitude. In the third experiment, LLM-agents replicate the direction of effects but the effect is not statistically significant, although this is likely due to lack of data. \textbf{Overall, we conclude that LLM-agents are able to replicate the direction of the effect of priming and transparency treatments, \color{orange}but testing their ability to replicate the effect of a varied endowment requires further simulations.\color{black}}

\subsubsection{Does priming LLM agents via game name replicate the effect of priming humans via game name?}

In experiments with human subjects, participants presented the PGG as the "Teamwork Game" contributed roughly 60\% of their endowments while participants presented the game as the "Taxation Game" contributed roughly 40\% of their endowments \cite{Eriksson_Strimling_2014}. Across ten simulations on average, LLM agents presented the PGG as the "Teamwork Game" (Alice and Bob) contributed approximately 70\% of their \$20 endowment. In comparison, agents presented the PGG as the "Taxation Game" (Casey and David) contributed only approximately 30\% of their endowment to the public pool. These results are summarized in Figure \ref{1Agraph}. A t-test shows that the difference in contributions between the two groups is statistically significant at the p < 0.01 level  
(\(t = 7.92, p < 1\text{e}{-8} \)).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/1A.png}
    \caption{Average contributions for "Teamwork" and "Taxation" priming conditions in simulations with LLM-agents and experiments with human subjects. Average contributions are above 60\% in the "Teamwork" priming condition for both groups. Average contributions are below 40\% in the "Taxation" priming condition for both groups.}
    \label{1Agraph}
\end{figure}

\textbf{From these results, we conclude that priming LLM agents by presenting the PGG under different names replicates the direction of the effect of doing the same on humans, but may overestimate the magnitude.}

\subsubsection{Does introducing transparency in contribution between LLM agents replicate the effect of introducing transparency in contribution between humans?}

In experiments with human subjects, participants contributed on average 6\% more of their endowment under transparency conditions as compared to no transparency. \cite{transparencytwo}. Across five simulations of each condition (ten simulations total) on average, LLM agents playing the PGG with transparency contributed approximately 60\% of their 20\$ endowment, whereas LLM agents playing the PGG without transparency contributed only approximately 35\% of their endowment. \color{orange}These results are summarized in Figure \ref{1Bgraph}\color{black}. A t-test shows that the difference in contributions between the two groups is statistically significant at the p < 0.05 level  
(\(t = 2.23, p = 0.031 \)).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/1B.png}
    \caption{Average contributions with and without transparency for simulations. Only the difference in contribution is listed in the lab experiment from which this treatment/effect was found. \cite{transparencytwo}.}
    \label{1Bgraph}
\end{figure}

\textbf{From these results, we conclude that introducing transparency of contributions in PGGs with LLM agents replicates the direction of the effect of doing the same on humans, but may overestimate the magnitude.}

% "If controlling for the MPCR, however, as is done in specifications (6) and (8), the positive effect of F.indichoice and the negative effect of F.indipayoffs have a larger magnitude and turn significant at the 5% level. The share contributed tends to be about 6 percentage points higher than in cases where players receive feedback about the distribution of choices in their group."


\subsubsection{Does varying the endowments of LLM agents replicate the effect of varying endowments of humans?}

In experiments with human subjects, it was found "poor" and "medium" wealth individuals contributed roughly the same amount in equal and varied endowment conditions, whereas "rich" individuals contributed more in the equal endowment condition than in the varied endowment condition \cite{HARGREAVESHEAP20164}. Across five simulations each of \$20-\$20-\$20, \$50-\$50-\$50, and \$80-\$80-\$80 equal endowment conditions, LLM agents on average contributed approximately 39\%, 48\%, and 63\% of their endowments, respectively. In five simulations of a \$20-\$50-\$80 varied endowment condition, on average the LLM agent given \$20 contributed approximately 35\%; the LLM agent given \$50 contributed approximately 42\%; and the LLM agent given \$80 contribute approximately 44\%. Thus, the contribution for agents endowed with \$20 was roughly the same between the equal and varied endowment conditions, whereas agents endowed with \$50 and \$80 both contributed less in the varied condition. These results are summarized in Table \ref{1Cgraph}. T-tests shows that there is no statistically significant difference at the p < 0.1 between the contributions of LLM agents endowed with \$20 in the equal and varied endowment condition (\(t = 0.18, p = 0.86 \)), nor for the \$50 (\(t = -0.56, p = 0.58 \)) endowment - both results mirroring those of human subjects. However, a t-test shows that the difference between the contributions of LLM agents endowed with \$80 is also not statistically significant at the p < 0.1 level (\(t = 1.25, p = 0.23 \)).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{images/1C.png}  % Change this value to make the figure larger
    \caption{Average contributions for equal and varied endowment conditions in simulations with LLM-agents and experiments with human subjects. Average contributions are roughly the same for humans and LLM-agents in the equal and varied endowment conditions with \$20 and \$50 endowments. Average contributions are lower in the varied condition than in the fixed condition with \$80 endowments.}
    \label{1Cgraph}
\end{figure}

% \begin{table}[htbp]
% \centering
% \begin{tabular}{|>{\columncolor{gray!20}}c|c|c|c|}
% \hline
% \rowcolor{gray!20}\multicolumn{1}{|c|}{} & \multicolumn{3}{c|}{\textbf{Initial Endowment}} \\ \hline
% \rowcolor{gray!20}\textbf{Condition} & \$20 & \$50 & \$80 \\ \hline
% Equal & 39\% & 48\% & 63\% \\ \hline
% Varied & 35\% & 42\% & 44\% \\ \hline
% p-value & 0.86 & 0.58 & 0.23 \\ \hline
% t-stat & 0.18 & -0.56 & 1.25 \\ \hline
% \end{tabular}
% \caption{\color{red}IK THIS TABLE MAKES NO SENSE\color{black}}
% \label{variedend}
% \end{table}

\color{orange}
From these results, we cannot fully conclude that LLM agents are affected by varying endowments in the same way as humans. However, the lack of difference between the average contribution in the equal and varied condition with endowments of \$20 and \$50 along with the difference between the averages in the equal and varied endowment conditions does suggest that varying endowments does have an impact similar to the effect observed in humans. The lack of statistical significance could be a result of the limited and unequal number of data points in both groups of comparison (for every endowment amount, there are 15 contributions in the equal endowment condition compared  to only 5 contributions in the varied endowment condition in our simulations).
\color{black}

\subsection{\underline{RQ2}: Can multi-agent LLM system simulations replicate human behavior extrapolated from combining the behaviors observed in multiple lab experiments with human subjects?}

Towards answering this question, we simulate two experiments designed as a combination of multiple lab experiments with human subjects: \color{red}(1) takes a priming methodology and effect from experiments with human subjects of different cooperative games than the PGG to see if the effect holds for the PGG, and (2) uses a priming methodology used on the one-shot PGG and measures if it has the same effect over multiple rounds similar to the way in which priming affects different economic games than the PGG. \color{black} \textbf{From the results of these experiments, we conclude that multi-agent LLM system simulations do replicate behavior extrapolated from combining the behaviors observed in multiple lab experiments with human subjects.}

\subsubsection{Does priming LLM agents with sentences known to increase/decrease generosity in humans have that effect in simulations of the PGG?}

In experiments of other cooperation games, priming participants via sentences alluding to "unity" resulted in participants being more generous than participants primed via sentences alluding to "proportionality" \cite{moralsmatter}. In ten simulations, LLM agents primed with the sentences alluding to "unity" (Alice and Bob) contributed on average approximately 65\% of their initial endowment. In comparison, agents primed with the sentences alluding to "proportionality" (Casey and David) contributed on average only approximately 30\% of their endowment to the public pool. The results are summarized in Figure \ref{2Agraph}. A t-test shows that the difference in contributions between the two groups is statistically significant at the p < 0.01 level (\(t = 8.76, p < 1\text{e}{-9} \)).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/2A.png}
    \caption{Average contributions for either "unity" or "proportionality" priming conditions. Average contributions under the "unity" condition are significantly higher than that under the "proportionality" condition.}
    \label{2Agraph}
\end{figure}

\textbf{From these results, we conclude that priming LLM agents with sentences known to increase/decrease generosity in humans does result in higher/lower contributions in simulations of the PGG.}

\subsubsection{Does the effect of priming LLM agents via game name in multi-round PGGs fade over time, like priming has been observed to fade over time in other experiments with human subjects?}
\bigskip
In experiments of competition games with human subjects, the effect of primings have been found to fade over time \cite{JIMENEZJIMENEZ201594}. In ten simulations, LLM agents presented a five-round PGG as the "Teamwork Game" (Alice and Bob) on average contributed 75\% of their initial endowment in the first round, compared to 55\% of their initial endowment in the fifth round. In comparison, agents presented the PGG as the "Taxation Game" (Casey and David) contributed 30\% of their initial endowment in the first round, compared to 45\% of their initial endowment in the fifth round. Hence, for both priming conditions, the average contribution was closer to 50\% of the initial endowment in the fifth round than in the first, meaning the effect of the priming was less pronounced in the fifth round than the first. The results are summarized in Figure \ref{2Bgraph}. T-tests show that the difference in contribution amount between the rounds is statistically significant for the "Teamwork" priming condition at the p < 0.01 level (\(t = 4.32, p = 0.002 \)) and for the "Taxation" priming condition at the p < 0.05 level (\(t = -2.30, p = 0.047 \)).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/2B.png}
    \caption{Average contributions in the first and fifth rounds for either "Teamwork" and "Taxation" priming conditions. Average contributions in the fifth round are closer to 50\% of the initial endowment, the average amount contributed without any priming \cite{labexperiments}.}
    \label{2Bgraph}
\end{figure}

\textbf{From these results, we conclude that the effect of priming LLM agents fades over time, as observed in experiments with human subjects.} The "Taxation" priming condition specifically suggests that the difference between first and fifth round contributions is not because contributions in PGGs with human subjects decrease over time \cite{labexperiments}, but rather likely the consequence of a fading priming effect.

\subsection{\underline{RQ3}: What are required mechanisms for simulations to
inform policy-makers regarding real-world situations?} 

\color{purple}

\begin{itemize}
\item[1.] Classroom with Late Policies
\begin{itemize}
\item We simulate a classroom setting, where students have 5 assignments to submit over the course of a semester.
\item We try varying late-assignment policies (lenient - all late assignments accepted, harsh - late assignments not accepted, medium - 20\% grade penalty for each late day). 
\item We add perturbations to student lives that reasonably would affect their ability to turn in assignments on time: (1) having a midterm and (2) a particular assignment being especially challenging.
\item We also give students personality types: that of a procrastinator, an overachiever, and someone who "values work-life balance."
\item We wanted to see if multi-agent LLM systems simulated reasonable interactions and dynamics within a classroom.
\item We sought to examine how students would (1) work together and (2) communicate with one another and the teacher.
\item In preliminary simulations with one room, a classroom, we found that student agents proposed working together to other student agents.
\item \color{red}Generally, we saw that procrastinators would suggest collaboration most frequently.\color{purple}
\item Student agents also would ask questions to the teacher that were both individual (ex. requesting a review) and for the group (ex. clarifying an assignment). 
\item But everybody in the class would be distracted by them.
\item Therefore, we added two rooms to the simulation environment to enable easier communication: the teacher's office, and a student work room.
\item In simulations with the lenient late policy, communication was somewhat similar with or without the added rooms.
\item Students did move into the work room to "work" as per their directives. 
\item They also used the office to ask questions to the teacher.
\item But students discussed working together in a similar way and at roughly the same frequency.
\item This was true after adding perturbations too.
\item In simulations with the medium late policy, the ways in which proposed collaboration changed once perturbations were added.
\item As opposed to broadly discussing working together, student agents sometimes asked to see other agent's assignments to copy in the work room. 
\item \color{red}Generally, we saw that procrastinators would suggest cheating most frequently.\color{purple}
\item In simulations with the harsh late policy, we saw this behavior before even adding perturbations.
\item \color{red}This makes sense, because students have been found to be more likely to cheat on exams if they have strict teachers.\color{purple}
\item We ran simulations under the lenient (LLP), harsh (HLP), and medium late policies (MLP).
\item We ran simulations under three perturbation conditions: (P0) without any, (P1) students having a midterm during the 3rd assignment, and (P2) students having the midterm AND the 2nd assignment being especially challenging.
\item We ran five simulations of each combination of late policy and perturbation (LLP-P0, LLP-P1, LLP-P2, HLP-P0, HLP-P1, HLP-P2, MLP-0, MLP-1, and MLP-2), or 45 simulations total.
\item We recorded if students (1) proposed collaboration, (2) proposed a form of cheating, and (3) communicated with the teacher.
\item \color{red}We did not record which student initiated each of the types of actions. We also did not record at which assignment it occurred.\color{purple}
\item The results are summarized in Table \ref{teachingsims} and Figure \ref{3Agraph}.
\item{\begin{center}
\begin{table}[H]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{10pt}
\begin{tabular}{|>{\columncolor{gray!20}\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|} 
 \hline
 \rowcolor{gray!20} \textbf{Condition} & \textbf{Collaboration} & \textbf{Cheating} & \textbf{Communication with Teacher} \\ 
 \hline\hline
 \textbf{LLP-P0} & 40\% & 0\% & 60\% \\ 
 \hline
 \textbf{LLP-P1} & 60\% & 0\% & 40\% \\ 
 \hline
 \textbf{LLP-P2} & 60\% & 0\% & 80\% \\ 
 \hline
 \textbf{MLP-P0} & 60\% & 0\% & 80\% \\ 
 \hline
 \textbf{MLP-P1} & 80\% & 20\% & 80\% \\ 
 \hline
 \textbf{MLP-P2} & 100\% & 20\% & 100\% \\ 
 \hline
 \textbf{HLP-P0} & 100\% & 20\% & 100\% \\ 
 \hline
 \textbf{HLP-P1} & 100\% & 20\% & 100\% \\ 
 \hline
 \textbf{HLP-P2} & 100\% & 60\% & 100\% \\ 
 \hline
\end{tabular}
\caption{\label{teachingsims}Percentage of simulations in which the specified behavior was observed for all 9 simulation conditions.}
\end{table}
\end{center}
}
\item{\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{images/3A.png}  % Change this value to make the figure larger
    \caption{Percentage of simulations in which the specified behavior was observed for all 9 simulation conditions.}
    \label{3Agraph}
\end{figure}}
\item \color{purple} We find that: (1) rooms enabled private communication which LLM-agents used to propose cheating, and (2) LLM-agents seemed to reasonably respond to changes in late policy and perturbations.
\end{itemize}
\end{itemize}

\begin{itemize}
\item[2.] Shopping Cart Return
\begin{itemize}
\item We simulate a store parking lot, where there are specific shopping cart return locations.
\item Each simulation has one agent with a plan to decide whether or not to return their shopping cart.
\item We try two perturbations that might contribute to someone not returning their cart: (1) being far from the receptacle (FFR), and (2) having a child whom should not be left unattended (HAC). \cite{scientificamerican2020shoppingcarts}
\item We have two rooms: the shopper agents car and the receptacle.
\item We find that despite the perturbations, shopper agents arill frequently return their carts if it the perturbation is merely stated ("you are far from the receptacle," and "you have a child")
\item However, alluding to what is at stake as a result of the perturbation starts causing shopper agents to stop returning their carts as often ("you are \textit{parked across the parking lot} from the receptacle," and "you have a \textit{five-month old} child").
\item We present this as \color{red}stake-prompting (SP), a way in which to guide LLM-agents towards acting more in-line with humans.\color{purple}
\item We ran five simulations of either perturbation (FFR and HAC) with and without prompts alluding to what is at stake, or 20 simulations total.
\item The results are summarized in Table ~\ref{shoppingcartsims} and Figure \ref{3Bgraph}.
\item{\begin{center}
\begin{table}[H]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{10pt}
\begin{tabular}{|>{\columncolor{gray!20}\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|} 
 \hline
 \rowcolor{gray!20} \textbf{Perturbation} & \textbf{Without SP} & \textbf{With SP} \\ 
 \hline\hline
 \textbf{FRB} & 100\% & 40\% \\ 
 \hline
 \textbf{HAC} & 60\% & 20\% \\ 
 \hline
\end{tabular}
\caption{Percentage of simulations in which the shopper agent decided to \color{red} MISSING THOUGHT HERE their shopping cart for both perturbations tested and under either prompting condition. ALSO, IF THE GRAPH HAS CRYTIC ACRYNYMS like SP FRR HAC, you MUST define in the cpation. \color{black}}
\label{shoppingcartsims}
\end{table}
\end{center}
}
\item{\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{images/3B.png}
    \caption{Percentage of simulations in which the shopper agent decided to their shopping cart for both perturbations tested and under either prompting condition.}
    \label{3Bgraph}
\end{figure}}
\item We find that alluding to what is at stake caused LLM-agents to be more \color{red} affected by perturbations more like people\color{black}.
\end{itemize}
\end{itemize}

\begin{itemize}
\item[3.] Graffiti \& Littering
\begin{itemize}
\item Finally, we simulate two scenarios: (1) a bike-parking station, where a piece of paper is left on the handlebars. people must choose whether or not to litter - there is a no littering sign but no trash can. there is either grafitti on the wall or not, people more likely to litter when there is graffitti. (2) a envelope with cash visible hanging outside of a mailbox. the mail box either has graffiti on it or not.
\item \color{red}LLM-simulations show .... WIP .... but looks like first sort of should be true, second one looks unlikely but is interesting they won't steal?\color{black}
\item IDEALLY WOULD BE: WE TRIED X AND IT DID NOT WORK... ADDING Y GOT US CLOSER TO REPLICATING
\end{itemize}
\end{itemize}

\color{black}






==> source/1_intro.tex <==
\section{Introduction}

% //Motivation: 
Human prosocial cooperation is essential for our collective health, education, and welfare, but cooperation is also difficult to maintain. 
When everyone pays taxes, societies can collectively benefit from public goods like roads, safety nets, and schools. However, individuals who do not contribute get to keep their wealth and still benefit from public goods. 
This "freeloading" behavior can eventually erode public trust and lead to a tragedy of the commons. 
Psychologists study this behavior in the lab using games like the public goods game (PPG) where a group of 3 or more people all decide how much to donate to a public fund. Public funds are multiplied then redistributed equally. If everyone donates, everyone is better off. However, if someone decides not to donate, they benefit more than others - they receive the public funds and get to keep their initial wealth. Eventually, this freeloading behavior discourages everyone else from donating, and public funds are emptied. 
Encouraging cooperation is thus important and psychologists have discovered many factors that affect prosocial behavior such as priming (positive framing), transparency (social pressure), and varying endowments (inequality).  

% //Problem:
However, human behavior in the lab is different than in the wild. In the lab, people’s choices and actions are bounded: they only get to choose from a small set of options, such as a choice from a menu of how much to donate. But in the wild, choices are unbounded. Humans exhibit more complex behaviors including lying, cheating, persuasion, and gaming the system. These are often the behaviors that cause programs and policies to fail. They’re also very difficult to foresee. Studying human behavior in the wild using experiments is very challenging. It requires large numbers of people interacting, creating a control group or a matched sample to compare to, and numerous runs a to achieve statistical significance. This is almost never done, and thus policies affecting human cooperative behavior are rarely informed by experimental evidence.

% //Approach:
Multi-agent LLM systems have the potential to simulate complex human behavior and interactions. 
They exhibit human-like behavior \cite{park2023generativeagentsinteractivesimulacra}, including doing actions they were not explicitly told to do (emergent behavior), thus displaying the potential for unbounded actions. 
Beyond human-like behavior, LLMs and multi-agent LLM systems have also shown a capacity to replicate actual human behavior seen in lab studies. This includes 70 psychology experiments \cite{aher2023usinglargelanguagemodels, hewitt2024predicting}, and multi-player economic games with strategic thinking about what other players will do, such as the 
%like in many game theoretic games, like the 
multi-turn Ultimatum Game \cite{sreedhar2024simulatinghumanstrategicbehavior} and auctions \cite{manning2024automated}. 
For a simulation to be useful, it does not necessarily have to replicate human behavior exactly, but it does have to exhibit a rich enough set of actions consistent with behaviors that are observed, and provide evidence that the results can generalize to previously unseen situations.
To lay the groundwork for a future where policy makers can ask LLM-agents to simulate human behavior in response to policy changes, we address the following  questions:
\begin{itemize}
    \item[(1)] Do multi-agent LLM systems understand human cooperative behavior well enough to simulate it, even in a lab setting?
    \item[(2)] Are multi-agent LLM systems simply echoing the results from previous papers, or can effects transfer across papers and apply more broadly?
    \item[(3)] To what extent are multi-agent LLMs complex enough to simulate the rich set of unbounded options, actions, and interactions people do in the real world, outside of the lab? 
    \item[(4)] To see the complex interactions observed in the real world, what simulation mechanisms do we have to add to the set up of the system?
\end{itemize}
% (1) Do multi-agent LLM systems understand human cooperative behavior well enough to simulate it, even in a lab setting?
% (2) Are multi-agent LLM systems simply echoing the results from previous papers, or can effects transfer across papers and apply more broadly?
% (3) To what extent are multi-agent LLMs complex enough to simulate the rich set of unbounded options, actions, and interactions people do in the real world, outside of the lab? 
% (4) To see the complex interactions observed in the real world, what simulation mechanisms do we have to add to the set up of the system?

% //Results:
Our experiments show that multi-agent LLM systems replicate findings of three lab studies of human cooperative prosocial behavior, showing that LLM-agents are consistent with humans in their responses to priming, transparency and varying endowments. The simulation accurately replicated the direction of the effect (positive or negative), but often exaggerated the effect size. In addition to replicating the findings of previous studies, we show that multi-agent LLM systems can apply insights from other games to the PGG. Specifically, we demonstrate that two priming effects previously studied in other games — but not tested in the PGG — also have a similar impact on behavior in the PGG. This indicates that multi-agent LLM systems are not simply echoing existing research but have a broader ability to simulate psychological mechanisms across different games, situations, and simulations.

We also show that for two real world situations, we do see complex, unbounded behavior consistent with anecdotal evidence. For a classroom scenario with a teacher testing various late policies, we find that when late policies are strict and assignments are hard, we can enable the behavior of cheating to emerge. For a shopping center parking lot scenario, we find that LLM-agents can be affected by external conditions like humans in returning or not returning their shopping cart. For both scenarios, simple mechanisms had to be added to the simulation to see these effects. For cheating, the simulation had to include communication channels like a private student room to initiate the communication needed for a behavior like cheating. For agents to not return their cart, their provided information had to allude to what was at stake as a result of their external condition.


% //Discussion:
Altogether, we conclude that multi-agent LLM systems show remarkable promise towards simulating human prosocial behavior.  
For broader real-world scenarios, we find that there remain additional mechanisms to identify in order for multi-agent LLM systems to simulate cooperative behavior, including (1) creating communication mechanisms that allow agents to coordinate behavior privately and (2) make sure the stakes (or incentives) driving behavior are clear. 
These are far from the only mechanisms needed, and there is much future work to discover more mechanisms, but there is reason to believe that these mechanisms
% might be fairly broad, and 
will be broadly applicable across domains. 
Our simulations show that in the future, there is a potential for multi-agent LLM simulations to be useful in informing policy makers. Currently, LLM-agents can simulate the general direction of human behavioral effects, although they struggle to accurately capture the magnitude. While fine-tuning may improve this, it likely never perfectly replicates human behavior. 
Nevertheless, the ability to simulate directional trends can still help policymakers anticipate potential policy outcomes. Given the complexity and high social stakes of such decisions, even preliminary simulations could provide a valuable framework for exploring possible scenarios and guiding decision-making.




% MOTIVATION 

% Human collaboration in its ideal form involves a  kind of fluid sharing of ideas and resources. However, humans working together is a tenuous proposition; it requires people to sometimes sacrifice closely held ideas or possessions. As a result, many situations lead to dysfunctional collaboration. Human collaboration is so important that psychologists study it in a well-defined setting called the public goods game (PGG). This game is directly related to many situations. Taxation is a case in point: A community can do big things that can benefit everyone if everyone contributes their fair share. However, when a single agent benefits from shared infrastructure and simply stops donating, they are essentially freeloading of the contributions of others. If the practice spreads, the infrastructure deteriorates, and the resulting situation is called the tragedy of the commons. Because this is so important, psychologists study the many ways to influence people's decisions to donate to the public good.  For example, priming and transparency are common techniques shown to increase contributions. 


% \bigskip

% \color{red}PROBLEM
% Doing experiments is hard, especially on large groups. Experiments also may not translate into practice. We seek to understand the way in which AI can simulate human behavior in the PGG. We do this in three ways. We see if AIs can simulate previous results of papers. We then see if AI can combine ...~


% An important assumption of lab experiments is that the observed behavior is generalizable to the real world \cite{labexperiments} - human behavior in the real world is more complex than in a lab setting. In lab experiments, the environment is mostly fixed; people's choices of actions are often limited, and defined by the experiments - for example, people can either PAY or NOT PAY. But in the real world, the environment and the action space is unbounded. People can do other actions like cheat - people can persuade people they've payed when they have not. People can even even make it seem like they are unable to pay when they can  (for example, tax havens, usually on boundary of legality, allow people to hide income in order to reduce the amount of tax they pay). Previous research suggests that LLMs, and multi-agent LLM systems in particular, have potential to display these "unscripted" actions in simulation \cite{horton2023largelanguagemodelssimulated} and therefore help policy makers forsee the ways in which actual people will react in response to their proposals. This is accomplished via a lower stakes method without the actual consequences that would ensue from enacting a new untested policy.

% % Human behavior in the real world is more complex than in a lab setting. In a lab, the environment is fixed, and user’s choices of actions are often limited, and defined by the experimenters - for example, users can either PAY or NOT PAY. But in the real world, the environment and the action space is unbounded. Users can do other actions like cheat, users can persuade people they’ve PAYED when they have not. Users have things in their environment like tax havens that allow them to avoid taxes semi-legally. LLMs are interesting way to potential see see of these “unscripted” actions in simulation, in order to help policy makers SEE REAL USER BEHAVIOR, BEYOND LAB BEHAVIOR.

% \color{black}

% \sout{When creating policies, plans, or designs for people, it is challenging for designers to foresee all of the ways in which people may reason and behave. Simulations can be very helpful in this context, but it is challenging to accurately model (1) the ways in which people collaborate, both allowed (i.e., working together to solve problems) and not (i.e., cheating/collusion) and (2) the ways in which people communicate (what and with whom). People do not collaborate or communicate uniformly – their personalities \cite{mccrae2008five}, experiences \cite{Kidd2013}, and circumstances \cite{mullainathan2013scarcity} all affect their decision making and behavior. However, these factors are important to accurately consider in simulations to enable designers to anticipate ways in which people may react to or circumvent proposed policies.}
 
% \color{red}APPROACH\color{black}

% Recently, multi-agent LLM systems have shown remarkable capabilities in simulating human-like knowledge and behavior in a range of domains, including but not limited to social systems \cite{park2023generativeagentsinteractivesimulacra, park2022socialsimulacracreatingpopulated}, entertainment \cite{Callison_Burch_2022}, education \cite{gpteach}, economics \cite{horton2023largelanguagemodelssimulated, aher2023usinglargelanguagemodels}, and judicial trials \cite{hamilton2023blindjudgementagentbasedsupreme}. Specifically, LLMs have also been shown to be able to replicate behavior observed in prior human experiments \cite{hewitt2024predicting}, allowing researchers to benchmark behavior in LLM-simulations with actual human behavior. We extend this by focusing on the interesting case of prosocial situations – where people can voluntarily act in a way that benefits another person or society as a whole. We (1) replicate treatments from prior lab experiments with human subjects in variations of the PGG to confirm LLMs capture observed human behavior; (2) simulate scenarios that combine treatments used in lab experiments of other games and the PGG to verify that LLMs are not parroting published literature; and (3) simulate two real-world scenarios (a classroom with late-policies and a grocery store shopping cart return) towards identifying mechanisms necessary to enable human-like behavior.
 
% The public goods game (PGG) is a classic economics experiment where players begin with a set endowment and can choose to voluntarily contribute a portion of it to a public pool, which will be multiplied by a factor then distributed evenly amongst the players. Players also keep the amount they do not contribute. In the PGG, the group’s total payoff is maximized when everyone contributes all of their initial endowment to the public pool. However, economic theory dictates that the most profitable strategy for individual players is to make zero contribution to the public pool, because they may benefit from the contributions of other more charitable people while at the same time hoarding their personal wealth. However, these decisions are rarely seen in human experiments – human players generally voluntarily contribute a portion of their endowment to the pot, although contribution levels can vary \cite{stuffinpgg}. Furthermore, priming \cite{Eriksson_Strimling_2014}, variations in endowment \cite{HARGREAVESHEAP20164}, and transparency of communication \cite{transparencyandcooperation} can greatly affect outcomes. \color{red}ITS LIKE TAXES\color{black}

% \color{red}RESULTS\color{black}
 
% We use the PGG to test if LLMs act like humans in prosocial contexts. We evaluate whether LLM-agents are affected by priming, transparency (i.e., social pressures), and varying endowments (i.e., unequal resources) similar to the ways in which humans are by extracting human actions from economics literature. We also verify the robustness of this replication by also testing combinations of existing literature, examining whether LLM simulations yield results consistent with reasonable extrapolation of what would happen based on the results from each experiment. We find that in replicating lab experiments of the PGG, multi-agent LLM systems display the differences observed as a result of experimental treatments (priming, transparency, and varying endowments), but with a larger effect-size. In combining experiments, we find that multi-agent LLM systems display the expected differences of experimental treatments.

% \color{orange}We try simulating two real-world scenarios as case studies towards beginning to identify specific mechanisms required for simulations to display plausible human communication and collaboration. First, we simulate a classroom setting with changing late policies and various perturbations to student lives, finding that even in the most pressing of conditions, student-agents do not ever consider cheating - until a separate room is introduced that only student-agents can enter and communicate with one another without the professor-agent overhearing. Second, we simulate shopping-cart returns in a store parking lot with various conditions affecting shopper-agents (ex. having a child with them, running late to a meeting, etc.), finding that shoper-agents almost always return their cart regardless of the conditions affecting them - until the prompts of the conditions allude to or explicitly state the consequences of them.\color{black}

% Altogether, we conclude that multi-agent LLM systems show remarkable promise towards simulating human prosocial behavior. However, for broader real-world scenarios, we find that there remain additional mechanisms to identify and introduce in order for multi-agent LLM systems to simulate plausible behavior, identifying two of them - partitioning agents into rooms to allow for private communication and defining consequences as part of the prompting - via case studies, a repeatable process for identifying further necessary mechanisms. Altogether, the results of our simulations of lab experiments and real-world case studies suggest a future in which simulations using multi-agent LLM systems will be a powerful tool to assist policy-makers.

==> source/2_related_work.tex <==
\section{Related Work}

\subsection{The Public Goods Game}

The public goods game (PGG) is a particularly important case of human cooperative prosocial behavior studied by psychologists and economists. In the PGG, a set of three or more players are each given an endowment of money, of which they choose a portion of to voluntarily contribute in-private to a public pool. The public pool will then be multiplied by a factor, say 2, then redistributed evenly amongst the players. In a game with four players, if every player has a \$20 endowment and contributes half of their endowment, \$10, each player will receive a payoff of \$30: \$10 from the amount of their endowment they kept and \$20 from the payoff from the public pool. If each player donates nothing, they all simply keep their initial endowment of \$20 without any additional payoff. In the PGG, working cooperatively can be mutually beneficial. However, if a player decides not to contribute to the public pool, the player can increase the payoff — in the example previously discussed, if one player decides not to contribute to the public pool, the payoff is \$35 — \$20 from the endowment the player kept, and \$15 from the payoff from the public pool. Hence, not contributing to the public pool can result in a greater payoff for an individual, despite contribution to the public pool by \textit{someone} being necessary for there to be any additional payoff for players. This game mimics situations involving prosocial behavior in the real-world, such as taxation — when paying taxes, people are forced to contribute some of their own money to a public pool to develop infrastructure and services for the broader community. People can even try to avoid paying taxes through tax havens or loopholes and freeload off public goods.

Lab experiments with human subjects show that in single-round (one-shot) PGGs, people do typically contribute a portion of their endowment — on average, 50\%. When the game is played for multiple rounds, the amount that players contribute decreases each round, until it is effectively zero \cite{labexperiments}. However, introducing variations to the game can increase or decrease prosocial behavior. Priming participants by presenting the game under different names \cite{Eriksson_Strimling_2014} or having participants primed with words alluding to cooperation before playing the PGG \cite{drouvelis2015priming} increases their average contribution amount. Introducing transparency of contributions also increases average contributions — having participants write their contribution on a blackboard after each round \cite{rege2004impact} or announce their contributions publicly \cite{transparencytwo} increases the average contributions made in the PGG. Finally, varying the endowments that players have to begin with in the PGG also has an effect on average contributions — in experiments with individuals given low (\$20), medium (\$50), and high (\$80) endowments, individuals with the low and medium endowments contributed the same amount in games where endowments were the same as in games where endowments were varied. However, individuals with the high endowment contributed much less in games where endowments were varied \cite{HARGREAVESHEAP20164}.
% were varied than in games where endowments were equal 

These effects are not limited to the PGG and can be seen in select real-world scenarios. In fundraisers, audiences may be primed to cooperate towards a common goal. In many settings, pledges are made publicly (that is, transparently), which increases donations \cite{Bhati2020-xw, Oppenheimer2011-zh}. Similar strategies are used by policy makers seeking to levy taxes for a bridge or other local public goods \cite{parks2013cooperation}. Furthermore, lower class individuals have been demonstrated to be more prosocial than their higher class counterparts in studies of generosity, charity, trust, and helpfulness \cite{piff2010having}. Overall, although free-loaders may be able to benefit off of public goods — whether in the PGG or in the real world — there are strategies that policy makers can use to increase prosocial behavior.

% \color{red}One can often see the above results play out in fund-raising events. Those doing fundraising will prime an audience to cooperate toward a common goal. In many settings, pledges are made publicly: this increases transparency, which in turn increases donations \cite{Bhati2020-xw, Oppenheimer2011-zh}. Similar advice is given to policy makers seeking to levy taxes for a bridge or other local public goods \cite{parks2013cooperation}. \color{black}


% \section{Background on the Public Goods Game}
% Background:
% A particularly important instance of human cooperative prosocial behavior studied by psychologists and economists is the public goods game (PGG). 
% In the PPG, a set of 3 or more players are each given an endowment of money, and they can choose to voluntarily contribute a portion to a public pool. 
% The public pool will then be multiplied by a factor (typically 2), and then redistributed evenly. 
% If the game has 4 players and every player has a $20 endowment and donates 50\% to the public good, each player has \$30 in the end 
% ($10 from their endowment + (\$20 from splitting the pot after multiplication). 
% But if each player donates nothing, they all simply keep the \$20. 
% In PPG, working collaboratively can be mutually beneficial. 
% However, if one player decided not to donate, the 3 players that donate all get \$25 (\$10+\$15 for the split pot), and the player that didn’t donate gets \$35 (\$20+\$15 from the split pot). 
% The PPG game can broadly mimic situations of prosocial behavior, such as taxation, ….., making it a valuable game to simulate. 


% Human subject studies show that when a single round of PPG is played, people do act prosoically and donate X\% of the money on average. 
% However, If the game is played for multiple rounds, the amount the players donate drops every round, until it is effectively zero. 
% However, factors like primincy and transparency can increase prosocial behavior.
% These lab results are important in that they show that humans do act prosocially and can be prompted to do so. 
% These results can guide policy makers, but don’t capture of complexity of most real world simulations or allow policy makers to compare two different policies. 

% BIG THING: IF YOU DON'T CONTRIBUTE, YOU GET MASSIVE PAYOFFS!

% \section{Related Work}

% \subsection{Human Prosocial Behavior?}

% \subsubsection{prosocial behavior / cooperation / big picture}

% \subsubsection{Human Behavior in Public Goods Game Experiments}

% \sout{Studies with human subjects demonstrate that humans often act "irrationally" in economic games, choosing to value social norms over profit maximization. This remains true for the PGG.} Humans are often better off when we collaborate with one another, when we all pay our taxes, when we shovel our sidewalks, when we pull over for ambulances.. but in any situation where everyone should contribute, there's ~stuff~ that happens. Someone prioritizes themselves over others, or someone cheats, or groups of people collude together. 

% In the PGG, total payoff is maximized when all participants contribute their entire endowment to the public pool, while individual profit is maximized when the individual participant contributes nothing \cite{6d947858-4a17-3462-9053-fc55b58ffee1}. However, in experiments with human subjects, participants typically contribute roughly half of their endowment in one-shot and the first round of multi-round PGGs \cite{labexperiments, stuffinpgg}.

% \color{red}explain, priming.... transparency..... endowments.....\color{black}

% Moreover, the behavior of human participants in such experiments is significantly affected by various treatments. More generous behavoir follows priming for teamwork, cooperation and unity; less generous behavior follows priming for taxation, competition, or proportionality concepts reduces their willingness to contribute \cite{Eriksson_Strimling_2014, moralsmatter, drouvelis2015priming}. Transparency in contributions (i.e, participants make their contributions publicly for all other participants to see) also results in higher contribution amounts as compared to without \cite{KHADJAVI2017468, transparencytwo}. Giving different players different endowment amount also leads to interesting results, with "rich" participants contributing less to the public pool when the remaining participants have lower endowments as compared to when everybody has the same endowment \cite{HARGREAVESHEAP20164}. \color{red} SO WHAT \color{black}

% \color{red}, Oppenheimer2011-zh}. Similar advice is given to policy makers seeking to levy taxes for a bridge or other local public goods \cite{parks2013cooperation}. \color{black}



\subsection{Replicating Bounded Scenarios with Human Subjects using LLM Simulations}

Prior research in psychology, economics, and artificial intelligence has compared results from LLM simulations to experimental data from studies with human subjects, finding that outcomes in LLM simulations generally mirror those from the real world. Using a single LLM, past work has been able to replicate results from economic and psychology experiments with humans, including the Ultimatum Game, Garden Path Sentences, Milgram Shock Experiment, and Wisdom of Crowds \cite{aher2023usinglargelanguagemodels}. Single LLMs have also been able to replicate results from an archive of seventy social science experiments — both published and unpublished. In published studies, LLM simulation results had correlation coefficient of r = 0.85 with results from lab experiments with humans. In unpublished studies which could not have appeared in the LLM's training data, the correlation was also strikingly high (r = 0.90) \cite{hewitt2024predicting}. However, LLMs have been found to potentially miss nuances in human behavior in psychology experiments, potentially overestimating and giving false positives \cite{cui2024aireplacehumansubjects}. But overall, past work suggests that single LLMs do have a general sense of human behavior in tightly bounded experimental situations. 

Prior research has also used multi-agent LLM systems to replicate human behavior in economic and psychological settings. Prior work has used multi-agent LLM systems to simulate economic games like the Dictator Game, as well as agents' immediate responses to price increases or budget allocations, finding that it is possible to change LLM-agent behavior by giving them different endowments, information, and preferences \cite{horton2023largelanguagemodelssimulated}. Frameworks have also been presented to simulate scenarios such as negotiations, bail hearings, job interviews, and auctions, finding that LLM-agents are able to predict the signs of effects, but not the magnitude \cite{manning2024automated}. However, these studies often lack robust comparisons to human behavior in similar real-world situations. Multi-agent systems have also shown the ability to replicate human strategic behavior in the ultimatum game more accurately than single LLMs, as assessed by comparing simulation results to human experimental data  \cite{sreedhar2024simulatinghumanstrategicbehavior}. However, the ultimatum game is a single economic experiment that has been extensively studied and thus likely appears often in the training data of LLMs, leaving room for further exploration.

% \color{red}Past research suggests that LLMs, and multi-agent LLM systems in particular, have immense potential to replicate human behavior in simulation. Prior research has replicated bounded behaviors in lab experiments with positive results. Prior research has also shown that LLM simulations can demonstrate realistic and emergent human behaviors, BUT HAS NOT TIED TO THE BASELINE SUFFICIENTLY.

% THIS PARA IS WEAK --> BETTER JOB OF SAYING OURS IS DIFFERENT BECAUSE... OBVIOUSLY THERE IS A LOT OF POTENTIAL, THERE"S BEEN SOME PRIOR WORK SHOWING ITS GOOD, BUT WE're EXACTLY FOCUSING ON UNBOUNDED BEHAVIORS THAT NEED MULTI-AGENT SYSTEMS, SO WE REPLICATE EXPERIMENTS BUT THEN GO BEYOND TO UNBOUNDED SCENARIOS WHICH IS NECESSARY FOR POLICY MAKERS. \color{black}

Past research has demonstrated that LLMs, and multi-agent LLM systems in particular, show promise in replicating human behavior in lab experiments where behavior is bounded. However, policymakers require simulations of unbounded scenarios - where people have nearly unlimited choices on ways to think, act, and behave. Our work begins by confirming that multi-agent LLM systems could replicate prosocial behavior in lab experiments, but then extends it into select real-world situations where agents had a more unbounded action space.\color{black}

% The discussed work suggests that LLMs are able to emulate human decision making in fixed scenarios, but do not explore open-ended scenarios that are actually necessary for simulations to provide value in real-world use cases.

% \sout{Overall, past research suggests that LLMs, and multi-agent LLM systems in particular, have immense potential to replicate human behaviors in simulation. This naturally leads to the exploration of multi-agent LLM systems ability to simulate specific types of human behaviors, such as prosocial behavior. BUT it doesn’t study PPG and doesn’t use an architecture that would allow for "unbounded behaviors" that are necessary for policymaking.}

% Prior research has compared results from LLM simulations to experimental data from studies with human subjects, finding that outcomes in LLM simulations generally mirror those from the real world. LLM has been demonstrated to produce results in simulations of social science experiments that strongly correlate with results from both published (85\%) and unpublished (90\%) studies with human subjects \cite{hewitt2024predicting}. LLM has also replicated results from economic and psychology experiments with humans such as the Ultimatum Game, Garden Path Sentences, Milgram Shock Experiment, and Wisdom of Crowds \cite{aher2023usinglargelanguagemodels, sreedhar2024simulatinghumanstrategicbehavior}. However, LLM does potentially miss nuances in human behavior in psychology experiments, potentially overestimating and giving false positives \cite{cui2024aireplacehumansubjects}.

% \color{red}THIS NEEDS TO BE MORE! WILLER STUDY IS SUPER HELPFUL — IF A READER COMES IN THINKING NO WAY AI CAN DO THIS,  THERE PAPER HELPS A TON

% PARAGRAPH ABOUT HORTON, PARAGRAPH ABOUT US, PARAGRAPH ABOUT WILLER

% Prior research in psychology, economics, and AI (non-HCI) have shown that LLMs do have some capacity to replicate human subjects. Using vanilla LLMs (no multi-agent), Kalai showed some consistency (GPS, UG). There was consistency with payoff but no the gender (OR WHATEVER IT WAS). WILLET REPLICATED A WHOLE BATTERY OF CLASSIC PSYCHOLOGY STUFF WITH A SINGLE LLM. This inlcuded zyshbsfdal, published and unpublished paper. This has a strong implication that LLMs have a general sense of human behavior. Unpublished studies being replicated is even greater evidence of that [ but somehow we are better], 

% A few people have also done this w multi-agent. Horton focuses on auction/bail hearing/etc. and show that people can haggle with a cup. But haggling with a cup isn't real, blah blah blah. One paper has looked at human strategic behavior in the Ultimatum Game, showing multi-agents is better than single agents, and GPT4 is better than GPT3.5. So we've reached this threshold of humans doing things thinking about other stuff. But this is just one game with well published results. So we need to extend these studies to see if LLMs can actually replicate broad enough of human psychology that they can be trusted to full simulations of society.

% \color{black}

\subsection{Multi-Agent LLM Systems}

Previously introduced multi-agent systems have varying capacities for allowing unbounded human behavior. Prior research has presented systems for simulating scenarios such as negotiations, bail hearings, job interviews, and auctions. In such systems, the action space is somewhat limited, with the system having rigid turn-taking guidelines and detailed information on how the simulation should proceed \cite{manning2024automated}. Similarly, ChatArena is a system which allows users to simulate turn-taking games: setups for tic-tac-toe, rock-paper-scissors, and chameleon are provided by default, while users can modify input information to simulate games such as the PGG. However, the system is again rigid in the actions agents can take and when agents can take such actions \cite{ChatArena}.

There are also multi-agent LLM systems in which LLM-agents are allowed more complexity and freedom in the ways they can "think" and act: these are referred to as "generative agents" \cite{park2022socialsimulacracreatingpopulated}. MetaAgents is a framework in which agents have four modules: perception, memory, reasoning, and execution. Using a simulated environment of a job fair, the research studies agents' abilities to create teams and workflows for collaborative tasks, finding that agents show promising results in simulation \cite{li2023metaagentssimulatinginteractionshuman}. Architectures have also been presented to simulate the inhabitants of a town. Agents have modules for observation, memory, reflection, planning, and reacting. Multiple locations can also be defined for agents to move between. In simulation, agents are found to demonstrate emergent behaviors, but not compared to observations of human actions explicitly \cite{park2023generativeagentsinteractivesimulacra}.

Past work has also explored coupling large language models with simulation models to better represent human behavior and decision-making \cite{Ghaffarzadegan_2024}, as well as using LLMs to mediate between end-users and simulations \cite{giabbanelli2024broadening}. However, there remains further room for exploration in identifying mechanisms within multi-agent systems themselves to achieve similar goals.

% These systems show more promise in simulating unbounded human behavior, so we focus our work around them. 

% \color{purple} Previous research shows that multi-agent LLM systems can simulate realistic human behavior, but does not rigorously compare the results to actually observed human behavior WHICH WE DO. \color{black}

Whereas previous research shows that multi-agent LLM systems can simulate realistic human behavior, our work goes further showing that multi-agent LLM systems can simulate real observed human behavior in the lab. Additionally, we show that LLMs can simulate observed human behavior outside the lab, where there is an unbounded action space. For example, people can cheat.\color{black}

% In addition, such systems sometimes require added mechanisms to be able to observe specific behaviors. For example, for agents representing students that make a decision to cheat, agents must have a way of doing so without an agent representing an instructor knowing. 

% Recent work has explored coupling large language models with simulation models to better represent human behavior and decision-making \cite{Ghaffarzadegan_2024}, as well as using LLMs to mediate between end-users and simulations \cite{giabbanelli2024broadening}. 

% In contrast, we focus on identifying mechanisms within multi-agent systems themselves to achieve similar goals.

% turn-taking, fixed action spaces
% — chatarena
% — johns stuff

% not turn-taking, unbounded action spaces
% — park
% — ghaffarzedegan
% — limeta2023

% we are interested in using systems of the latter group. these have unbounded action spaces and allow the user to define the environments to varying levels of specificity. we identify specific mechansims that allow for unbounded behavior but put bounds on the environment


 
% \color{red}THIS SHOUDL NOT BE FIRST: Previous research suggests that multi-agent LLM systems especially show promise in simulating human behavior. Multi-agent LLM systems are able to successfully simulate simple games such as tic-tac-toe, rock-paper-scissors, and chameleon \cite{ChatArena}.\color{black} They have also been used as economic agents, being given endowments, information and preferences, and generating reasonable human behavior in scenarios via simulation \cite{horton2023largelanguagemodelssimulated}. Multi-agent LLM systems have also shown promise in simulating human behavior in more open-ended scenarios. Such systems have been used to simulate interactions within social systems \cite{Ghaffarzadegan_2024, li2023metaagentssimulatinginteractionshuman, park2023generativeagentsinteractivesimulacra}, demonstrated to create human-like negotiation strategies \cite{gandhi2023strategicreasoninglanguagemodels} and shown to adhere to human trust behaviors \cite{xie2024largelanguagemodelagents}. They have demonstrated the ability to simulate human-like behavior in a variety of contexts, including supreme court decisions \cite{hamilton2023blindjudgementagentbasedsupreme} as well as bail hearings, job interviews, and auctions (Manning, 2024). Multi-agent LLM systems have also been used to simulate human behavior in larger-scale settings, such as the inhabitants of a town \cite{park2023generativeagentsinteractivesimulacra} and people’s behavior during an epidemic \cite{williams2023epidemicmodelinggenerativeagents}.

% \color{red}THIS FEELS LIKE A LIST... NO MENTION OF MECHANISMS, THOUGHTS FEELINGS BEHAVIORS IN PARK THAT HORTONS/CHATARENA DOESNT. SETUP A SPACE. pARK HAS TAHIS PAPER TAHT GIVE PEOPLE XYZ AND THEY EXHIBITAED BEHAVIORS. LESS ABOUT THEY REPLICATE HUMANS BUT SHOULD BE ABOUT THE TECH. PARK IS NOT TURN-TAKING, CHATARENA IS, ETC. SO THESE SYSTEMS HAVE VARIOUS COMPONENTS ALL TOGETHER. SO PARK IS GOOD CAUSE IT CAN DO UNBOUNDED BUT THERE'S NO LIKE COMPARISON TO REAL WORLD. WE WANT UNBOUNDED ACTION SPACE BUT BOUNDED ENVIRONMENT TO SEE WHAT HAPPENS. WE CHOOSE TO USE THESE UNBOUNDED SYSTEMS BECAUSE THEY GIVE US GOOD ACTIONS, BUT THEN WE HAVE TO FIND THE MECHANISMS THAT DO APPROPRIATELY BOUNDED\color{black}

% Notably, multi-agent LLM systems (that is, systems in which agents have separate context windows and are thus partitioned from each other) have also specifically been demonstrated to outperform single LLMs in simulating human behavior. Previous research has found that multi-agent LLM systems more often replicate human-like outcomes in simulation than single LLMs in economic experiments \cite{sreedhar2024simulatinghumanstrategicbehavior}. Multi-agent LLM systems built with collaborative frameworks are able outperform single LLMs in task accomplishment \cite{chen2023agentversefacilitatingmultiagentcollaboration}.

==> source/3_4_reordered.tex <==
\section{Experimental Setup}

With the goal of better understanding the ability of multi-agent LLM systems to model prosocial human behavior, we simulate three different types of experiments: (1) simulations which aim to directly capture effects observed in a previous lab experiment with human subjects; (2) simulations which combine effects from multiple previous lab experiments with human subjects; and (3) select "in-the-wild" real-world scenarios we use as case studies towards identifying mechanisms necessary for simulations to display human-like behavior. For all experiments, we use OpenAI's GPT4 (model gpt-4o-mini), which has been shown to have the ability to interpret inherently human concepts such as equity and also scores  well on a variety of standardized tests, ranging from the Bar Exam to the GRE \cite{openai2023gpt4}. 

We specifically address the following three research questions:

\bigskip

\begin{itemize}[itemindent=0em]
  \item[\underline{\textbf{RQ1}}] Can multi-agent LLM system simulations replicate behaviors observed in PGG lab experiments with human subjects?
\begin{itemize} [leftmargin=0.15in]
\item[\underline{a.}] Does priming LLM agents via game name replicate the effect of priming humans via game name?
\item[\underline{b.}] Does introducing transparency in contribution between LLM agents replicate the effect of introducing transparency in contribution between humans?
\item[\underline{c.}] Does varying the endowments of LLM agents replicate the effect of varying endowments of humans?
\end{itemize}
\end{itemize}

% \bigskip
% 

% \begin{itemize}[itemindent=2.5em]
%   \item[\underline{\textbf{RQ1}}] \textit{Can multi-agent LLM system simulations replicate behaviors observed in PGG lab experiments with human subjects?} We answer this research question via three experiments comparing results from simulations with LLM-agents to results from lab experiments with human subjects:
  
%   \begin{itemize} [leftmargin=0.5in]
%     \item[\underline{1.}] Priming via Game Name
%     \item[\underline{2.}] Introducing Transparency of Contributions
%     \item[\underline{3.}] Varying Endowments
%   \end{itemize}
% \end{itemize}

% \color{black}

\bigskip

\begin{itemize}[itemindent=0em]

  \item[\underline{\textbf{RQ2}}] Can multi-agent LLM system simulations transfer effects observed in non-PGG lab experiments to simulations of the PGG?
\begin{itemize}[leftmargin=0.15in]
    % \item[\underline{a.}] Does priming LLM agents with sentences known to increase/decrease generosity in humans have that effect in simulations of the PGG?
    \item[\underline{a.}] Does priming LLM agents with a methodology used in non-PGG cooperation game lab experiments have the expected result in LLM simulations of the PGG?
    % \color{red}Priming methodology\color{black}
% \item[\underline{b.}] Does the effect of priming LLM agents via game name in multi-round PGGs fade over time, like priming has been observed to fade over time in other experiments with human subjects?\color{red}priming over time\color{black}
\item[\underline{b.}] Does the effect of priming over time, observed to fade in non-PGG competition game lab experiments, hold in LLM simulations of the PGG?
\end{itemize}
\end{itemize}

  \bigskip
% 
% \begin{itemize}[itemindent=2.5em]

%   \item[\underline{\textbf{RQ2.}}] \textit{Can multi-agent LLM system simulations replicate human behavior extrapolated from combining the behaviors observed in multiple lab experiments with human subjects?} We answer this research question via two experiments combining treatments and expected effects from multiple lab experiments with human subjects:
%   \begin{itemize}[leftmargin=0.5in]
%     \item[\underline{1.}] Using a priming methodology from other cooperation games in the PGG
%     \item[\underline{2.}] Measuring the change in effect of priming over time, using results of priming over time from a different competition game
%   \end{itemize}
% \end{itemize}
% \color{black}

% \bigskip

\begin{itemize}[itemindent=0em]
  \item[\underline{\textbf{RQ3}}] To what extent are multi-agent LLMs complex enough to simulate the rich set
of unbounded options, actions, and interactions people do in the real world, outside of the lab?
\begin{itemize}[leftmargin=0.15in]
    % \item[\underline{a.}] Does priming LLM agents with sentences known to increase/decrease generosity in humans have that effect in simulations of the PGG?
    \item[\underline{a.}] To see the complex
interactions observed in the real world, what simulation mechanisms do we have to add to the set up of the system?
    % \color{red}Priming methodology\color{black}
% \item[\underline{b.}] Does the effect of priming LLM agents via game name in multi-round PGGs fade over time, like priming has been observed to fade over time in other experiments with human subjects?\color{red}priming over time\color{black}
\end{itemize}
\end{itemize}

% \bigskip

% 

% \begin{itemize}
%   \item[\underline{\textbf{RQ3.}}] \textit{What are required mechanisms for simulations to
% inform policy-makers regarding real-world situations to test policies that encourage human collaboration?} We answer this research question via three real-world case studies towards identifying necessary mechanisms:
% \begin{itemize}[leftmargin=0.5in]
%     \item[\underline{1.}] A classroom setting with varying late-assignment policies
%     \item[\underline{2.}] A store parking lot where shoppers need to return shopping carts to designated areas
%     \item[\underline{3.}] Graffitti?
%   \end{itemize}
% \end{itemize}

% \color{black}

\bigskip

We expect generally positive results for the first two research questions, given that other work has shown the ability of LLMs to replicate lab experiments that are both published and unpublished \cite{hewitt2024predicting}, but still verify this in the context of the PGG towards understanding the abilities of multi-agent LLM systems to simulate prosocial behavior. The third research question is more open-ended - we use case studies of real-world scenarios towards identifying mechanisms required for simulations to show expected outcomes, a process which can be continued to be used by policy makers. As policy makers consider the specific scenarios which they need to simulate, they may realize and implement new mechanisms required to enable their simulation. However, we also expect that mechanisms will be generalizable to an extent across simulations of various situations.


\subsection{Multi-Agent Architecture}
For all studies, we adapted a previously introduced and open-source multi-agent system for simulating social emergent behavior \cite{GPTeam}. The system is implemented in Python and uses gpt-4o-mini. The input to the system is a JSON file describing the \textit{locations} and \textit{agents} in the simulation. The output is a series of logs for \textit{events} (things done by agents and witnessed by other agents). The input files and system we use for the simulations in our studies are publicly available \cite{prosocialGPTeam}.

The system architecture consists of a class structure defined as follows. At the highest level, the simulation is represented by a \textit{world} class consisting of 3 sub-classes: \textit{locations}, \textit{events}, and \textit{agents}. 

 Locations represent places that agents can go within the world.  Locations are specified by a name, description, and agents allowed within them. Agents can only talk to other agents or witness events in the same location as them. Events are created when agents take action, whether that be moving or speaking.  Events are specified by a timestamp, the agent that acted, the location it occurred, a description, and witnesses.

Agents are separate LLM instances that are used to represent "people" in the environment.  Agents are specified by a name, a private biography, a public biography and an initial plan. The private biography is information about the agent only known to the agent. The public biography is information about the agent that other agents also are aware of. The initial plan instructs the agent on what to do when the simulation starts. It is specified by a location (i.e., where it occurs), a description of what the agent should do, and a stop condition that specifies when the agent should stop executing on the plan. The initial plan is private - it is only known to the agent. 

Agents have subclasses \textit{plans} – specified by a description, location, and stop condition – and \textit{memories} – specified by a description, creation time, and importance score. Plans are created by agents as they witness events in simulation. All plans are specified in the same format as the initial plan. Memories are created each time an agent witnesses an event. When a memory is created, an importance score is also created simply by asking an LLM to generate one. When agents act, they first identify memories that are relevant and use them to maintain or adjust their current plan before executing on their action. 

% Agents are specified by a name, biographies, an initial plan (with a location, description, and stop condition) that are unique (and other than the public biography) and only known to them.   

Simulations can be run once the user specifies the locations and agents in the input file. The system executes simulation via \textit{agent loops}, which involve (1) agents \textit{observing} the events in their current location, (2) agents adding events to memory, (3) agents creating \textit{plans}, (4) agents \textit{reacting} as to whether or not to continue the current plan, (5) and agents \textit{acting}, carrying out plans. Agents \textit{speak} to communicate with one another.  The agent loop is what enables emergent behavior - agents are able to "reason" about their surroundings and events and then decide on new courses of actions. This type of architecture has been shown to be more accurate in replicating human behavior in social science/economics games than just prompting a single LLM \cite{sreedhar2024simulatinghumanstrategicbehavior}.

When implementing the PGG in this environment, we create 4-5 agents: 3-4 players, and one moderator. The private biography is used to provide agents with their unique priming or endowment that other agents should not know. There are typically two locations;  a game room where players are by default, and a contribution room where players make their contribution. Players are aware of the existence of these locations and can move between them. In every agent loop, the agent waits for the player before them to come back from the contribution room, then goes to the contribution room, tells the moderator their contribution, the moderator records it to his memory, and the player agent leaves. When all the players are done, the moderator comes out and announces the game outcome. 

\color{black}

\section{Study 1: Replicating Lab Experiments of PGG}

% The first study aims to answer the following research question:

% \begin{itemize}[itemindent=0em]
%   \item[\underline{\textbf{RQ1}}] Can multi-agent LLM system simulations replicate behaviors observed in PGG lab experiments with human subjects?
% \begin{itemize} [leftmargin=0.25in]
% \item[\underline{a.}] Does priming LLM agents via game name replicate the effect of priming humans via game name?
% \item[\underline{b.}] Does introducing transparency in contribution between LLM agents replicate the effect of introducing transparency in contribution between humans?
% \item[\underline{c.}] Does varying the endowments of LLM agents replicate the effect of varying endowments of humans?
% \end{itemize}
% \end{itemize}

% \subsection{LLM-Agent Simulation Setup for the Public Goods Game}

% \subsubsection{PGG Simulation Setup} \sout{There are three main necessary components for simulating the PGG: (1) agents, (2) locations, and (3) game play instructions.} \sout{To setup the PGG simulation, we intialize \color{black} two types of people: one moderator and multiple players (typically 3-4). These are all represented by separate LLM-agents.
% The simulation requires two locations: (1) a moderation room where players tell the moderator their contribution in private and (2) a game room where players wait their turn to talk to the moderator and the moderator delivers the result of the game. Players know these locations exist and that they can move between them. There are also game play instructions that are given to all agents so they know what to do: the players know their endowment, that they will take turns telling the moderator their contribution in the moderation room, and that they will receive an announcement of the results in the game room. For variants of the game testing different treatments, additional instructions and player information is added.}


% % The game requires four to five agents: three to four player agents and one moderator agent. We  two rooms: the game room and the moderation room. 

% % We need four to five agents (three players and one moderator), rooms (2 rooms, the game room and moderation room), and (3)initialization instructions (agents are told their role and ).

% % WAIT FOR THEIR TURN. players are given an initial endowment. for all of these experiments, there is only one round. they will take turns making contributions. and then the moderator will announce the outcomes to the group.

% % there are separate additional instructions for each variant of the game. 

% \subsubsection{Multi-Agent LLM Architecture Implementation} \sout{We implement the simulation by adapting a previously introduced agent architecture for simulating social emergent behavior \cite{GPTeam}. In this architecture, the person running simulations provides each agent with a name, public and private biographies, instructions, and an initial plan, which consists of a description, stop condition, and a location. The architecture also allows for the creation of locations (specified by a name and description) between which agents can move, but does not have an explicit turn-taking process.}\sout{The architecture used does not have an excplicit turn-taking process. \color{black} Instead, turn-taking can be implemented by ordering the player agents and telling every player to see to the moderator after the player ordered immediately ahead of them.}

% % Communication between agents  the architecture is not inherently turn-taking - we specify the order of contributions via agents instructions and initial plan.




% When implementing the PGG in the multi-agent framework, we initialize it as follows. The moderator agent's name is "Moderator," and its public biography is simple: "This agent plays the role of the moderator". The moderator agent has no private biography. The moderator has an initial plan to start in the moderation room and wait for all players to make their contribution, and has instructions to then move to the game room and announce payoffs once all agents have made their contribution.

% The player agents are given arbitrary alphabetical names (Alice, Bob, Casey, and David) and each have public biographies with a statement that the agent is playing a PGG-like game and contains their initial endowment, which all other agents can see. The player agents' private biography is blank by default, but is used to realize the priming condition of experiments  - for example, the name priming is realized by adding to the agents private biography, "You are playing a game called the \textit{Taxation Game}." \color{black} 

% The architecture used does not have an explicit turn-taking process. \color{black} To implement the mechanics of turn-taking, player agents' have an initial plan to wait for the player before them to return from the moderation room. Player agents are ordered alphabetically by being told the player before them (in the case of Bob, Casey, and David) or by being told they are first (in the case of Alice). They also have instructions to move to the moderation room and make their contribution (with the payoff specified here for player agents to take into account) once the player before them has returned, and to not engage with any other player agents' in the game room until the Moderator comes to the room and payoffs are announced. In each \textit{agent loop}, the agent thus waits for the player before them to come back from the contribution room before going themselves, tells the moderator their contribution (which the moderator records to their memory), then returns to the main room.\color{black}

% % the Generative Agents Structure does not have a mechanism for turn-taking, thus

% % In the initial plan description, 
% % players initial location is the game room. 
% % The Generative Agents Structure does not have a mechanism for turn-taking, thus we implement this is the initial description: every player must wait for the player before them to return from the Moderator room (where they take their turn TELLING THE CONTRIBUTION).
% % The 

% % player agents are told to wait for the player that comes before them to return to the game room. The stop condition of the initial plan is when the player before returns to the game room from making a contribu The location of the initial plan is specified as the game room. In the directives, player agents are instructed to move to the moderation room and make their contribution once the initial plan stop condition is hit.



% % Initial Plan (for Bob)
% % description: wait for ALICE to return from the game room (for the first one it's slightly different)
% % location: game room
% % stop condition: ALICE  has returned from the game room

% % Instruction: once alice is back, move into the moderation room to make your contribution
% % Instruction: after making the contribution come back
% % Instruction: in the game room, do not engage with any other players until the moderator returns and announces payoffs

% % In the simulation setup for the PGG within this architecture, there is an agent named and directed to act as the moderator. The remaining agents (varies from three to four depending upon the experiment) are given arbitrary alphabetical names (Alice, Bob, Casey, and David). Each agent's initial endowment is specified in their public biography, which all other agents can see. If there is a priming condition, it is included in the private biography as to expose the desired agent to the priming without leakage to other agents. Communication is not inherently turn-taking in the architecture; so we have to specify the order and method of contribution to player agents via their directives and initial plan. We initialize two separate rooms - the game room and the moderation room. Player agents are by default in the game room, then travel to the moderation room to tell the moderator their contribution once the player specified as being before them returns to game room from the moderation room after making their contribution. The moderator remains in the moderation room other than to announce payoffs after all players have made contributions. To realize transparency, we simply remove the moderation room, and have all agents make their contributions publicly in the game room. 


% \subsubsection{Data Collection} As the simulation progresses, all of the thoughts and actions of each player agent (and the moderator agent) are displayed in separate output logs, each representing one of the agents involved in the simulation. Each output log contains a plethora of information, ranging from the events each agents observed, their reactions to them, and the creation of new plans, but we are only interested in the contributions they make.

%  To collect data on the contribution amount of each agent, we used a script on each player agent's output logs. The script used string matching and regular expressions to look for when each agent was in the moderation room and the dollar amount said by the agent. This data was then output into a table. A human verified that the data was accurately transcribed by reading the sections identified by the script and making corrections as needed.


\subsection{Methodology}

To test whether LLMs can replicate lab experiments, we pick three lab experiments with human subjects. We create simulations for them, run it, and compare results to human behavior. These three studies focus on three different effects: (1) priming via game, (2) transparency of contributions, and (3) variation in endowment. They found the following:

\subsubsection{Experiment \#1} \label{oneofone} The first experiment studies the effect of positive and negative priming on contributions in the PGG. We obtain data on human behavior from a 2014 lab experiment in \textit{Judgement and Decision Making} \cite{Eriksson_Strimling_2014} with 100 human participants. Participants were explained the rules of the game, but told one of two different names for the game. \color{black} In the positive condition, people were told the game was called the "Teamwork Game." In the negative case, people were told the game was called the "Taxation Game." The remaining conditions were the same. In the positive priming condition ("Teamwork"), people on average contributed 60\% of their endowment. In the negative priming condition ("Taxation"), people on average contributed only 40\% of their endowment. \textbf{Thus, positive priming increases prosocial behavior.}

% \sout{People were put into one of two conditions.} 
% \sout{\cite{Eriksson_Strimling_2014}}

We test whether this effect applies to LLM-agents by simulating ten one-shot PGGs with four players, two under each priming condition and all four with a \$20 endowment, and comparing the average contribution amount of players from either group. Specifically, we prime players by including sentences containing the appropriate name in their private biographies (for example, "Alice is playing a game called the "Teamwork Game."). In the simulation, 1.6 times the amount of the public pool is split evenly amongst the players as their payoff - players are made aware of this to inform the way in which they act, but the simulation is of a one-shot PGG.

\subsubsection{Experiment \#2} The second experiment studies the effect of transparency of contributions in the PGG. We obtain data on human behavior from a 2017 review paper of 71 human lab studies published in \textit{Experimental Economics} \cite{transparencytwo}. \color{black} Specifically, the difference in contribution is presented for people who played the PGG in two conditions: one where people knew the contributions made by others and another where they did not. When there was transparency of contributions, people contributed 6\% more on average than when there was not. \textbf{Thus, transparency of contributions increases prosocial behavior.}

%\sout{\cite{transparencytwo}}

% \sout{It collects data from a variety of prior studies with and without transparency.}

We test whether this effect applies to LLM-agents by simulating ten four-player one-shot PGGs, five with transparency of contributions and five without, and comparing the average contribution amounts in either condition. Specifically, we realize transparency by removing the moderation room - contributions are made in the "public" game room where all other agents can overhear other's contributions. In the simulation, 1.6 times the amount of the public pool is split evenly amongst the players as their payoff - players are made aware of this to inform the way in which they act, but the simulation is of a one-shot PGG.

\subsubsection{Experiment \#3} The third experiment studies the effect of unequal endowments on contributions in the PGG.  We obtain data on human behavior from a 2016 lab experiment published in \textit{Economics Letters} \cite{HARGREAVESHEAP20164}. \color{black}The experiment included four separate PGG games with different endowment conditions: (1) where all players had \$20, (2) where all players had \$50, (3) where all players had \$80, and (4) where one player had \$20, one player had \$50, and one player had \$80. The results of the experiment find that people endowed with \$20 and \$50 contributed roughly the same in both games were all players had the same endowment and games where endowments were varied, but that people endowed with \$80 contributed much more in games were all players had the same endowment than games in which endowments were varied.
%\sout{\cite{HARGREAVESHEAP20164}}. 
\textbf{Thus, varying endowments does not seem to have an effect on prosocial behavior in "poor" and "medium" wealth individuals, but reduces prosocial behavior in "rich" individuals.}

We test whether this effect applies to LLM-agents by simulating twenty-five three-player one-shot PGGs, fifteen where players have equal endowments (five for \$20, \$50, and \$80 respectively) and ten where players have varied endowments (one player with \$20, one with \$50, and one with \$80), then comparing the average contribution of players with each endowment amount under the equal and varied endowment conditions. Specifically, we realize the variation in endowments simply by changing the players public biographies, where their endowments are set. In the simulation, 1.6 times the amount of the public pool is split evenly amongst the players as their payoff - players are made aware of this to inform the way in which they act, but the simulation is of a one-shot PGG.


\subsection{LLM-Agent Simulation Setup for the Public Goods Game}

% \subsubsection{PGG Simulation Setup} \sout{There are three main necessary components for simulating the PGG: (1) agents, (2) locations, and (3) game play instructions.} \sout{To setup the PGG simulation, we intialize \color{black} two types of people: one moderator and multiple players (typically 3-4). These are all represented by separate LLM-agents.
% The simulation requires two locations: (1) a moderation room where players tell the moderator their contribution in private and (2) a game room where players wait their turn to talk to the moderator and the moderator delivers the result of the game. Players know these locations exist and that they can move between them. There are also game play instructions that are given to all agents so they know what to do: the players know their endowment, that they will take turns telling the moderator their contribution in the moderation room, and that they will receive an announcement of the results in the game room. For variants of the game testing different treatments, additional instructions and player information is added.}


% The game requires four to five agents: three to four player agents and one moderator agent. We  two rooms: the game room and the moderation room. 

% We need four to five agents (three players and one moderator), rooms (2 rooms, the game room and moderation room), and (3)initialization instructions (agents are told their role and ).

% WAIT FOR THEIR TURN. players are given an initial endowment. for all of these experiments, there is only one round. they will take turns making contributions. and then the moderator will announce the outcomes to the group.

% there are separate additional instructions for each variant of the game. 

\subsubsection{Multi-Agent LLM Architecture Implementation} 
% \sout{We implement the simulation by adapting a previously introduced agent architecture for simulating social emergent behavior \cite{GPTeam}. In this architecture, the person running simulations provides each agent with a name, public and private biographies, instructions, and an initial plan, which consists of a description, stop condition, and a location. The architecture also allows for the creation of locations (specified by a name and description) between which agents can move, but does not have an explicit turn-taking process.}\sout{The architecture used does not have an excplicit turn-taking process. \color{black} Instead, turn-taking can be implemented by ordering the player agents and telling every player to see to the moderator after the player ordered immediately ahead of them.}

% Communication between agents  the architecture is not inherently turn-taking - we specify the order of contributions via agents instructions and initial plan.




When implementing the PGG in the multi-agent framework, we initialize it as follows. The moderator agent's name is "Moderator," and its public biography is simple: "This agent plays the role of the moderator". The moderator agent has no private biography. The moderator has an initial plan to start in the moderation room and wait for all players to make their contribution, and has instructions to then move to the game room and announce payoffs once all agents have made their contribution.

The player agents are given arbitrary alphabetical names (Alice, Bob, Casey, and David) and each have public biographies with a statement that the agent is playing a PGG-like game and contains their initial endowment, which all other agents can see. The player agents' private biography is blank by default, but is used to realize the priming condition of experiments  - for example, the name priming is realized by adding to the agents private biography, "You are playing a game called the \textit{Taxation Game}." \color{black} 

The architecture used does not have an explicit turn-taking process. \color{black} To implement the mechanics of turn-taking, player agents' have an initial plan to wait for the player before them to return from the moderation room. Player agents are ordered alphabetically by being told the player before them (in the case of Bob, Casey, and David) or by being told they are first (in the case of Alice). They also have instructions to move to the moderation room and make their contribution (with the payoff specified here for player agents to take into account) once the player before them has returned, and to not engage with any other player agents' in the game room until the Moderator comes to the room and payoffs are announced. In each \textit{agent loop}, the agent thus waits for the player before them to come back from the contribution room before going themselves, tells the moderator their contribution (which the moderator records to their memory), then returns to the main room.\color{black}

% the Generative Agents Structure does not have a mechanism for turn-taking, thus

% In the initial plan description, 
% players initial location is the game room. 
% The Generative Agents Structure does not have a mechanism for turn-taking, thus we implement this is the initial description: every player must wait for the player before them to return from the Moderator room (where they take their turn TELLING THE CONTRIBUTION).
% The 

% player agents are told to wait for the player that comes before them to return to the game room. The stop condition of the initial plan is when the player before returns to the game room from making a contribu The location of the initial plan is specified as the game room. In the directives, player agents are instructed to move to the moderation room and make their contribution once the initial plan stop condition is hit.



% Initial Plan (for Bob)
% description: wait for ALICE to return from the game room (for the first one it's slightly different)
% location: game room
% stop condition: ALICE  has returned from the game room

% Instruction: once alice is back, move into the moderation room to make your contribution
% Instruction: after making the contribution come back
% Instruction: in the game room, do not engage with any other players until the moderator returns and announces payoffs

% In the simulation setup for the PGG within this architecture, there is an agent named and directed to act as the moderator. The remaining agents (varies from three to four depending upon the experiment) are given arbitrary alphabetical names (Alice, Bob, Casey, and David). Each agent's initial endowment is specified in their public biography, which all other agents can see. If there is a priming condition, it is included in the private biography as to expose the desired agent to the priming without leakage to other agents. Communication is not inherently turn-taking in the architecture; so we have to specify the order and method of contribution to player agents via their directives and initial plan. We initialize two separate rooms - the game room and the moderation room. Player agents are by default in the game room, then travel to the moderation room to tell the moderator their contribution once the player specified as being before them returns to game room from the moderation room after making their contribution. The moderator remains in the moderation room other than to announce payoffs after all players have made contributions. To realize transparency, we simply remove the moderation room, and have all agents make their contributions publicly in the game room. 


\subsubsection{Data Collection} As the simulation progresses, all of the thoughts and actions of each player agent (and the moderator agent) are displayed in separate output logs, each representing one of the agents involved in the simulation. Each output log contains a plethora of information, ranging from the events each agents observed, their reactions to them, and the creation of new plans, but we are only interested in the contributions they make.

 To collect data on the contribution amount of each agent, we used a script on each player agent's output logs. The script used string matching and regular expressions to look for when each agent was in the moderation room and the dollar amount said by the agent. This data was then output into a table. A human verified that the data was accurately transcribed by reading the sections identified by the script and making corrections as needed.

%To test what happens in simulation,  / we implement this (from the paragraph below)

% \color{black}

% For experiments of the first type, we run simulations of the PGG using treatments from published lab experiments with human subjects, checking whether the effect of said treatments on LLM-agents in simulation in similar to that of on humans. The treatments and effects we replicate from previous lab experiments are listed in Table ~\ref{labexperiments}.

% \begin{center}
% \begin{table}[H]
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{10pt}
% \begin{tabular}{|>{\columncolor{gray!20}\centering\arraybackslash}m{0.5cm}|p{6cm}|p{6cm}|} 
%  \hline
%  \rowcolor{gray!20} \textbf{Exp.} & \multicolumn{1}{c|}{\textbf{Treatment}} & \multicolumn{1}{c|}{\textbf{Expected Result}} \\ [0.5ex] 
%  \hline\hline
%  \textbf{1} & \textbf{Priming via Game Name:} Participants are presented the PGG as a game called either the "Taxation Game" or "Teamwork Game." & Participants presented the game as the "Taxation Game" contribute less than participants presented the "Teamwork Game." \cite{Eriksson_Strimling_2014} \\ 
%  \hline
%  \textbf{2} & \textbf{Transparency of Contribution:} Participants know what others contribute to the public pool (under standard conditions, contributions are made privately with respect to other players). & Participants make larger contributions when participants are aware of each other's contributions compared to when contributions are made privately without other's knowledge. \cite{transparencytwo}\\
%  \hline
%  \textbf{3} & \textbf{Variations in Endowment:} Participants start the PGG with different endowment amounts. & "Rich" participants contribute more when other participants are also "rich." \cite{HARGREAVESHEAP20164}  \\
%  \hline
% \end{tabular}
% \caption{\label{labexperiments}Table of treatments and expected results (effects) from previous lab experiments of the PGG with human subjects. Actual experiments that are drawn from are cited in the second column.}
% \end{table}
% \end{center}

% For these experiments, we simulate one-shot PGGs with three or four players, measuring whether the impact the treatments have on player contributions is similar to what has been observed in experiments with human subjects (i.e., the expected result listed). For the first experiment, we run ten simulations of the PGG with four players, two under each priming condition, and compare the average contribution amount of players from either group. For the second experiment, we also run ten simulations of the PGG with four players: five simulations with transparency of contributions and five without. We compare the average contribution amount of players in either of the two conditions. In the first and second experiments, players are all endowed with \$20. For the third experiment, we run twenty simulations with three players: fifteen simulations where all players have the same initial endowment (five where that endowment is \$20, five where it is \$50, and five where it is \$80) and five simulations where players have different initial endowments (namely, \$20, \$50, and \$80). We compare the average contributions of players with each of the three endowments in the fixed and the varied endowment conditions (i.e., we compare how much a player with \$X contributes in the condition where everyone has \$X vs. the varied condition). In all three experiments, 1.6 times the amount of the public pool is split evenly amongst the players as their payoff - players are made aware of this to inform the way in which they act, but the simulations are of one-shot PGGs.

\subsection{Results}

% Towards answering this question, we simulate treatments from three different lab experiments with human subjects: (1) priming via game name, (2) transparency of contributions, and (3) variations in endowment. In the first two experiments, LLM-agents replicate the direction of effects with statistical significance, but overestimate the magnitude. In the third experiment, LLM-agents replicate the direction of effects but the effect is not statistically significant, although this is likely due to insufficient data for comparison. \textbf{Overall, we conclude that LLM-agents are able to replicate the direction of the effect of priming and transparency treatments, \color{orange}but testing their ability to replicate the effect of a varied endowment requires further simulations.\color{black}}

\subsubsection{Does priming LLM agents via game name replicate the effect of priming humans via game name?}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{images/1A.png}
    \caption{Average contributions for "Teamwork" and "Taxation" priming conditions in simulations with LLM-agents and experiments with human subjects. Average contributions are above 60\% in the "Teamwork" priming condition for both groups. Average contributions are below 40\% in the "Taxation" priming condition for both groups.}
    \Description{A bar chart titled "Average Contribution by Priming" compares the average contributions in two priming conditions: "Teamwork" and "Taxation." The y-axis represents average contributions as a percentage of endowment, ranging from 0 to 100\%. The x-axis lists the two priming conditions. Each condition has two bars: a gray bar representing LLM-agents and a blue bar representing human participants. In the "Teamwork" condition, both groups contribute above 60\%, with LLM-agents contributing slightly more than humans. In the "Taxation" condition, contributions are below 40\% for both groups, with humans contributing slightly more than LLM-agents.}
    \label{1Agraph}
\end{figure}

% \sout{A t-test shows that the difference in contributions between the two groups is statistically significant at the p < 0.01 level  
% (\(t = 7.92, p < 0.00000001 \)). However, t-tests also show that there are statistically significant differences between the contributions made LLM-agents and the average human contribution under the "Teamwork" priming condition (\(t = 3.59, p = 0.002 \)) at the p < 0.01 level and the "Taxation" priming condition (\(t = -2.34, p < 0.031 \)) at the p < 0.05 level. \textbf{From these results, we conclude that priming LLM agents by presenting the PGG under different names replicates the direction of the effect of doing the same on humans, but may overestimate the magnitude.}}

A t-test shows that the difference in LLM contributions between the two groups is statistically significant at the p < 0.01 level  
(\(t = 7.92, p < 0.00000001 \)). We use one-sample one-tail t-tests to compare the LLM-simulation sample data with the human average contribution, finding that under the "Teamwork" priming condition, the LLM contributions are greater than the human average of 60\% (\(t = 3.59, p = 0.001 \)) at the p < 0.01 level. Under the "Taxation" priming condition, LLM contributions are less than the human average of 40\% (\(t = -2.33, p = 0.016 \)) at the p < 0.05 level. \textbf{From these results, we conclude that priming LLM agents by presenting the PGG under different names replicates the direction of the effect of doing the same on humans, but may overestimate the magnitude.}\color{black} 

\subsubsection{Does introducing transparency in contribution between LLM agents replicate the effect of introducing transparency in contribution between humans?}

In experiments with human subjects, participants contributed on average 6\% more of their endowment under transparency conditions as compared to no transparency. \cite{transparencytwo}. Across five simulations of each condition (ten simulations total) on average, LLM agents playing the PGG with transparency contributed approximately 60\% of their \$20 endowment, whereas LLM agents playing the PGG without transparency contributed only approximately 35\% of their endowment. These results are in Figure \ref{1Bgraph}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{images/1B.png}
    \caption{Average contributions with and without transparency of contributions for simulations. Experiments with humans show that average contributions in PGGs with transparency of contributions is 6\% higher than in PGGs without without transparency. In simulations with LLM-agents, average contributions in PGGs with transparency of contributions were 25\% higher than in PGGs without transparency. So, the direction of the difference is accurately captured.}
    \Description{A bar chart titled "Average Contribution by Transparency" compares the average contributions in two transparency conditions: "Without Transparency" and "With Transparency." The y-axis represents average contributions as a percentage of endowment, ranging from 0 to 100\%. The x-axis lists the two transparency conditions. The bar for "Without Transparency" is lower (35\%), indicating a lower contribution percentage, while the bar for "With Transparency" is noticeably higher (60\%). This suggests that contributions increase when transparency of contributions is present.}
    \label{1Bgraph}
\end{figure}

% \sout{A t-test shows that the difference in contributions between the two groups is statistically significant at the p < 0.05 level  
% (\(t = 2.23, p = 0.031 \)).} 
A one-tailed t-test shows that the mean contribution of LLMs under the transparency condition is significantly greater than the mean contribution of LLMs under the non-transparent condition (\(t = 2.23, p = 0.016 \)) at the p < 0.05 level. \color{black} \textbf{From these results, we conclude that introducing transparency of contributions in PGGs with LLM agents replicates the direction of the effect of doing the same on humans.}

% "If controlling for the MPCR, however, as is done in specifications (6) and (8), the positive effect of F.indichoice and the negative effect of F.indipayoffs have a larger magnitude and turn significant at the 5% level. The share contributed tends to be about 6 percentage points higher than in cases where players receive feedback about the distribution of choices in their group."


\subsubsection{Does varying the endowments of LLM agents replicate the effect of varying endowments of humans?}

In experiments with human subjects, it was found "poor" and "medium" wealth individuals contributed roughly the same amount in equal and varied endowment conditions, whereas "rich" individuals contributed more in the equal endowment condition than in the varied endowment condition \cite{HARGREAVESHEAP20164}. Across five simulations each of \$20-\$20-\$20, \$50-\$50-\$50, and \$80-\$80-\$80 equal endowment conditions, LLM agents on average contributed approximately 39\%, 48\%, and 63\% of their endowments, respectively. In five simulations of a \$20-\$50-\$80 varied endowment condition, on average the LLM agent given \$20 contributed approximately 35\%; the LLM agent given \$50 contributed approximately 42\%; and the LLM agent given \$80 contribute approximately 44\%. Thus, the contribution for agents endowed with \$20 was roughly the same between the equal and varied endowment conditions, whereas agents endowed with \$50 and \$80 both contributed less in the varied condition.These results are summarized in Table \ref{1Cgraph}.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.75\textwidth]{images/1C.png}  % Change this value to make the figure larger
%     \caption{Average contributions for equal and varied endowment conditions in simulations with LLM-agents and experiments with human subjects. Average contributions are roughly the same for humans and LLM-agents in the equal and varied endowment conditions with \$20 and \$50 endowments. Average contributions are lower in the varied condition than in the fixed condition with \$80 endowments for both humans and LLM-agents.}
%     \label{1Cgraph}
% \end{figure}

\begin{figure*}[t]  % Use figure* for spanning both columns
    \centering
    \includegraphics[width=\textwidth]{images/1C.png}  % Adjust width to span across the page
    \caption{Average contributions for equal and varied endowment conditions in simulations with LLM-agents and experiments with human subjects. Average contributions are roughly the same for humans and LLM-agents in the equal and varied endowment conditions with \$20 and \$50 endowments. Average contributions are lower in the varied condition than in the fixed condition with \$80 endowments for both humans and LLM-agents.}
    \Description{A bar chart titled "Average Contribution by Endowment" compares contributions as a percentage of endowment across different endowment amounts (\$20, \$50, and \$80) for humans and LLM-agents. The x-axis represents the endowment amounts and groups participants into "Human" and "LLM-Agents" under each endowment level. The y-axis represents the average contribution as a percentage of endowment, ranging from 0 to 100\%. Each group has two bars: a dark gray bar for "Equal Endowments" and a light blue bar for "Varied Endowments." Contributions generally increase with higher endowments, with variations between humans and LLM-agents. The impact of equal vs. varied endowments is also visible across conditions.}
    \label{1Cgraph}
\end{figure*}

% \begin{table}[htbp]
% \centering
% \begin{tabular}{|>{\columncolor{gray!20}}c|c|c|c|}
% \hline
% \rowcolor{gray!20}\multicolumn{1}{|c|}{} & \multicolumn{3}{c|}{\textbf{Initial Endowment}} \\ \hline
% \rowcolor{gray!20}\textbf{Condition} & \$20 & \$50 & \$80 \\ \hline
% Equal & 39\% & 48\% & 63\% \\ \hline
% Varied & 35\% & 42\% & 44\% \\ \hline
% p-value & 0.86 & 0.58 & 0.23 \\ \hline
% t-stat & 0.18 & -0.56 & 1.25 \\ \hline
% \end{tabular}
% \caption{\color{red}IK THIS TABLE MAKES NO SENSE\color{black}}
% \label{variedend}
% \end{table}

T-tests shows that there is no statistically significant difference at the p < 0.1 between the contributions of LLM agents endowed with \$20 in the equal and varied endowment condition (\(t = -9.42, p = 0.678 \)), nor for the \$50 (\(t = -0.56, p = 0.58 \)) endowment - both results mirroring those of human subjects. However, a t-test shows that the difference between the contributions of LLM agents endowed with \$80 is statistically significant at the p < 0.1 level (\(t = -1.94, p = 0.065 \)). A one-tailed t-test specifically shows that the contribution of LLM-agents endowed with \$80 is significantly greater in the equal condition than in the varied condition (\(t = 2.05, p = 0.026 \)) at the p < 0.05 level. \color{black} \textbf{From these results, we conclude that varying endowments in the PGG with LLM agents replicates the effect of doing the same on humans.}

% \color{orange}
% % From these results, we cannot fully conclude that LLM agents are affected by varying endowments in the same way as humans. However, the lack of difference between the average contribution in the equal and varied condition with endowments of \$20 and \$50 along with the difference between the averages in the equal and varied endowment conditions does suggest that varying endowments does have an impact similar to the effect observed in humans. The lack of statistical significance could be a result of the limited and unequal number of data points in both groups of comparison (for every endowment amount, there are 15 contributions in the equal endowment condition compared  to only 5 contributions in the varied endowment condition in our simulations).

% % REDO THIS AS - COMPARE THE HUMAN EQUAL WITH LLM EQUAL, COMPARE THE HUMAN VARIED WITH LLM VARIED
% \color{black}

\section{Study 2: Testing Multi-Agent Systems Ability to Transfer Effects from non-PGG Lab Experiments to Simulations of the PGG}

% \color{red}We choose papers still in experimental psychology/economics, but NOT THE WORD PGG. This is about if we use different key words, does it still work. NEED TO DO REWRITE RQ2 to reflect this.\color{black}

% The second study aims to answer the following research question:


% \begin{itemize}[itemindent=0em]

%   \item[\underline{\textbf{RQ2.}}] Can multi-agent LLM system simulations transfer effects observed in non-PGG lab experiments to simulations of the PGG?
%   \begin{itemize}
%     \item[\underline{a.}] Does priming LLM agents with sentences known to increase/decrease generosity in humans have that effect in simulations of the PGG?
% \item[\underline{b.}] Does the effect of priming LLM agents via game name in multi-round PGGs fade over time, like priming has been observed to fade over time in other experiments with human subjects?
% \end{itemize}
% \end{itemize}

% \begin{itemize}[itemindent=0em]

%   \item[\underline{\textbf{RQ2}}] Can multi-agent LLM system simulations transfer effects observed in non-PGG lab experiments to simulations of the PGG?
% \begin{itemize}[leftmargin=0.25in]
%     % \item[\underline{a.}] Does priming LLM agents with sentences known to increase/decrease generosity in humans have that effect in simulations of the PGG?
%     \item[\underline{a.}] Does priming LLM agents with a methodology used in non-PGG cooperation game lab experiments have the expected result in LLM simulations of the PGG?
%     % \color{red}Priming methodology\color{black}
% % \item[\underline{b.}] Does the effect of priming LLM agents via game name in multi-round PGGs fade over time, like priming has been observed to fade over time in other experiments with human subjects?\color{red}priming over time\color{black}
% \item[\underline{b.}] Does the effect of priming over time, observed to fade in non-PGG competition game lab experiments, hold in LLM simulations of the PGG?
% \end{itemize}
% \end{itemize}

To test whether LLMs can actually simulate human-like behavior and are not just parroting previously published lab experiments, we design two further experiments. These experiments take effects from lab experiments not containing the key word "public goods game." We then measure if LLMs are able to produce the expected outcomes in simulations of the PGG. We run two experiments; the first applies positive and negative priming methods used in other cooperation games, to assess if LLMs can generalize these effects to the PGG. The second tests priming effects from a one-shot PGG lab experiment, but over multiple rounds, incorporating the observed changes in priming effects over time from competition games. This approach confirms that the results in Study 1 were not simply due to LLMs parroting the results from a single lab experiment - it demonstrates that LLMs can integrate information from multiple various sources to simulate human-like behavior. 

% \begin{itemize}
%     \item[1.]
% \end{itemize}

% \color{red}TO REWRITE BIG PICTURE IS BREAK UP THE FIRST AND LAST SENTENCES, MAYBE BULLET POINTS FOR THE MIDDLE ONE: Particularly, studies on other games show that the effects of priming fade over time. MA-LLM simulations of multi-round PGG simulartions, also show priming effects diminishing over tiem, which is consistent with expected behavior, but not explicitly shown in any study of the PGG.  USE THIS TO REWRITE THIS: To test whether LLMs can actually simulate human-like behavior in simulation and are not just parroting previously published single papers, we design two further experiments which take effects from lab experiments not containing the key word "public goods game" and measure whether LLMs are able to produce the expected outcomes in simulations of the PGG. We run two experiments: (1) tests the effects of positive and negative priming, but with a priming methodology used in lab experiments of other cooperation games and (2) tests the effects of a positive and negative priming used in a lab experiment of the one-shot PGG, but over multiple rounds by using an observed change in priming effect over time from lab experiments with a competition game. By doing so, we confirm that the results in Study 1 were not merely due to LLMs parroting the lab experiment from which the effects were derived from and demonstrate that LLMs are able to obtain information from multiple sources to simulate expected human-like behavior.\color{black}

\color{purple}

% \subsection{LLM-Agent Simulation Setup for COMBINATIONS}

% The setup for these experiments is nearly identical to that of Study 1 - simulating the PGG still requires: (1) people, (2) rooms, and (3) game play instructions. The simulation still involves two types of people: one moderator and multiple players (specifically, 4). The simulation requires the same two rooms: (1) a moderation room and (2) a game room. Players are given the same instructions as in Study 1 for the first experiment; the second involves multiple rounds, so players are given slightly modified instructions to repeat their actions multiple times.

% The implementation of these experiments is also very similar to that of Study 1. We use the same architecture as in Study 1. The moderator agent is defined the same as in Study 1 for experiment 1; for experiment 2, the moderator agent has an additional instruction to continue the instructions to listen to contributions and announce payoffs for multiple rounds. Player agents are defined the same as in Study 1 for experiment 1 as well; for experiment 2, player agents are similarly given an additional instruction to make multiple contributions over multiple rounds of the PGG.

% We collect data via the outputs of the architecture in the same process as Study 1. The thoughts and actions of each player agent (and the moderator agent) are displayed in separate output logs, from which we extract the information necessary for our results. 

\color{black}

\subsection{Methodology}

% To test whether LLMs can \color{red} CAN ACTUALLY SIM ULATE HUMAN BEHAVIOR AND IS NOT JUST PARROTING PAPERS DIRECTLY\color{black}\sout{replicate the effects from combining lab experiments, we design two experiments which combine the effects from two lab experiments and check if results are reasonably representative of the combined effect. }\color{red}WE DO THIS TO TEST WHETHER THE PREVIOUS EXPERIMENTS WERE JUST GPT PARROTING SINGLE PAPERS. THIS IS A PROBLEM, SO WE WANT TO TAKE IT A STEP FURTHER AND SEE IF THE RESULTS STILL STAND IF YOU'RE NOT JUST LIFTING IT FROM A PAPER. SO WE DO THIS THING: (1) SAME BASIC TEST, BUT WITH DIFFERENT KEY WORDS and (2) KEY WORD SURE AND DIMENSION/GAMEPLAYSETUP/SOMETHING, .... THIS IS A GOOD THING\color{black}The two experiments test the following: (1) using a priming methodology used in lab experiments in other cooperation games and checking if it affects LLM-agent contributions as expected and (2) measuring the impact of the game name priming over time, using results from an experiment of a multi-round competition game with primed participants.

% We design two experiments based on a combination of treatments and effects from multiple lab experiments with human subjects. The first takes a priming methodology and effect from experiments with human subjects of different cooperative games than the PGG to see if the effect holds for the PGG. The second uses a priming methodology used on the one-shot PGG and measures if it has the same effect over multiple rounds similar to the way in which priming affects competition economic games. The treatments and effects in the combined experiments we design are listed in Table ~\ref{combinedexperiments}.

% \begin{center}
% \begin{table}[H]
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{10pt}
% \begin{tabular}{|>{\columncolor{gray!20}\centering\arraybackslash}m{0.5cm}|p{6cm}|p{6cm}|} 
%  \hline
%  \rowcolor{gray!20} \textbf{Exp.} & \multicolumn{1}{c|}{\textbf{Treatment}} & \multicolumn{1}{c|}{\textbf{Expected Result}} \\ [0.5ex] 
%  \hline\hline
%  \textbf{1} & \textbf{Priming via Sentences:} Participants are presented with 5 sentences alluding to either "unity" or "proportionality" concepts. & Participants presented with sentences alluding to "unity" should contribute more than participants primed with "proportionality". \cite{6d947858-4a17-3462-9053-fc55b58ffee1, moralsmatter} \\ 
%  \hline
%  \textbf{2} & \textbf{Priming via Game Name over Multiple Rounds:} Participants are presented the PGG as a game called either the "Taxation Game" or "Teamwork Game" and play for five rounds. & The effect of priming should fade over time; although there should still be a disparity between participants in either group's initial contributions, it should lessen over time. \cite{Eriksson_Strimling_2014, JIMENEZJIMENEZ201594} \\
%  \hline
% \end{tabular}
% \caption{\label{combinedexperiments}Table of treatments and expected results (effects) from combining previous lab experiments with human subjects. Actual experiments that are drawn from are cited in the second column.}
% \end{table}
% \end{center}

\subsubsection{Experiment \#1} The first experiment uses a priming methodology used in a 2013 lab experiment of a modified solidarity game with 75 participants published in \textit{Plos One} \cite{moralsmatter}. The solidarity game is another cooperative economics game, but the priming methodology used \color{black} has not been tested on the PGG in prior lab experiments to our knowledge. Positive priming has shown to induce generosity in the PGG and other cooperative games, so we test whether LLMs are able to replicate the effects of a positive priming methodology used in a non-PGG lab experiment in simulations of the PGG. The positive priming involves showing participants three sentences alluding to "unity" ('\textit{we are family},' '\textit{mine is also yours},' and '\textit{caring for each other}'), while the negative priming involves showing participants three sentences alluding to "proportionality" ('\textit{how are you useful for me},' '\textit{I want to profit},' and '\textit{making a deal}'). The results of the lab experiment find that people in the positive priming condition displayed more generosity than people in the negative priming condition in the solidarity game. Thus, the positive priming increased prosocial behavior, meaning that it should increase contributions in the PGG as well.

% \subsubsection{Experiment \#1} The first experiment uses a priming methodology used for other \color{red} X OTHER GAMES, SUCH AS BLANK, BUT NOT THE PGG. TO OUR KNOWLEDGE, NOBODY HAS DONE THIS FOR THE PGG. Positive priming has been shown to work for the PGG and other games. Here we are testing if we can replicate the effect of a positive priming \color{black}contribution games: a positive priming which involves showing participants three sentences alluding to "unity" ('\textit{we are family},' '\textit{mine is also yours},' and '\textit{caring for each other}') and a negative priming which involves showing participants three sentences alluding to "proportionality" ('\textit{how are you useful for me},' '\textit{I want to profit},' and '\textit{making a deal}'). The results of the lab experiment find that people in the positive priming condition displayed more generosity than people in the negative priming condition in the solidarity game. \textbf{Thus, the positive priming increased prosocial behavior.}

We test whether this effect applies to LLM agents by simulating ten one-shot PGGs with four players, two under each priming condition, and all four with a \$20 endowment, and comparing the average contribution amount of players from either group. Specifically, we prime players by adding the three sentences to the player's private biography as something they have read (for example: "Alice read the following sentences prior to playing the game: '\textit{we are family},' '\textit{mine is also yours},' and '\textit{caring for each other}.'"). In the simulation, 1.6 times the amount of the public pool is split evenly amongst the players as their payoff - players are made aware of this to inform the way in which they act, but the simulation is of a one-shot PGGs.

\subsubsection{Experiment \# 2} The second experiment measures the effect of positive and negative priming over time (multiple rounds). Prior lab experiments of the one-shot PGG have shown that positive priming (by presenting the game as the "Teamwork Game") increases contributions while negative priming (by presenting the game as the "Taxation Game") decreases contributions \cite{Eriksson_Strimling_2014}\color{black}. Meanwhile, prior lab experiments of multi-round Bertrand competition games show that the effect of primings fades over time \cite{JIMENEZJIMENEZ201594}\color{black}. By combining these results, we expect that positive/negative priming should respectively increase/decrease the average contribution in the first round of the PPG, but should trend closer to half over multiple rounds. 

%Thus, we combine these results to expect that positive and negative priming should increase and decrease the average contribution in the first round of the PGG. However, contributions should trend closer to half of the endowment (the expected contribution without priming) over multiple rounds.

\color{black}

% \subsubsection{Experiment \#2} The second experiment measures the effect of priming over time. Results of a lab experiment of a competition game show that players take actions less influenced by various primings they are subject to in later rounds of the competition game than in the first round. \textbf{Thus, the effect of priming fades over time.}

% \color{red}PEOPLE HAVEN'T TRIED PRIMING WITH THE PGG OVER MULTIPLE ROUNDS (make sure this is true). SO WE TEST, DOES THE RESULT OF PRIMING FADING OVER TIME WHICH COMES FROM OTAHER EXPERIMENTS ALSO HOLD FOR THE PGG\color{black}

We test whether this effect applies to LLM-agents by simulating ten five-round PGGs with four players, two subject to a positive priming (the "Teamwork" priming discussed in Study 1, Experiment \#1) and two subject to a negative priming (the "Taxation" priming discussed in Study 1, Experiment \#1). We compare the average contribution in the first round for either priming condition with the average contribution in the last round for either priming condition. We also compare the initial contributions between priming conditions, checking that there was an initial disparity that ultimately begins to fade. In this experiment, payoffs are computed the same as in previous experiments (namely, 1.6 times the amount of the public pool split evenly amongst the players). Since there are multiple rounds, the payoff and amount not contributed are summed to determine each players endowment for the next round.

\subsection{Results}

% Towards answering this question, we simulate two experiments designed as a combination of multiple lab experiments with human subjects: \color{red}(1) takes a priming methodology and effect from experiments with human subjects of different cooperative games than the PGG to see if the effect holds for the PGG, and (2) uses a priming methodology used on the one-shot PGG and measures if it has the same effect over multiple rounds similar to the way in which priming affects different economic games than the PGG. \color{black} \textbf{From the results of these experiments, we conclude that multi-agent LLM system simulations do replicate behavior extrapolated from combining the behaviors observed in multiple lab experiments with human subjects.}

\subsubsection{Does priming LLM agents with a methodology used in non-PGG cooperation game lab experiments have the expected result in LLM simulations of the PGG?}

In experiments of other cooperation games, priming participants via sentences alluding to "unity" resulted in participants being more generous than participants primed via sentences alluding to "proportionality" \cite{moralsmatter}. In ten simulations, LLM agents primed with the sentences alluding to "unity" (Alice and Bob) contributed on average approximately 65\% of their initial endowment. In comparison, agents primed with the sentences alluding to "proportionality" (Casey and David) contributed on average only approximately 30\% of their endowment to the public pool. The results are summarized in Figure \ref{2Agraph}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{images/2A.png}
    \caption{Average contributions for either "unity" or "proportionality" priming conditions. Average contributions under the "unity" condition are significantly higher than that under the "proportionality" condition.}
    \Description{A bar chart titled "Average Contribution by Priming" compares average contributions under two priming conditions: "Unity" and "Proportionality." The y-axis represents average contributions as a percentage of endowment, ranging from 0 to 100\%. The x-axis lists the two priming conditions. The bar for "Unity" is significantly higher, showing contributions above 60\%, while the bar for "Proportionality" is much lower, below 40\%. This indicates that priming with a "Unity" condition leads to higher contributions compared to the "Proportionality" condition.}
    \label{2Agraph}
\end{figure}

% \color{red}FROM THESE RESULTS, THE PSYCHOLOGICAL MECHANISM DOES TRANSFER ACROSS PAPERS\color{black}

A t-test shows that the difference in contributions between the two groups is statistically significant at the p < 0.01 level (\(t = 8.76, p < 1\text{e}{-9} \)). \textbf{From these results, we conclude that the effects of priming on humans is transferred from papers not involving the PGG to simulations of the PGG with LLM-agents.}

% A t-test shows that the difference in contributions between the two groups is statistically significant at the p < 0.01 level (\(t = 8.76, p < 1\text{e}{-9} \)). \textbf{From these results, we conclude that priming LLM agents with sentences known to increase (or decrease) generosity in humans does result in higher (or lower) contributions in simulations of the PGG with LLM-agents.}

\subsubsection{Does the effect of priming over time, observed to fade in non-PGG competition game lab experiments, hold in LLM simulations of the PGG?}
\bigskip
In experiments of competition games with human subjects, the effect of priming has been found to fade over time \cite{JIMENEZJIMENEZ201594}. In ten simulations, LLM agents presented a five-round PGG as the "Teamwork Game" (Alice and Bob) on average contributed 75\% of their initial endowment in the first round, compared to 55\% of their initial endowment in the fifth round. In comparison, agents presented the PGG as the "Taxation Game" (Casey and David) contributed 30\% of their initial endowment in the first round, compared to 45\% of their initial endowment in the fifth round. Hence, for both priming conditions, the average contribution was closer to 50\% of the initial endowment in the fifth round than in the first, meaning the effect of the priming was less pronounced in the fifth round than the first. The results are summarized in Figure \ref{2Bgraph}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{images/2B.png}
    \caption{Average contributions in the all five rounds rounds for either "Teamwork" and "Taxation" priming conditions. Average contributions in the fifth round are closer to 50\% of the initial endowment, the average amount contributed without any priming \cite{labexperiments}. Hence, the effects of priming appears to fade over time in simulations with LLM-agents.}
    \Description{A line chart titled "Average Contribution by Priming and Round" shows how average contributions change over five rounds under two priming conditions: "Teamwork" and "Taxation." The y-axis represents average contributions as a percentage of the initial endowment, ranging from 0 to 100\%. The x-axis represents the round numbers (Round #1 to Round #5). The blue line represents contributions under the "Teamwork" priming condition, which starts high and gradually decreases over time. The black line represents contributions under the "Taxation" priming condition, which starts lower but increases slightly across rounds. By Round #5, contributions in both conditions converge closer to 50\%, suggesting that the effects of priming diminish over time in simulations with LLM-agents.}
    \label{2Bgraph}
\end{figure}

% \color{red}{FROM THESE RESULTS, SOMETHING TRANSFERS.... GPT DID NOT JUST PARROT A PAPER USING KEY WORDS. SOMEHOW IT WAS ABLE TO TRANSFER. SO GPT CAN TELL US MORE THAN WHAT PAPERS ALREADY KNOW}\color{black}

T-tests show that the difference in contribution amount between the rounds is statistically significant for the "Teamwork" priming condition at the p < 0.01 level (\(t = 4.32, p = 0.002 \)) and for the "Taxation" priming condition at the p < 0.05 level (\(t = -2.30, p = 0.047 \)). A t-test also shows that there is a statistically significant difference in the first round contributions of players in either priming condition (\(t = 9.64, p < 0.0000000001 \)). \textbf{From these results, we observe that the effect of priming LLM agents fades over time, concluding that LLMs are not just parroting past literature, but are able to transfer the multi-round effect observed in non-PGG lab experiments to simulations of the PGG.} The "Taxation" priming condition specifically suggests that the difference between first and fifth round contributions is not because contributions in PGGs with human subjects decrease over time \cite{labexperiments}, but rather that it is likely the consequence of a fading priming effect.

% T-tests show that the difference in contribution amount between the rounds is statistically significant for the "Teamwork" priming condition at the p < 0.01 level (\(t = 4.32, p = 0.002 \)) and for the "Taxation" priming condition at the p < 0.05 level (\(t = -2.30, p = 0.047 \)). A t-test also shows that there is a statistically significant difference in the first round contributions of players in either priming condition (\color{red}IN NEW YORK I MILLY ROCK\color{black}). \textbf{From these results, we conclude that the effect of priming LLM agents fades over time, as observed in experiments with human subjects.} The "Taxation" priming condition specifically suggests that the difference between first and fifth round contributions is not because contributions in PGGs with human subjects decrease over time \cite{labexperiments}, but rather likely the consequence of a fading priming effect.

\section{Study 3: Simulating "In-the-Wild" Scenarios}

% The third study aims to answer the following research question:

% \begin{itemize}[itemindent=0em]
%   \item[\underline{\textbf{RQ3}}] To what extent are multi-agent LLMs complex enough to simulate the rich set
% of unbounded options, actions, and interactions people do in the real world, outside of the lab?
% \begin{itemize}[leftmargin=0.25in]
%     % \item[\underline{a.}] Does priming LLM agents with sentences known to increase/decrease generosity in humans have that effect in simulations of the PGG?
%     \item[\underline{a.}] To see the complex
% interactions observed in the real world, what simulation mechanisms do we have to add to the set up of the system?
%     % \color{red}Priming methodology\color{black}
% % \item[\underline{b.}] Does the effect of priming LLM agents via game name in multi-round PGGs fade over time, like priming has been observed to fade over time in other experiments with human subjects?\color{red}priming over time\color{black}
% \end{itemize}
% \end{itemize}

This study aims to test whether LLM-agents can demonstrate realistic prosocial-related behavior in "in-the-wild" real-world situations. Real-world situations require a greater level of complexity in setup than lab experiments, as individuals do not have as explicit of instructions on when and how to act or speak. Furthermore, there is a lack of specific papers for LLMs to draw from to simulate human behavior in such open-ended settings. We test two specific real-world situations: (1) a classroom setting and (2) a grocery store parking lot setting. In a classroom, we have anecdotal evidence from university faculty that changing the harshness of late policies or adding perturbations to student lives have an effect on student behaviors. Specifically, we test whether the emergent behavior of cheating, a "bad" form of cooperation, occurs in simulation. In leaving a grocery store parking lot, shoppers may be affected by other factors in their lives that change how they act \cite{scientificamerican2020shoppingcarts}. Specifically, we test whether the emergent behavior of returning their shopping cart, a form of prosocial behavior, occurs in simulation. We test if we can see these emergent behaviors in a basic simulation setup, finding that in both scenarios our basic setup is insufficient to observe the desired behaviors. Hence, we add a mechanism in each to increase the complexity of the setup that guides LLM simulations to produce results closer to expected human behavior.

% \color{red}These are bad prosocial behaviors... add these sentences throughout\color{black}

% \color{red}REORDER THIS TO BE SCENARIO 1 - ALL INFORMATION, SCENARIO 2 - ALL INFORMATION\color{black}

% \color{red}THE GOAL OF STUDY 3 IS TO ..... SEE IF LLM-AGENTS DEMONSTRATE PLAUSIBLE BEHAVIOR IN REAL-WORLD SITUATIONS. We know simulations require a level of complexity in setup. We want to see if these things happen in basic simulation in response to harsh policies. And then if they don't, we want to figure out the mechanism that makes it happen. Classrooms are an environment that have policies like a late policy. It's hard to figure out what goes on. THere haven't been studies, but people anecdotally told us....  \color{black}

% \color{red} One of the problems is that we don't know how much setup is necessary to get the behaviors. BASIC IMPLEMENTATION: NO ROOMS. MORE COMPLICATED IMPLEMENTATION: THERE ARE THE ROOMS\color{black}

% We do this via simulating two \color{red} OR MAYBE THREE THREE \color{black} "in-the-wild" scenarios that are seen in the real world: a classroom \color{red}\sout{and} \color{black} a shopping-cart return setting, \color{red} and MAYBE a graffitti.\color{purple}


\subsection{Classroom Setting}

\subsubsection{Setup}

\paragraph{Classroom Simulation Setup}

Towards simulating the behaviors in a classroom setting, we first try basic simulation setup with only one location, but find that expected student behaviors (specifically, cheating) are not present. Hence, we add a mechanism to the simulation setup - locations for private communication - to enable students to communicate with one another without the teacher overhearing and discuss the things that real students may discuss in private.

To simulate the classroom setting, we identify two main necessary components for the basic setup: (1) people, (2) a location, and (3) homework assignment and submission instructions. The simulation involves two types of people: one professor and multiple students (specifically, 3). These are all represented by separate LLM-agents, all located in the same location. Students are given various personality traits (over-achiever, procrastinator, or values work-life-balance) and can be affected by two perturbations (having a midterm or a particularly challenging assignment). The professor is instructed to announce the late-policy and make assignment announcements at a regular interval. Students are instructed to listen to assignment announcements at the interval at which the professor announces them, and to "work" on the assignments in the meantime. Students are able to converse with the professor and other students, although only by addressing all at the same time.

For the more complicated setup, we introduce using locations as a mechanism for private communication. The simulation requires three locations: (1) a classroom, where assignments are announced, (2) an office, where the professor goes while students "work", and (3) a work room, where students "work." All students know these locations exist; the students can move between all of them, while the professor only moves between the classroom and office. The professor is instructed to announce the late-policy and make assignment announcements at a regular interval in the classroom, and to remain in the office otherwise. Students are instructed to listen to assignment announcements in the classroom at the interval at which the professor announces them, and then to be in the work room otherwise, with the option to move to the office to talk to or ask the professor questions.

% There are three main necessary components for simulating the classroom setting: (1) people, (2) rooms, and (3) homework assignment and submission instructions. The simulation involves two types of people: one professor and multiple students (specifically, 3). These are all represented by separate LLM-agents. The simulation requires three rooms: (1) a classroom, where assignments are announced, (2) an office, where the professor goes while students "work", and (3) a work room, where students "work." All agents know these rooms exist; the students can move between all of them, while the professor only moves between the classroom and office. Students are given various personality traits (over-achiever, procrastinator, or values work-life-balance) and can be affected by two perturbations (having a midterm or a particularly challenging assignment). The professor is instructed to announce the late-policy and make assignment announcements at a regular interval in the classroom, and to remain in the office otherwise. Students are instructed to listen to assignment announcements in the classroom at the interval at which the professor announces them, and then to be in the work room otherwise, with the option to move to the office to talk to or ask the professor questions.

\paragraph{Multi-Agent LLM Architecture Implementation}

We implement the simulation by adapting the same architecture as in the previous studies. When implementing the classroom setting in the multi-agent framework, we initialize it accordingly. In both setups, the professor agent's name is "Professor." The professor agent's public biography contains their late policy for assignments, as well as a general sentence indicating that they are the instructor for the course. The professor agent has no private biography. In the basic setup, the professor has an initial plan to announce their late policy and the first assignment's due date. The professor agent has instructions to answer student questions and to announce additional assignments at regular intervals (five total). The student agents are given arbitrary alphabetical names (Alice, Bob, and Casey). The student agents' public biographies contain their personality types, whereas their private biographies contain the perturbations as needed. Student agents are given an initial plan to listen to the late policy and first assignment announcement. Student agents have instructions to: (1) "work" on assignments, (2) listen to the professor's announcements of new assignments, and (3) state how many days late they will need to submit each assignment.

After adding separate office, work, and class rooms, we modify the instructions to each agent to utilize the ability to move between them appropriately. The professor agent has an initial plan to start in the classroom and announce their late policy and the first assignment's due date, then to move to the office. The professor agent has instructions to (1) answer student questions in the office, (2) move to the classroom at regular intervals to announce additional assignments, and (3) never enter the work room. Student agents are given an initial plan to listen to the late policy and first assignment announcement in the classroom. Student agents have instructions to: (1) work on assignments in the work room, (2) return to the classroom at regular intervals to hear announcements for new assignments, (3) state how many days late they will submit each assignment, and (4) use the office to talk to or ask questions to the professor. 

% The professor agent has an initial plan to start in the classroom and announce their late policy and the first assignment's due date, then to move to the office. The professor agent has instructions to answer student questions in the office, and to move to the classroom at regular intervals to announce additional assignments (five total). The student agents are given arbitrary alphabetical names (Alice, Bob, and Casey). The student agents' public biographies contain their personality types, whereas their private biographies contain the perturbations as needed. Student agents are given an initial plan to listen to the late policy and first assignment announcement in the classroom. Student agents have instructions to: (1) work on assignments in the work room, (2) return to the classroom at regular intervals to hear new assignments, (3) state how many days late they will need to submit each assignment, and (4) use the office to talk to or ask questions to the professor. 

\paragraph{Data Collection} As the simulation progresses, all of the thoughts and actions of each student agent (and the
professor agent) are displayed in separate output logs, each representing one of the agents involved in the simulation.
Each output log contains a plethora of information, ranging from the events each agents observed, their reactions to
them, and the creation of new plans, but we are only interested in tracking the specific behavior of cheating, which occurs by LLM-agents requesting to see and/or copy other's work. To collect data on the presence of this behaviors, we manually read through each student agent's output logs. A human manually recorded whether or not cheating was suggested and formatted this information into a table.

\subsubsection{Methodology}

We run simulations with three different late policies: (1) a lenient late policy (LLP) in which assignments turned in late are not given any penalty, (2) a medium late policy (MLP) in which assignments are docked 10\% for each late day, and (3) a harsh late policy (HLP) in which late assignments are not accepted. We also run simulations under three different perturbation conditions: (1) where students do not have any perturbations (P0), (2) where students have a midterm during the third assignment period (P1), and (3) where students have a midterm during the third assignment period and the second assignment is especially challenging (P2). We ran five simulations of each of the nine combinations of late policy and perturbation conditions (LLP-P0, LLP-P1, LLP-P2, MLP-P0, MLP-P1, MLP-P2, HLP-P0, HLP-P1, and HLP-P2) under two conditions: with or without locations. In each simulation, we recorded if any student proposed cheating at any point.

\subsubsection{Results}

In simulations with only one room, we found that students never suggested cheating, likely due to the professor always being in the same room as them. However, the introduction of locations changed this. In the lenient late policy condition, students still never suggested cheating, regardless of perturbations. In the medium late policy, students never suggested cheating in the no perturbation condition, but did so in one simulation in each of the one perturbation and two perturbation conditions. In the harsh late policy, students suggested cheating in all three perturbation conditions: students suggested cheating at an equal frequency in the no perturbation and one perturbation conditions, and the most in the two perturbation condition. The results are presented in Figure ~\ref{3Agraph}. \textbf{From these results, we conclude that locations can be used a mechanism for private communication to observe emergent behaviors such as cheating (a "bad" form of cooperation), which can only occur if students are able to converse without the professor overhearing.}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.75\textwidth]{images/3A.png}  % Change this value to make the figure larger
%     \caption{Percentage of simulations in which cheating was observed under the 9 late policy and perturbation conditions, for simulations with and without multiple locations. Without multiple locations, cheating is never observed. With multiple locations, cheating first begins to be observed under the medium late policy under the one perturbation condition. The number of simulations in which cheating occurs is the same for the medium late policy in the two perturbation condition, as well as for the harsh late policy under the no perturbation and one perturbation conditions. The number of simulations in which cheating occurs is greatest with the harsh late policy under the two perturbation condition.}
%     \label{3Agraph}
% \end{figure}

\begin{figure*}[t]  % Use figure* for spanning across both columns
    \centering
    \includegraphics[width=\textwidth]{images/3A.png}  % Scale the figure to the full page width
    \caption{Percentage of simulations in which cheating was observed under the 9 late policy and perturbation conditions, for simulations with and without multiple locations. Without multiple locations, cheating is never observed. With multiple locations, cheating first begins to be observed under the medium late policy under the one perturbation condition. The number of simulations in which cheating occurs is the same for the medium late policy in the two perturbation condition, as well as for the harsh late policy under the no perturbation and one perturbation conditions. The number of simulations in which cheating occurs is greatest with the harsh late policy under the two perturbation condition.}
    \Description{A bar chart titled "\% of Simulations with Cheating by Classroom Conditions and With or Without Rooms" illustrates the percentage of simulations in which cheating was observed under different classroom conditions. The y-axis represents the percentage of simulations with cheating, ranging from 0\% to 70\%. The x-axis represents three classroom conditions: LLP (Low Late Policy), MLP (Medium Late Policy), and HLP (Harsh Late Policy), each divided into three perturbation conditions (P0, P1, P2). Two sets of bars are shown for each condition: dark gray for "Without Rooms" and light gray for "With Rooms." Results indicate that cheating is not observed under LLP regardless of perturbation conditions. Under MLP, cheating emerges in P1 and P2, with slightly higher occurrences when multiple locations (rooms) are present. Under HLP, cheating is observed across all perturbation conditions and increases sharply in P2, particularly when multiple locations are involved, reaching the highest cheating percentage in the entire dataset.}
    \label{3Agraph}
\end{figure*}



\subsection{Shopping-Cart Return Setting}

\subsubsection{Setup}

\paragraph{Shopping-Cart Return Simulation Setup}

There are three main necessary components for simulating the shopping-cart return setting: (1) people, (2) locations, and (3) instructions on what to act on. The simulation involves one person, a shopper, who is preparing to leave the parking lot and represented by a LLM-agent. The simulation requires two locations: (1) the area where the shopper has parked, and (2) the receptacle, where carts \textit{should} be returned. The shopper agent knows these locations exist, and can decide whether or not to move between them. The shopper agent can be affected by conditions that affect their ability to return their cart (being far from the receptacle or having a child with them) \cite{scientificamerican2020shoppingcarts}. The shopper is told to prepare to leave the parking lot and instructed that they cannot leave with their shopping cart - the shopper hence must decide \textit{something} to do with their shopping cart.

\paragraph{Multi-Agent LLM Architecture Implementation} We implement the simulation by adapting the same architecture as in the previous studies. When implementing the shopping-cart return setting in the multi-agent framework, we initialize it accordingly. The shopper agent is given the name "Shopper." The shopper agent has a blank public biography. The shopper agent's private biography states that they have a cart, and conditions that affect their ability to return their cart. The shopper agent has an initial plan to prepare to leave the parking lot, then instructions to act on the outcomes of their initial plan. We create two locations: (1) which represents the area where the shopper has parked and (2) the designated shopping-cart return receptacle. This way, we capture that LLM-agents must move in order to return their shopping cart.

However, we find that simply stating the condition affecting the shopper's ability to return their cart ("you are far from the receptacle," and "you have a child") is insufficient to have the desired effect of shoppers returning their carts less frequently; the prompt must allude towards what is at stake ("you are \textit{parked across the parking lot} from the receptacle," and "you have a \textit{five-month old} child"). In the condition where shoppers are far from the receptacle, adding that shoppers are "\textit{parked across the parking lot}" alludes to the fact that going to receptacle will take effort, whereas adding that the child is an infant alludes to the fact that the child cannot be left unattended. We present this as stake-prompting (SP), a mechanism to have prompts allude to what is at stake, using which LLM-agents can be guided towards demonstrating more human-like behavior in simulation.

\paragraph{Data Collection} As the simulation progresses, all of the thoughts and actions of the shopper agent are displayed in an output log. The output log contains a plethora of information, ranging from the events the agent observed (which is minimal in this simulation), their reactions to them (similarly minimal), and the creation of new plans. But we are only interested in recording whether or not the shopper agent returns their cart, based on whether the shopper agent moves to the receptacle location. A human manually recorded this information and formatted it into a table.

\subsubsection{Methodology} We run simulations with two different conditions that shoppers can be affected by: (1) being far from the receptacle (FFR) and (2) having a child (HAC). We run five simulations each of either condition under with and without stake-prompting. Given that the condition affecting the shopper should influence them to not return their shopping cart, we track whether or not the shopping cart is returned in each simulation and then compare the frequency of returns between simulations with and without stake-prompting.

\subsubsection{Results} In simulations without stake-prompting, we find that shopper agents still frequently return their carts despite the conditions affecting their ability to do so. However, alluding to what is at stake as a result of the condition  causes shopper agents to stop returning their carts as often. The results are summarized in Figure \ref{3Bgraph}. \textbf{From these results, we conclude that alluding to what is at stake via stake-prompting causes LLM-agents to demonstrate less prosocial behavior when affected by personal conditions, like humans.}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{images/3B.png}
    \caption{Percentage of simulations in which the shopper agent decided to their shopping cart for both external conditions tested and under either prompting condition: with or without stake-prompting. LLM-Agents returned their cart less frequently with stake-prompting than without.}
    \Description{ bar chart titled "Effect of Stake-Prompting on Cart Return by Condition" illustrates the percentage of simulations in which a shopper agent returned their shopping cart under two conditions: FPR and HAC. The y-axis represents the percentage of simulations where the cart was returned, ranging from 0\% to 100\%. The x-axis lists the two conditions. Each condition has two bars: a gray bar for the "Without SP" (stake-prompting) condition and a yellow bar for the "With SP" condition. Results show that cart return rates are higher when no stake-prompting is applied, with significantly lower return percentages when stake-prompting is present. This pattern is consistent across both conditions, suggesting that LLM-agents return their carts less frequently when stake-prompting is introduced.}
    \label{3Bgraph}
\end{figure}

% \subsubsection{Methodology}

% \subsubsection{Classroom}

% We run simulations with three different late policies: (1) a lenient late policy (LLP) in which assignments turned in late are not given any penalty, (2) a medium late policy (MLP) in which assignments are docked 10\% for each late day, and (3) a harsh late policy (HLP) in which late assignments are not accepted. We also run simulations under three different perturbation conditions: (1) where students do not have any perturbations (P0), (2) where students have a midterm during the third assignment period (P1), and (3) where students have a midterm during the third assignment period and the second assignment is especially challenging (P2). We ran five simulations of each of the nine combinations of late policy and perturbation conditions (LLP-P0, LLP-P1, LLP-P2, MLP-P0, MLP-P1, MLP-P2, HLP-P0, HLP-P1, and HLP-P2) under two conditions: with or without locations. In each simulation, we recorded if any student proposed cheating at any point.

% \subsubsection{Shopping-Cart} We run simulations with two different conditions that shoppers can be affected by: (1) being far from the receptacle (FFR) and (2) having a child (HAC). We run five simulations each of either condition under with and without stake-prompting. Given that the condition affecting the shopper should influence them to not return their shopping cart, we track whether or not the shopping cart is returned in each simulation and then compare the frequency of returns between simulations with and without stake-prompting.

% five simulations of shopper agents for each condition and with or without \color{red}stake-prompting\color{black}, resulting in twenty simulations total.



% \subsubsection{g}

% \subsection{Results}

% \subsubsection{Classroom}

% In simulations with only one room, we found that students never suggested cheating, likely due to the professor always being in the same room as them. However, the introduction of locations changed this. In the lenient late policy condition, students still never suggested cheating, regardless of perturbations. In the medium late policy, students never suggested cheating in the no perturbation condition, but did so in one simulation in each of the one perturbation and two perturbation conditions. In the harsh late policy, students suggested cheating in all three perturbation conditions: students suggested cheating at an equal frequency in the no perturbation and one perturbation conditions, and the most in the two perturbation condition. The results are presented in Figure ~\ref{3Agraph}. \textbf{From these results, we conclude that locations can be used a mechanism for private communication to observe emergent behaviors such as cheating, which can only occur if students are able to converse without the professor overhearing.}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.75\textwidth]{images/3A.png}  % Change this value to make the figure larger
%     \caption{Percentage of simulations in which cheating was observed under the 9 late policy and perturbation conditions, for simulations with and without multiple locations. Without multiple locations, cheating is never observed. With multiple locations, cheating first begins to be observed under the medium late policy under the one perturbation condition. The number of simulations in which cheating occurs is the same for the medium late policy in the two perturbation condition, as well as for the harsh late policy under the no perturbation and one perturbation conditions. The number of simulations in which cheating occurs is greatest with the harsh late policy under the two perturbation condition.}
%     \label{3Agraph}
% \end{figure}

% However, we find that in this simulation setup, behaviors that students would display with one another without the professor's presence are not present in simulation. In addition, having all questions directed to the professor being overheard by all students distracts students to which the information is not relevant to.

% \color{red}Anecdotally, we also saw behaviors where students proposed simple collaboration (working together) and students communicated with the professor\color{black}

% \color{red}In preliminary simulations with one room, we found that students did not suggest cheating, likely due to the professor being in the same room as them. We thus introduced rooms and recorded results. The results of the number of simulations in which students (1) proposed collaboration, (2) proposed cheating, and (3) communicated with the professor are in Figure ~\ref{3Agraph}.\color{purple}

% \textbf{Collaboration.} Across the lenient and medium late policy conditions, adding perturbations to student lives generally increased the frequency in which students proposed collaboration. In the harsh late policy condition, students proposed collaboration in all simulations, regardless of perturbations. 

% \textbf{Cheating.} \color{red}In preliminary simulations without rooms, the behavior of cheating was never observed. This changed after the introduction of rooms. \color{purple} In the lenient late policy condition, students never suggested cheating, regardless of perturbations. In the medium late policy conditions, students never suggested cheating in the no perturbation condition, but did so in one simulation in each of the one perturbation and two perturbation conditions. In the harsh late policy, students suggested cheating in all three perturbation conditions: students suggested cheating at an equal frequency in the no perturbation and one perturbation conditions, and the most in the two perturbation condition. 

% % \textbf{Communication with the Professor} In the lenient late policy condition, students communicated the most with the professor in the condition with two perturbations. However, students communicated with the professor slightly less in condition with one perturbation than in the condition with no perturbation. In the medium late policy condition, students communicated with the professor an equal amount in the no perturbation and one perturbation conditions, and more frequently in the two perturbation condition. In the harsh late policy condition, students communicated with the professor in all simulations regardless of perturbations, similar to the results observed for collaboration.

% % \begin{figure}[h]
% %     \centering
% %     \includegraphics[width=0.75\textwidth]{images/3A.png}  % Change this value to make the figure larger
% %     \caption{Percentage of simulations in which the specified behavior was observed for all 9 simulation conditions.}
% %     \label{3Agraph}
% % \end{figure}

% % The results of the number of simulations in which students (1) proposed collaboration, (2) proposed cheating, and (3) communicated with the professor are in Figure ~\ref{3Agraph}. \color{red}\textbf{From these results, we conclude that SOMEATHING ABOUT ROOMS .... LLM agents collaborate more with harder late policy/perturbations.... and cheat less frequently than they collaborate but also cheat more with harder late policy/perturbations }\color{purple}


% % \color{red} \sout{We find that: (1) rooms enabled private communication which LLM-agents used to propose cheating, and (2) LLM-agents seemed to reasonably respond to changes in late policy and perturbations.}\color{black}

% \subsubsection{Shopping-Cart Return}

% In simulations without stake-prompting, we find that shopper agents still frequently return their carts despite the conditions affecting their ability to do so. However, alluding to what is at stake as a result of the condition  causes shopper agents to stop returning their carts as often. The results are summarized in Figure \ref{3Bgraph}. \textbf{From these results, we conclude that alluding to what is at stake via stake-prompting causes LLM-agents to be affected by external conditions more like humans than without doing so.}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.75\textwidth]{images/3B.png}
%     \caption{Percentage of simulations in which the shopper agent decided to their shopping cart for both external conditions tested and under either prompting condition: with or without stake-prompting. LLM-Agents returned their cart less frequently with stake-prompting than without.}
%     \label{3Bgraph}
% \end{figure}

% % \subsubsection{g}
% % hadhda

% \bigskip
% \bigskip

% \color{red}We use two real-world settings as case studies to identify mechanisms needed to enable informative simulations. For these case studies, we run several simulations with slightly varying conditions to generally understand the ways in which agents act, and then use that to create a mechanism which enables a behavior we identify as missing from a combination of general knowledge and informative studies.

% The first is a classroom setting, where we specifically focus the impact of various late policies (no penalty, full penalty, and penalty by days late) on student communicative and collaborative behaviors. We define a professor agent (named the Professor) and three student agents with arbitrary names (Alice, Bob, and Casey). The professor agent is given instructions to announce a late policy to the class, and then begin assigning assignments. In student agents public biography, they are given one of three "personalities" - an overachiever, a hard-worker, and a balanced individual. In the private biographies of the agents, we add various perturbations to student lives that would reasonably affect their ability to turn in assignments on time, such as having a midterm in another class, having special difficulty with a particular assignment, or having a busy week in general. We do not need to implement a rigid turn-taking guideline, however we do generally add a framework within which agents act - the professor agent announces assignments on a fixed frequency in the classroom, between which student agents "work" on assignments and consider how many days late they will need to submit it based on the other factors in their lives.

% Second, we simulate shoppers in a parking lot who can either return or not return their shopping cart. In each simulation, we define one shopper. We add various perturbations to the shopper life that affect their ability to return their shopping cart \cite{scientificamerican2020shoppingcarts} in their private biography. The shopper agent by default has blank public biographies; but if perturbations added to the shopper's private biography would reasonably be extrapolated other people in real life (such as having a child), we also include it in the shopper's public biography. The shopper agent are not given directives, but have an initial plan to decide whether or not to return their shopping cart, and then to act on it. \color{black}

% \subsubsection{\color{red}Evaluation \& Results for RQ3\color{black}}

% \color{red}

% \begin{itemize}
% \item[1.] Classroom with Late Policies
% \begin{itemize}
% \item We simulate a classroom setting, where students have 5 assignments to submit over the course of a semester.
% \item We try varying late-assignment policies (lenient - all late assignments accepted, harsh - late assignments not accepted, medium - 20\% grade penalty for each late day). 
% \item We add perturbations to student lives that reasonably would affect their ability to turn in assignments on time: (1) having a midterm and (2) a particular assignment being especially challenging.
% \item We also give students personality types: that of a procrastinator, an overachiever, and someone who "values work-life balance."
% \item We wanted to see if multi-agent LLM systems simulated reasonable interactions and dynamics within a classroom.
% \item We sought to examine how students would (1) work together and (2) communicate with one another and the teacher.
% \item In preliminary simulations with one room, a classroom, we found that student agents proposed working together to other student agents.
% \item \color{red}Generally, we saw that procrastinators would suggest collaboration most frequently.\color{purple}
% \item Student agents also would ask questions to the teacher that were both individual (ex. requesting a review) and for the group (ex. clarifying an assignment). 
% \item But everybody in the class would be distracted by them.
% \item Therefore, we added two rooms to the simulation environment to enable easier communication: the teacher's office, and a student work room.
% \item In simulations with the lenient late policy, communication was somewhat similar with or without the added rooms.
% \item Students did move into the work room to "work" as per their directives. 
% \item They also used the office to ask questions to the teacher.
% \item But students discussed working together in a similar way and at roughly the same frequency.
% \item This was true after adding perturbations too.
% \item In simulations with the medium late policy, the ways in which proposed collaboration changed once perturbations were added.
% \item As opposed to broadly discussing working together, student agents sometimes asked to see other agent's assignments to copy in the work room. 
% \item \color{red}Generally, we saw that procrastinators would suggest cheating most frequently.\color{purple}
% \item In simulations with the harsh late policy, we saw this behavior before even adding perturbations.
% \item \color{red}This makes sense, because students have been found to be more likely to cheat on exams if they have strict teachers.\color{purple}
% \item We ran simulations under the lenient (LLP), harsh (HLP), and medium late policies (MLP).
% \item We ran simulations under three perturbation conditions: (P0) without any, (P1) students having a midterm during the 3rd assignment, and (P2) students having the midterm AND the 2nd assignment being especially challenging.
% \item We ran five simulations of each combination of late policy and perturbation (LLP-P0, LLP-P1, LLP-P2, HLP-P0, HLP-P1, HLP-P2, MLP-0, MLP-1, and MLP-2), or 45 simulations total.
% \item We recorded if students (1) proposed collaboration, (2) proposed a form of cheating, and (3) communicated with the teacher.
% \item \color{red}We did not record which student initiated each of the types of actions. We also did not record at which assignment it occurred.\color{purple}
% \item The results are summarized in Table \ref{teachingsims} and Figure \ref{3Agraph}.
% \item{\begin{center}
% \begin{table}[H]
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{10pt}
% \begin{tabular}{|>{\columncolor{gray!20}\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|} 
%  \hline
%  \rowcolor{gray!20} \textbf{Condition} & \textbf{Collaboration} & \textbf{Cheating} & \textbf{Communication with Teacher} \\ 
%  \hline\hline
%  \textbf{LLP-P0} & 40\% & 0\% & 60\% \\ 
%  \hline
%  \textbf{LLP-P1} & 60\% & 0\% & 40\% \\ 
%  \hline
%  \textbf{LLP-P2} & 60\% & 0\% & 80\% \\ 
%  \hline
%  \textbf{MLP-P0} & 60\% & 0\% & 80\% \\ 
%  \hline
%  \textbf{MLP-P1} & 80\% & 20\% & 80\% \\ 
%  \hline
%  \textbf{MLP-P2} & 100\% & 20\% & 100\% \\ 
%  \hline
%  \textbf{HLP-P0} & 100\% & 20\% & 100\% \\ 
%  \hline
%  \textbf{HLP-P1} & 100\% & 20\% & 100\% \\ 
%  \hline
%  \textbf{HLP-P2} & 100\% & 60\% & 100\% \\ 
%  \hline
% \end{tabular}
% \caption{\label{teachingsims}Percentage of simulations in which the specified behavior was observed for all 9 simulation conditions.}
% \end{table}
% \end{center}
% }
% \item{\begin{figure}[h]
%     \centering
%     \includegraphics[width=0.75\textwidth]{images/3A.png}  % Change this value to make the figure larger
%     \caption{Percentage of simulations in which the specified behavior was observed for all 9 simulation conditions.}
%     \label{blah}
% \end{figure}}
% \item \color{red} We find that: (1) rooms enabled private communication which LLM-agents used to propose cheating, and (2) LLM-agents seemed to reasonably respond to changes in late policy and perturbations.
% \end{itemize}
% \end{itemize}

% \begin{itemize}
% \item[2.] Shopping-Cart Return
% \begin{itemize}
% \item We simulate a store parking lot, where there are specific shopping-cart return locations.
% \item Each simulation has one agent with a plan to decide whether or not to return their shopping cart.
% \item We try two perturbations that might contribute to someone not returning their cart: (1) being far from the receptacle (FFR), and (2) having a child whom should not be left unattended (HAC). \cite{scientificamerican2020shoppingcarts}
% \item We have two rooms: the shopper agents car and the receptacle.
% \item We find that despite the perturbations, shopper agents arill frequently return their carts if it the perturbation is merely stated ("you are far from the receptacle," and "you have a child")
% \item However, alluding to what is at stake as a result of the perturbation starts causing shopper agents to stop returning their carts as often ("you are \textit{parked across the parking lot} from the receptacle," and "you have a \textit{five-month old} child").
% \item We present this as \color{red}stake-prompting (SP), a way in which to guide LLM-agents towards acting more in-line with humans.\color{purple}
% \item We ran five simulations of either perturbation (FFR and HAC) with and without prompts alluding to what is at stake, or 20 simulations total.
% \item The results are summarized in Table ~\ref{shoppingcartsims} and Figure \ref{3Bgraph}.
% \item{\begin{center}
% \begin{table}[H]
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{10pt}
% \begin{tabular}{|>{\columncolor{gray!20}\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|} 
%  \hline
%  \rowcolor{gray!20} \textbf{Perturbation} & \textbf{Without SP} & \textbf{With SP} \\ 
%  \hline\hline
%  \textbf{FRB} & 100\% & 40\% \\ 
%  \hline
%  \textbf{HAC} & 60\% & 20\% \\ 
%  \hline
% \end{tabular}
% \caption{Percentage of simulations in which the shopper agent decided to their shopping cart for both perturbations tested and under either prompting condition.}
% \label{shoppingcartsims}
% \end{table}
% \end{center}
% }
% \item{\begin{figure}[h]
%     \centering
%     \includegraphics[width=0.75\textwidth]{images/3B.png}
%     \caption{Percentage of simulations in which the shopper agent decided to their shopping cart for both perturbations tested and under either prompting condition.}
%     \label{3Bgraph}
% \end{figure}}
% \item We find that alluding to what is at stake caused LLM-agents to be more \color{red} affected by perturbations more like people\color{black}.
% \end{itemize}
% \end{itemize}

% \begin{itemize}
% \item[3.] Graffiti \& Littering
% \begin{itemize}
% \item Finally, we simulate two scenarios: (1) a bike-parking station, where a piece of paper is left on the handlebars. people must choose whether or not to litter - there is a no littering sign but no trash can. there is either grafitti on the wall or not, people more likely to litter when there is graffitti. (2) a envelope with cash visible hanging outside of a mailbox. the mail box either has graffiti on it or not.
% \item \color{red}LLM-simulations show .... WIP .... but looks like first sort of should be true, second one looks unlikely but is interesting they won't steal?\color{black}
% \item IDEALLY WOULD BE: WE TRIED X AND IT DID NOT WORK... ADDING Y GOT US CLOSER TO REPLICATING
% \end{itemize}
% \end{itemize}
% \bigskip\bigskip

% \color{red}

% \begin{itemize}
%     \item setup: bike rack location. there is a no littering sign. the wall either has graffiti or not. there is no trash can. there is some trash on the persons bike. in experiments with humans, people litter more often when there is graffiti
%     \item Graffiti on the wall and the no littering sign are set via the location
%     \item we also have to explicitly say, there is no trash can in the location
%     \item we indicate that there is trash on the agents bike via the public biography
%     \item initial plan: take your bike from the station
%     \item so agents are forced to figure out what to do with the trash that is on the bike
%     \item this works, in that LLM-agents do recognize that they need to do something with the trash
%     \item if they start thinking OH LET ME FIND A NEARBY TRASH CAN IN ANOTHER AREA / TAKE THE TRASH WITH THEM, then we say ok they did not litter
%     \item if they simply said I AM GOING TO REMOVE THIS TRASH / DROP THIS TRASH / LITTER etc. we count that as littering
%     \item but im not sure if the impact of the graffiti condition is correctly shown: In 10 simulations, without grafitti, LLMs litter twice. in ten with grafitti, LLMs litter three times. so i guess technically it is higher. but im not really sure if this is telling us anything conclusively
%     \item could write yeah it sort of works but is that even worth the changes we'd have to make elsewhere? if so I can definitely write these sections tonight
% \end{itemize}

% \color{black}

==> source/3_setup.tex <==
% 3 sections; 1. lab experiments, 2. combinations, and 3. evaluation/results

\section{Experimental Setup}

\color{red}wrote this whole section (esp eval) using the word "treatment" either need to define it or (preferably) change it\color{black}

With the goal of better understanding the ability of multi-agent LLM systems to model prosocial human behavior, we simulate three different types of experiments: (1) simulations which aim to directly capture the effect of a treatment observed in a previous lab experiment with human subjects; (2) simulations which combine treatments/effects from multiple previous lab experiments with human subjects; and (3) select "out-of-the-lab" real-world scenarios we use as case studies.

For all experiments, we use OpenAI's GPT. Specifically, we use GPT4 (model gpt-4o-mini), which has been shown to have the ability to interpret inherently human concepts such as equity and also scores  well on a variety of standardized tests, ranging from the Bar Exam to the GRE \cite{openai2023gpt4}.

\subsection{Research Questions}

We specifically address the following three research questions:

\bigskip

\begin{itemize}[itemindent=2.5em]
  \item[\underline{\textbf{RQ1}}] Can multi-agent LLM system simulations replicate behaviors observed in PGG lab experiments with human subjects?
\begin{itemize} [leftmargin=0.5in]
\item[\underline{a.}] Does priming LLM agents via game name replicate the effect of priming humans via game name?
\item[\underline{b.}] Does introducing transparency in contribution between LLM agents replicate the effect of introducing transparency in contribution between humans?
\item[\underline{c.}] Does varying the endowments of LLM agents replicate the effect of varying endowments of humans?
\end{itemize}
\end{itemize}

\bigskip
\color{blue}

\begin{itemize}[itemindent=2.5em]
  \item[\underline{\textbf{RQ1}}] \textit{Can multi-agent LLM system simulations replicate behaviors observed in PGG lab experiments with human subjects?} We answer this research question via three experiments comparing results from simulations with LLM-agents to results from lab experiments with human subjects:
  
  \begin{itemize} [leftmargin=0.5in]
    \item[\underline{1.}] Priming via Game Name
    \item[\underline{2.}] Introducing Transparency of Contributions
    \item[\underline{3.}] Varying Endowments
  \end{itemize}
\end{itemize}

\color{black}

\bigskip

\begin{itemize}[itemindent=2.5em]

  \item[\underline{\textbf{RQ2.}}] Can multi-agent LLM system simulations replicate human behavior extrapolated from combining the behaviors observed in multiple lab experiments with human subjects?
\begin{itemize}[leftmargin=0.5in]
    \item[\underline{a.}] Does priming LLM agents with sentences known to increase/decrease generosity in humans have that effect in simulations of the PGG?
\item[\underline{b.}] Does the effect of priming LLM agents via game name in multi-round PGGs fade over time, like priming has been observed to fade over time in other experiments with human subjects?
\end{itemize}
\end{itemize}

  \bigskip
\color{blue}
\begin{itemize}[itemindent=2.5em]

  \item[\underline{\textbf{RQ2.}}] \textit{Can multi-agent LLM system simulations replicate human behavior extrapolated from combining the behaviors observed in multiple lab experiments with human subjects?} We answer this research question via two experiments combining treatments and expected effects from multiple lab experiments with human subjects:
  \begin{itemize}[leftmargin=0.5in]
    \item[\underline{1.}] Using a priming methodology from other cooperation games in the PGG
    \item[\underline{2.}] Measuring the change in effect of priming over time, using results of priming over time from a different competition game
  \end{itemize}
\end{itemize}
\color{black}

\bigskip

\begin{itemize}
  \item[\underline{\textbf{RQ3.}}] What are required mechanisms for simulations to
inform policy-makers regarding real-world situations to test policies that encourage human collaboration?
\end{itemize}

\bigskip

\color{blue}

\begin{itemize}
  \item[\underline{\textbf{RQ3.}}] \textit{What are required mechanisms for simulations to
inform policy-makers regarding real-world situations to test policies that encourage human collaboration?} We answer this research question via three real-world case studies towards identifying necessary mechanisms:
\begin{itemize}[leftmargin=0.5in]
    \item[\underline{1.}] A classroom setting with varying late-assignment policies
    \item[\underline{2.}] A store parking lot where shoppers need to return shopping carts to designated areas
    \item[\underline{3.}] Graffitti?
  \end{itemize}
\end{itemize}

\color{black}

\bigskip

We expect generally positive results for the first two research questions, given other work has shown the ability of LLMs to replicate lab experiments that are both published and unpublished \cite{hewitt2024predicting}, but still verify this in the context of the PGG towards specifically understanding the abilities of multi-agent LLM systems to simulate prosocial behavior. \color{red}The third research question is more open-ended - we use case studies of two real-world scenarios towards identifying two mechanisms required for simulations to show expected outcomes, a process which can be continued to be used by policy makers. As policy makers consider the specific scenarios which they need to simulate, they may realize and implement new mechanisms required to enable their simulation.\color{black}

\subsection{Multi-Agent-LLM System}

For our experiments, we adapt a previous introduced agent architecture for simulating social emergent behavior \cite{park2023generativeagentsinteractivesimulacra}. In this architecture, the administrator provides each agent with a name, public and private biographies, instructions (called directives), and an initial plan, which consists of a description, stop condition, and a location. The architecture also allows for the creation of rooms, between which agents are able to move. 

\subsubsection{System Setup for Public Goods Game Experiments}

In PGG experiments, there is an agent named and directed to act as the moderator. The remaining agents (varies from three to four depending upon the experiment) are given arbitrary alphabetical names (Alice, Bob, Casey, and David). Each agent's initial endowment is specified in their public biography, which all other agents can see. If there is a priming condition, it is included in the private biography as to expose the desired agent to the priming without leakage to other agents. Communication is not inherently turn-taking in the architecture; so we have to specify the order and method of contribution to player agents via their directives and initial plan. We initialize two separate rooms - the Game Room and the Moderation Room. Player agents are by default in the game room, then travel to the moderation room to tell the moderator their contribution once the player specified as being before them returns to game room from the moderation room after making their contribution. The moderator remains in the moderation room other than to announce payoffs after all players have made contributions. To realize transparency, we simply remove the moderation room, and have all agents make their contributions publicly in the game room. For the experiment with multiple rounds, we use nearly the same instruction set, other than specifying to the moderator and player agents via directives to repeat the same process for multiple rounds.

The thoughts and actions of each player (and the moderator) are displayed in separate output logs, each representing one of the agents involved in the simulation. In each of the output logs, the agent waits for the condition required (the return of the player before them), then acts on the plan of moving to the moderation room and making a contribution by speaking with the moderator. The moderator stores each contribution to memory in order to later announce payoffs. We extract the contribution amount of each agent using a script on each agent's output logs, identifying the section in which the agent speaks in the moderation room and taking the monetary amount in that sentence. We also manually verified these contribution amounts to ensure accuracy.

\subsubsection{System Setup for Real-World Case Studies}

\color{red}We use two real-world settings as case studies to identify mechanisms needed to enable informative simulations. For these case studies, we run several simulations with slightly varying conditions to generally understand the ways in which agents act, and then use that to create a mechanism which enables a behavior we identify as missing from a combination of general knowledge and informative studies.

The first is a classroom setting, where we specifically focus the impact of various late policies (no penalty, full penalty, and penalty by days late) on student communicative and collaborative behaviors. We define a professor agent (named the Professor) and three student agents with arbitrary names (Alice, Bob, and Casey). The professor agent is given instructions to announce a late policy to the class, and then begin assigning assignments. In student agents public biography, they are given one of three "personalities" - an overachiever, a hard-worker, and a balanced individual. In the private biographies of the agents, we add various perturbations to student lives that would reasonably affect their ability to turn in assignments on time, such as having a midterm in another class, having special difficulty with a particular assignment, or having a busy week in general. We do not need to implement a rigid turn-taking guideline, however we do generally add a framework within which agents act - the professor agent announces assignments on a fixed frequency in the classroom, between which student agents "work" on assignments and consider how many days late they will need to submit it based on the other factors in their lives.

Second, we simulate shoppers in a parking lot who can either return or not return their shopping cart. We define five shopper agents with arbitrary names (Alice, Bob, Casey, David, and Emery). We add various perturbations to shopper lives that affect their ability to return their shopping cart \cite{scientificamerican2020shoppingcarts} in their private biographies. Shopper agents by default have blank public biographies; but if perturbations added to the shopper's private biography would reasonably be extrapolated other people in real life (such as having a child), we also include it in the shopper's public biography. Shopper agents are not given directives, but have an initial plan to decide whether or not to return their shopping cart, and then to act on it. We also try changing the environment by adding agents who are employees of the store tasked with taking the shopping carts from the parking lot back into the store. These agents are given the name "Employee," have public biographies which indicate that they are a store employee, have an initial plan (and related directives) to move carts, and otherwise have all other fields left blank.\color{black}

\subsection{Evaluation}

\subsubsection{Replicating Observed Outcomes from Past Public Goods Game Experiments}

For experiments of the first type, we run simulations of the PGG using treatments from published lab experiments with human subjects, checking whether the effect of said treatments on multi-agents LLMs in simulation in similar to that of on humans. The treatments and effects we replicate from previous lab experiments are listed in Table ~\ref{labexperiments}.

\begin{center}
\begin{table}[H]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{10pt}
\begin{tabular}{|>{\columncolor{gray!20}\centering\arraybackslash}m{0.5cm}|p{6cm}|p{6cm}|} 
 \hline
 \rowcolor{gray!20} \textbf{Exp.} & \multicolumn{1}{c|}{\textbf{Treatment}} & \multicolumn{1}{c|}{\textbf{Expected Result}} \\ [0.5ex] 
 \hline\hline
 \textbf{1} & \textbf{Priming via Game Name:} Participants are presented the PGG as a game called either the "Taxation Game" or "Teamwork Game." & Participants presented the game as the "Taxation Game" contribute less than participants presented the "Teamwork Game." \cite{Eriksson_Strimling_2014} \\ 
 \hline
 \textbf{2} & \textbf{Transparency of Contribution:} Participants know what others contribute to the public pool (under standard conditions, contributions are made privately with respect to other players). & Participants make larger contributions when participants are aware of each other's contributions compared to when contributions are made privately without other's knowledge. \cite{transparencytwo}\\
 \hline
 \textbf{3} & \textbf{Variations in Endowment:} Participants start the PGG with different endowment amounts. & "Rich" participants contribute more when other participants are also "rich." \cite{HARGREAVESHEAP20164}  \\
 \hline
\end{tabular}
\caption{\label{labexperiments}Table of treatments and expected results (effects) from previous lab experiments of the PGG with human subjects. Actual experiments that are drawn from are cited in the second column.}
\end{table}
\end{center}




For these experiments, we simulate one-shot PGGs with three or four players, measuring whether the impact the treatments have on player contributions is similar to what has been observed in experiments with human subjects (i.e., the expected result listed). For the first experiment, we run ten simulations of the PGG with four players, two under each priming condition, and compare the average contribution amount of players from either group. For the second experiment, we also run ten simulations of the PGG with four players: five simulations with transparency of contributions and five without. We compare the average contribution amount of players in either of the two conditions. In the first and second experiments, players are all endowed with \$20. For the third experiment, we run twenty simulations with three players: fifteen simulations where all players have the same initial endowment (five where that endowment is \$20, five where it is \$50, and five where it is \$80) and five simulations where players have different initial endowments (namely, \$20, \$50, and \$80). We compare the average contributions of players with each of the three endowments in the fixed and the varied endowment conditions (i.e., we compare how much a player with \$X contributes in the condition where everyone has \$X vs. the varied condition). In all three experiments, 1.6 times the amount of the public pool is split evenly amongst the players as their payoff - players are made aware of this to inform the way in which they act, but the simulations are of one-shot PGGs.

\subsubsection{Verifying Outcomes from Combinations of Past Lab Experiments}

We also design two additional experiments based on a combination of treatments and effects from multiple lab experiments with human subjects. The first takes a priming methodology and effect from experiments with human subjects of different cooperative games than the PGG to see if the effect holds for the PGG. The second uses a priming methodology used on the one-shot PGG and measures if it has the same effect over multiple rounds similar to the way in which priming affects different economic games than the PGG. The treatments and effects in the combined experiments we design are listed in Table ~\ref{combinedexperiments}.

\begin{center}
\begin{table}[H]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{10pt}
\begin{tabular}{|>{\columncolor{gray!20}\centering\arraybackslash}m{0.5cm}|p{6cm}|p{6cm}|} 
 \hline
 \rowcolor{gray!20} \textbf{Exp.} & \multicolumn{1}{c|}{\textbf{Treatment}} & \multicolumn{1}{c|}{\textbf{Expected Result}} \\ [0.5ex] 
 \hline\hline
 \textbf{1} & \textbf{Priming via Sentences:} Participants are presented with 5 sentences alluding to either "unity" or "proportionality" concepts. & Participants presented with sentences alluding to "unity" contribute more than participants primed with "proportionality". \cite{6d947858-4a17-3462-9053-fc55b58ffee1, moralsmatter} \\ 
 \hline
 \textbf{2} & \textbf{Priming via Game Name over Multiple Rounds:} Participants are presented the PGG as a game called either the "Taxation Game" or "Teamwork Game" and play for five rounds. & The effect of priming should fade over time; although there should still be a disparity between participants in either group's initial contributions, it should lessen over time. \cite{Eriksson_Strimling_2014, JIMENEZJIMENEZ201594} \\
 \hline
\end{tabular}
\caption{\label{combinedexperiments}Table of treatments and expected results (effects) from combining previous lab experiments with human subjects. Actual experiments that are drawn from are cited in the second column.}
\end{table}
\end{center}

For both experiments, all players are endowed with \$20. For the first experiment, we run ten simulations a one-shot PGG with four players, two under each priming condition ("unity" and "proportionality"), and compare the average contribution amount of players from either group. We prime each player by exposing them to five sentences alluding to each concept, taken from the lab experiment \cite{moralsmatter}. In this experiment, 1.6 times the amount of the public pool is split evenly amongst the players as their payoff - players are made aware of this to inform the way in which they act, but the simulations are of one-shot PGGs. For the second experiment, we run ten simulations of a PGG with five rounds and four players, two under each priming condition ("Taxation" and "Teamwork"). In this experiment, payoffs are computed the same as in the previous experiment (namely, 1.6 times the amount of the public pool split evenly amongst the players). Since there are multiple rounds, the payoff and amount not contributed are summed to determine each players endowment for the next round. Within each priming condition, we compare the average contribution in the first round compared to the fifth round. We also compare the contributions between priming conditions, checking that there was an initial disparity that ultimately begins to fade.

\color{red}

\subsubsection{Real-World Case Studies}

SEE RESULTS, THERE'S A BIG BULLET POINT LIST OF EVAL / RESULTS COMBINED I'M TRYING TO FIGURE OUT HOW TO SEPARATE. 

TALK ABOUT HOW THESE CONNECT TO PROSOCIAL SITUATIONS HERE?

\color{black}

==> source/4_results.tex <==
\section{Results}

Based on the results from our experiments, we answer our research questions.

\subsection{\underline{RQ1}: Can multi-agent LLM system simulations replicate behaviors observed in PGG lab experiments with human subjects?}

Towards answering this question, we simulate treatments from three different lab experiments with human subjects: (1) priming via game name, (2) transparency of contributions, and (3) variations in endowment. In the first two experiments, LLM-agents replicate the direction of effects with statistical significance, but overestimates the magnitude. In the third experiment, LLM-agents replicate the direction of effects but the effect is not statistically significant, although this is likely due to lack of data. \textbf{Overall, we conclude that LLM-agents are able to replicate the direction of the effect of priming and transparency treatments, \color{orange}but testing their ability to replicate the effect of a varied endowment requires further simulations.\color{black}}

\subsubsection{Does priming LLM agents via game name replicate the effect of priming humans via game name?}

In experiments with human subjects, participants presented the PGG as the "Teamwork Game" contributed roughly 60\% of their endowments while participants presented the game as the "Taxation Game" contributed roughly 40\% of their endowments \cite{Eriksson_Strimling_2014}. Across ten simulations on average, LLM agents presented the PGG as the "Teamwork Game" (Alice and Bob) contributed approximately 70\% of their \$20 endowment. In comparison, agents presented the PGG as the "Taxation Game" (Casey and David) contributed only approximately 30\% of their endowment to the public pool. These results are summarized in Figure \ref{1Agraph}. A t-test shows that the difference in contributions between the two groups is statistically significant at the p < 0.01 level  
(\(t = 7.92, p < 1\text{e}{-8} \)).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/1A.png}
    \caption{Average contributions for "Teamwork" and "Taxation" priming conditions in simulations with LLM-agents and experiments with human subjects. Average contributions are above 60\% in the "Teamwork" priming condition for both groups. Average contributions are below 40\% in the "Taxation" priming condition for both groups.}
    \label{1Agraph}
\end{figure}

\textbf{From these results, we conclude that priming LLM agents by presenting the PGG under different names replicates the direction of the effect of doing the same on humans, but may overestimate the magnitude.}

\subsubsection{Does introducing transparency in contribution between LLM agents replicate the effect of introducing transparency in contribution between humans?}

In experiments with human subjects, participants contributed on average 6\% more of their endowment under transparency conditions as compared to no transparency. \cite{transparencytwo}. Across five simulations of each condition (ten simulations total) on average, LLM agents playing the PGG with transparency contributed approximately 60\% of their 20\$ endowment, whereas LLM agents playing the PGG without transparency contributed only approximately 35\% of their endowment. \color{orange}These results are summarized in Figure \ref{1Bgraph}\color{black}. A t-test shows that the difference in contributions between the two groups is statistically significant at the p < 0.05 level  
(\(t = 2.23, p = 0.031 \)).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/1B.png}
    \caption{Average contributions with and without transparency for simulations. Only the difference in contribution is listed in the lab experiment from which this treatment/effect was found. \cite{transparencytwo}.}
    \label{1Bgraph}
\end{figure}

\textbf{From these results, we conclude that introducing transparency of contributions in PGGs with LLM agents replicates the direction of the effect of doing the same on humans, but may overestimate the magnitude.}

% "If controlling for the MPCR, however, as is done in specifications (6) and (8), the positive effect of F.indichoice and the negative effect of F.indipayoffs have a larger magnitude and turn significant at the 5% level. The share contributed tends to be about 6 percentage points higher than in cases where players receive feedback about the distribution of choices in their group."


\subsubsection{Does varying the endowments of LLM agents replicate the effect of varying endowments of humans?}

In experiments with human subjects, it was found "poor" and "medium" wealth individuals contributed roughly the same amount in equal and varied endowment conditions, whereas "rich" individuals contributed more in the equal endowment condition than in the varied endowment condition \cite{HARGREAVESHEAP20164}. Across five simulations each of \$20-\$20-\$20, \$50-\$50-\$50, and \$80-\$80-\$80 equal endowment conditions, LLM agents on average contributed approximately 39\%, 48\%, and 63\% of their endowments, respectively. In five simulations of a \$20-\$50-\$80 varied endowment condition, on average the LLM agent given \$20 contributed approximately 35\%; the LLM agent given \$50 contributed approximately 42\%; and the LLM agent given \$80 contribute approximately 44\%. Thus, the contribution for agents endowed with \$20 was roughly the same between the equal and varied endowment conditions, whereas agents endowed with \$50 and \$80 both contributed less in the varied condition. These results are summarized in Table \ref{1Cgraph}. T-tests shows that there is no statistically significant difference at the p < 0.1 between the contributions of LLM agents endowed with \$20 in the equal and varied endowment condition (\(t = 0.18, p = 0.86 \)), nor for the \$50 (\(t = -0.56, p = 0.58 \)) endowment - both results mirroring those of human subjects. However, a t-test shows that the difference between the contributions of LLM agents endowed with \$80 is also not statistically significant at the p < 0.1 level (\(t = 1.25, p = 0.23 \)).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{images/1C.png}  % Change this value to make the figure larger
    \caption{Average contributions for equal and varied endowment conditions in simulations with LLM-agents and experiments with human subjects. Average contributions are roughly the same for humans and LLM-agents in the equal and varied endowment conditions with \$20 and \$50 endowments. Average contributions are lower in the varied condition than in the fixed condition with \$80 endowments.}
    \label{1Cgraph}
\end{figure}

% \begin{table}[htbp]
% \centering
% \begin{tabular}{|>{\columncolor{gray!20}}c|c|c|c|}
% \hline
% \rowcolor{gray!20}\multicolumn{1}{|c|}{} & \multicolumn{3}{c|}{\textbf{Initial Endowment}} \\ \hline
% \rowcolor{gray!20}\textbf{Condition} & \$20 & \$50 & \$80 \\ \hline
% Equal & 39\% & 48\% & 63\% \\ \hline
% Varied & 35\% & 42\% & 44\% \\ \hline
% p-value & 0.86 & 0.58 & 0.23 \\ \hline
% t-stat & 0.18 & -0.56 & 1.25 \\ \hline
% \end{tabular}
% \caption{\color{red}IK THIS TABLE MAKES NO SENSE\color{black}}
% \label{variedend}
% \end{table}

\color{orange}
From these results, we cannot fully conclude that LLM agents are affected by varying endowments in the same way as humans. However, the lack of difference between the average contribution in the equal and varied condition with endowments of \$20 and \$50 along with the difference between the averages in the equal and varied endowment conditions does suggest that varying endowments does have an impact similar to the effect observed in humans. The lack of statistical significance could be a result of the limited and unequal number of data points in both groups of comparison (for every endowment amount, there are 15 contributions in the equal endowment condition compared  to only 5 contributions in the varied endowment condition in our simulations).
\color{black}

\subsection{\underline{RQ2}: Can multi-agent LLM system simulations replicate human behavior extrapolated from combining the behaviors observed in multiple lab experiments with human subjects?}

Towards answering this question, we simulate two experiments designed as a combination of multiple lab experiments with human subjects: \color{red}(1) takes a priming methodology and effect from experiments with human subjects of different cooperative games than the PGG to see if the effect holds for the PGG, and (2) uses a priming methodology used on the one-shot PGG and measures if it has the same effect over multiple rounds similar to the way in which priming affects different economic games than the PGG. \color{black} \textbf{From the results of these experiments, we conclude that multi-agent LLM system simulations do replicate behavior extrapolated from combining the behaviors observed in multiple lab experiments with human subjects.}

\subsubsection{Does priming LLM agents with sentences known to increase/decrease generosity in humans have that effect in simulations of the PGG?}

In experiments of other cooperation games, priming participants via sentences alluding to "unity" resulted in participants being more generous than participants primed via sentences alluding to "proportionality" \cite{moralsmatter}. In ten simulations, LLM agents primed with the sentences alluding to "unity" (Alice and Bob) contributed on average approximately 65\% of their initial endowment. In comparison, agents primed with the sentences alluding to "proportionality" (Casey and David) contributed on average only approximately 30\% of their endowment to the public pool. The results are summarized in Figure \ref{2Agraph}. A t-test shows that the difference in contributions between the two groups is statistically significant at the p < 0.01 level (\(t = 8.76, p < 1\text{e}{-9} \)).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/2A.png}
    \caption{Average contributions for either "unity" or "proportionality" priming conditions. Average contributions under the "unity" condition are significantly higher than that under the "proportionality" condition.}
    \label{2Agraph}
\end{figure}

\textbf{From these results, we conclude that priming LLM agents with sentences known to increase/decrease generosity in humans does result in higher/lower contributions in simulations of the PGG.}

\subsubsection{Does the effect of priming LLM agents via game name in multi-round PGGs fade over time, like priming has been observed to fade over time in other experiments with human subjects?}
\bigskip
In experiments of competition games with human subjects, the effect of primings have been found to fade over time \cite{JIMENEZJIMENEZ201594}. In ten simulations, LLM agents presented a five-round PGG as the "Teamwork Game" (Alice and Bob) on average contributed 75\% of their initial endowment in the first round, compared to 55\% of their initial endowment in the fifth round. In comparison, agents presented the PGG as the "Taxation Game" (Casey and David) contributed 30\% of their initial endowment in the first round, compared to 45\% of their initial endowment in the fifth round. Hence, for both priming conditions, the average contribution was closer to 50\% of the initial endowment in the fifth round than in the first, meaning the effect of the priming was less pronounced in the fifth round than the first. The results are summarized in Figure \ref{2Bgraph}. T-tests show that the difference in contribution amount between the rounds is statistically significant for the "Teamwork" priming condition at the p < 0.01 level (\(t = 4.32, p = 0.002 \)) and for the "Taxation" priming condition at the p < 0.05 level (\(t = -2.30, p = 0.047 \)).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/2B.png}
    \caption{Average contributions in the first and fifth rounds for either "Teamwork" and "Taxation" priming conditions. Average contributions in the fifth round are closer to 50\% of the initial endowment, the average amount contributed without any priming \cite{labexperiments}.}
    \label{2Bgraph}
\end{figure}

\textbf{From these results, we conclude that the effect of priming LLM agents fades over time, as observed in experiments with human subjects.} The "Taxation" priming condition specifically suggests that the difference between first and fifth round contributions is not because contributions in PGGs with human subjects decrease over time \cite{labexperiments}, but rather likely the consequence of a fading priming effect.

\subsection{\underline{RQ3}: What are required mechanisms for simulations to
inform policy-makers regarding real-world situations?} 

\color{purple}

\begin{itemize}
\item[1.] Classroom with Late Policies
\begin{itemize}
\item We simulate a classroom setting, where students have 5 assignments to submit over the course of a semester.
\item We try varying late-assignment policies (lenient - all late assignments accepted, harsh - late assignments not accepted, medium - 20\% grade penalty for each late day). 
\item We add perturbations to student lives that reasonably would affect their ability to turn in assignments on time: (1) having a midterm and (2) a particular assignment being especially challenging.
\item We also give students personality types: that of a procrastinator, an overachiever, and someone who "values work-life balance."
\item We wanted to see if multi-agent LLM systems simulated reasonable interactions and dynamics within a classroom.
\item We sought to examine how students would (1) work together and (2) communicate with one another and the teacher.
\item In preliminary simulations with one room, a classroom, we found that student agents proposed working together to other student agents.
\item \color{red}Generally, we saw that procrastinators would suggest collaboration most frequently.\color{purple}
\item Student agents also would ask questions to the teacher that were both individual (ex. requesting a review) and for the group (ex. clarifying an assignment). 
\item But everybody in the class would be distracted by them.
\item Therefore, we added two rooms to the simulation environment to enable easier communication: the teacher's office, and a student work room.
\item In simulations with the lenient late policy, communication was somewhat similar with or without the added rooms.
\item Students did move into the work room to "work" as per their directives. 
\item They also used the office to ask questions to the teacher.
\item But students discussed working together in a similar way and at roughly the same frequency.
\item This was true after adding perturbations too.
\item In simulations with the medium late policy, the ways in which proposed collaboration changed once perturbations were added.
\item As opposed to broadly discussing working together, student agents sometimes asked to see other agent's assignments to copy in the work room. 
\item \color{red}Generally, we saw that procrastinators would suggest cheating most frequently.\color{purple}
\item In simulations with the harsh late policy, we saw this behavior before even adding perturbations.
\item \color{red}This makes sense, because students have been found to be more likely to cheat on exams if they have strict teachers.\color{purple}
\item We ran simulations under the lenient (LLP), harsh (HLP), and medium late policies (MLP).
\item We ran simulations under three perturbation conditions: (P0) without any, (P1) students having a midterm during the 3rd assignment, and (P2) students having the midterm AND the 2nd assignment being especially challenging.
\item We ran five simulations of each combination of late policy and perturbation (LLP-P0, LLP-P1, LLP-P2, HLP-P0, HLP-P1, HLP-P2, MLP-0, MLP-1, and MLP-2), or 45 simulations total.
\item We recorded if students (1) proposed collaboration, (2) proposed a form of cheating, and (3) communicated with the teacher.
\item \color{red}We did not record which student initiated each of the types of actions. We also did not record at which assignment it occurred.\color{purple}
\item The results are summarized in Table \ref{teachingsims} and Figure \ref{3Agraph}.
\item{\begin{center}
\begin{table}[H]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{10pt}
\begin{tabular}{|>{\columncolor{gray!20}\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|} 
 \hline
 \rowcolor{gray!20} \textbf{Condition} & \textbf{Collaboration} & \textbf{Cheating} & \textbf{Communication with Teacher} \\ 
 \hline\hline
 \textbf{LLP-P0} & 40\% & 0\% & 60\% \\ 
 \hline
 \textbf{LLP-P1} & 60\% & 0\% & 40\% \\ 
 \hline
 \textbf{LLP-P2} & 60\% & 0\% & 80\% \\ 
 \hline
 \textbf{MLP-P0} & 60\% & 0\% & 80\% \\ 
 \hline
 \textbf{MLP-P1} & 80\% & 20\% & 80\% \\ 
 \hline
 \textbf{MLP-P2} & 100\% & 20\% & 100\% \\ 
 \hline
 \textbf{HLP-P0} & 100\% & 20\% & 100\% \\ 
 \hline
 \textbf{HLP-P1} & 100\% & 20\% & 100\% \\ 
 \hline
 \textbf{HLP-P2} & 100\% & 60\% & 100\% \\ 
 \hline
\end{tabular}
\caption{\label{teachingsims}Percentage of simulations in which the specified behavior was observed for all 9 simulation conditions.}
\end{table}
\end{center}
}
\item{\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{images/3A.png}  % Change this value to make the figure larger
    \caption{Percentage of simulations in which the specified behavior was observed for all 9 simulation conditions.}
    \label{3Agraph}
\end{figure}}
\item \color{purple} We find that: (1) rooms enabled private communication which LLM-agents used to propose cheating, and (2) LLM-agents seemed to reasonably respond to changes in late policy and perturbations.
\end{itemize}
\end{itemize}

\begin{itemize}
\item[2.] Shopping Cart Return
\begin{itemize}
\item We simulate a store parking lot, where there are specific shopping cart return locations.
\item Each simulation has one agent with a plan to decide whether or not to return their shopping cart.
\item We try two perturbations that might contribute to someone not returning their cart: (1) being far from the receptacle (FFR), and (2) having a child whom should not be left unattended (HAC). \cite{scientificamerican2020shoppingcarts}
\item We have two rooms: the shopper agents car and the receptacle.
\item We find that despite the perturbations, shopper agents arill frequently return their carts if it the perturbation is merely stated ("you are far from the receptacle," and "you have a child")
\item However, alluding to what is at stake as a result of the perturbation starts causing shopper agents to stop returning their carts as often ("you are \textit{parked across the parking lot} from the receptacle," and "you have a \textit{five-month old} child").
\item We present this as \color{red}stake-prompting (SP), a way in which to guide LLM-agents towards acting more in-line with humans.\color{purple}
\item We ran five simulations of either perturbation (FFR and HAC) with and without prompts alluding to what is at stake, or 20 simulations total.
\item The results are summarized in Table ~\ref{shoppingcartsims} and Figure \ref{3Bgraph}.
\item{\begin{center}
\begin{table}[H]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{10pt}
\begin{tabular}{|>{\columncolor{gray!20}\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{3cm}|} 
 \hline
 \rowcolor{gray!20} \textbf{Perturbation} & \textbf{Without SP} & \textbf{With SP} \\ 
 \hline\hline
 \textbf{FRB} & 100\% & 40\% \\ 
 \hline
 \textbf{HAC} & 60\% & 20\% \\ 
 \hline
\end{tabular}
\caption{Percentage of simulations in which the shopper agent decided to \color{red} MISSING THOUGHT HERE their shopping cart for both perturbations tested and under either prompting condition. ALSO, IF THE GRAPH HAS CRYTIC ACRYNYMS like SP FRR HAC, you MUST define in the cpation. \color{black}}
\label{shoppingcartsims}
\end{table}
\end{center}
}
\item{\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{images/3B.png}
    \caption{Percentage of simulations in which the shopper agent decided to their shopping cart for both perturbations tested and under either prompting condition.}
    \label{3Bgraph}
\end{figure}}
\item We find that alluding to what is at stake caused LLM-agents to be more \color{red} affected by perturbations more like people\color{black}.
\end{itemize}
\end{itemize}

\begin{itemize}
\item[3.] Graffiti \& Littering
\begin{itemize}
\item Finally, we simulate two scenarios: (1) a bike-parking station, where a piece of paper is left on the handlebars. people must choose whether or not to litter - there is a no littering sign but no trash can. there is either grafitti on the wall or not, people more likely to litter when there is graffitti. (2) a envelope with cash visible hanging outside of a mailbox. the mail box either has graffiti on it or not.
\item \color{red}LLM-simulations show .... WIP .... but looks like first sort of should be true, second one looks unlikely but is interesting they won't steal?\color{black}
\item IDEALLY WOULD BE: WE TRIED X AND IT DID NOT WORK... ADDING Y GOT US CLOSER TO REPLICATING
\end{itemize}
\end{itemize}

\color{black}






==> source/5_discussion.tex <==
\section{Discussion}
\subsection{Generalizable Mechanisms to Enable Unbounded Behaviors in Simulation}

Simulations of real-world scenarios are particularly valuable when they produce realistic human behaviors that were not explicitly prompted. We refer to these as "unbounded behaviors" because they occur outside the expected framework of the simulation. Such behaviors are difficult to predict with traditional models, but multi-agent LLM systems have the unique potential to generate them. In Study 3, we observed unbounded behaviors such as cheating in a classroom simulation and shoppers neglecting to return carts in a parking lot.%, and littering in a graffiti simulation.

However, in these scenarios, additional mechanisms were needed to enable the emergence of unbounded behaviors. For instance, we had to introduce private rooms to observe cheating in the classroom, and we had to add clear stakes (such as "you have an infant waiting in the car") to see agents failing to return shopping carts. %In the graffiti simulation, littering occurred without any modifications, but not in the proportions observed in real-world studies.
If every simulation requires a custom mechanism to produce specific unbounded behaviors, the value of simulations diminishes —they would only reflect behaviors that researchers expect, thus undermining the purpose of simulation. However, if the mechanisms are generalizable, they can be widely implemented, allowing simulations to still produce meaningful unbounded behaviors. The question remains: were the mechanisms we added general or specific? With only two examples, it's hard to draw definitive conclusions, but there is reason to believe they could be broadly applicable.

In the classroom simulation, the introduction of private rooms was necessary to observe cheating. In hindsight, it seems obvious that students would only cheat if they had a private space to communicate without getting caught. Broadly speaking, communication is a fundamental mechanism in society that enables many unexpected outcomes. The invention of the telephone, the internet, and even home-delivered mail has had significant effects on the economy (increasing global trade and commerce), employment (enabling remote work), and culture (connecting distant people). Any simulation that tests cooperation will likely need diverse communication channels (private, public, synchronous, asynchronous) to allow for various forms of interaction and collaboration.

In the shopping cart simulation, adding stakes was essential. Studies show that people with a child waiting in the car are less likely to return their cart. However, we initially did not see this effect in the simulation. Upon reflection, the condition "having a child" was too vague. If the child was 12 years old, there was little pressure to skip returning the cart. But if the child was 5 months old, there was significant urgency. When we clarified the child's age in the simulation, the unbounded behavior emerged for parents with a 5-month-old more frequently than for parents with a child of unspecified age. This outcome makes sense, as it was a flaw in the initial setup to specify only "having a child" without including age. To simulate unbounded behaviors effectively, simulations need enough contextual details for agents to understand the stakes and reason for their actions.

In the future, more work is needed to discover a set of mechanisms that enable simulations to exhibit rich, bounded human behavior. Communication channels and detailed contextual stakes are likely two such mechanisms, but there are probably many more that need to be discovered.

\subsection{How can policymakers benefit from imperfect simulations with multi-agent systems?}
These experiments showed that multi-agent LLM simulations can replicate the direction of effects (though perhaps not the magnitude) and extend to situations not explicitly covered in the literature. They also have the capability to exhibit unbounded actions. These are all encouraging signs that these simulations could be a valuable tool for policymakers, but the reality is that they will never be perfect. The question is: can they still be useful despite their imperfections?

Even if simulations are not completely accurate, they can still serve as ideation tools to imagine different possible outcomes. Prospection — the ability to think and reason about the future—is a hallmark of human intelligence, yet it is something that many people struggle with. When thinking about the future, people often find it difficult to account for the complexity of multiple independent actors' decisions, fall prey to cognitive biases (such as optimism bias when they want a policy to succeed), and struggle to imagine novel situations for which they have little prior experience. Although future thinking is important, it is cognitively taxing, and any aids might be better than relying solely on our limited cognition. LLM systems, while imperfect, are relatively fast, low-cost, and can run multiple scenarios. In many cases, a reasonable simulation is better than none at all.

If simulations are accurate in predicting the direction of effects and relative effect sizes (even if not their exact magnitude), they can still be valuable for testing different policies to determine whether they will be effective (even if not precisely how effective). This can be especially useful because some policies are known to fade quickly over time, becoming ineffective unless frequently renewed, while others persist by establishing new norms—such as making organ donation the default option instead of requiring an opt-in. A simulation, particularly one that tracks effects over time, could reveal these policy limitations. Additionally, simulations can expose potential negative externalities, such as added bureaucracy or unintentionally excluding participants (for example, when new market regulations make it harder for newcomers to enter).

Simulations can also serve as a boundary object that helps individuals from diverse backgrounds integrate their knowledge. Many complex scenarios involve various areas of expertise and perspectives. In a city, a proposal like introducing a bike lane affects many departments —- transportation, waste management, emergency route planning, and legal services. Instead of each department prioritizing its own concerns, a simulation might help different groups see how their concerns intersect, fostering a more collaborative discussion. Thus, simulations could function as a social glue for large organizations.

While there is much work to be done with policymakers to determine the value of imperfect simulations, there are reasons to believe they could be useful for tackling a challenging and important problem that currently has few affordable and accessible feedback mechanisms.

% These experiments showed that MA-LLM simulations can replication the direct of effects (although not the magnitude), and can extend to situations not explicitly seen before the the literature. They also have the capability to exhibit unbounded actions. These are all encouraging signs that these simulations could be a tool for policymakers, but the obvious truth is that these simulations will never be perfect. Can they still be useful, even if they are imperfect?

% Even if simulations are not completely accurate, In the worst case they can act as ideation tools to imagine different possible outcomes. Prospection - the ability to think and reason about the future - is one of the hallmarks of human intelligence - and yet it is something most people struggle with. When trying to think about the future people struggle with the complexity of thinking through multiple independent actors' decisions, they struggle with cognitive biases, such as optimism bias when they want a policy to have the desired effect, and they struggle to imagine novel situations for which the brain has less experience to draw from. Although future thinking is important, it is hugely cognitively taxing, and any aids might be better than our own limited cognition. AI systems - albeit imperfect - are fast, low cost, and can be done many times. In many situations, any reasonable simulation might be better than none.

% If simulations are accurate in their effect direction and the relative effect size (but not magnitude), this can still be a good tool to test different policies to at least say if they will be effective (even if they can’t say how effective). This is useful because some policys are known to fade quickly over time, rendering them ineffective unless repeated often. Whereasother policies are known to persist - because they create a new norm - like making organ donation the default (rather than an opt-in). A simulation  - particularly one that helps look at effects over time could expose these policy flaws. Additionally, simulations can expose potential negative externalities - such as like additional paperwork or inadvertently excluding participants (often adding regulation to markets makes it harder for new people to enter). 

% Simulations can also be a boundary object that help people from multiple backgrounds integrate their knowledge. Many complex scenarios involve many types of expertise and personas. Cities have many types of experts, and a proposal like introducing a bike lane will affect many of them - transportation, garbage collection, emergency route planning. Legal. Rather than every department seeing it’s concerns as the top priority, a simulation might help groups see how their concerns are integrated and start a conversation. Thus, simulations could function as  “AI as social glue.” for large organizations [AI as social glue]

% Whereas there is much work to be done with policymakers to find the value of imperfect simulations, there are reasons to believe they can have utility for a very hard and important problem that currently has few alternatives for cheap and easy feedback mechanisms. 

\subsection{Future interfaces for simulations}
Although the simulations in this study were set up and run in a console without a specialized user interface, there are many ways people might want to interact with simulations in the future that would require rich user interfaces. After a simulation has been run, users may want to step through it to better understand the sequence of events that led to a particular outcome. They might also wish to compare two runs of the simulation with different outcomes to hypothesize which factors contributed to those differences. While these simulations were run in a batch mode (without user interaction), many users may prefer interactive simulations that allow them to interrupt the process, adjust parameters, or intervene to try to create or prevent certain outcomes. Additionally, users may want to fork a simulation at a particular stage to explore multiple parallel scenarios.

Since designing and validating a comprehensive simulation environment with all the necessary mechanisms is challenging, there could be a future where people use or modify existing environments rather than building one from scratch. For example, a large city simulation could be utilized by various organizations: city governments could use it to prepare for natural disasters, hospitals to allocate resources during medical emergencies, businesses to explore store locations, and civic planners to mitigate the effects of climate change. Such environments could be developed collectively and made available to the public, much like open-source code. However, there are also ethical concerns; simulations could be misused in harmful ways, and there may be reasons to restrict access to simulations of public places or sensitive areas.  As LLM simulations become easier to use, it is critical to build safegaurds to limit "bad actors" from using simulations to model nefarious situations like war or voter/consumer manipulation. Furthermore, overreliance on simulations is a major concern - AI simulations are much cheaper and easier to conduct than real design and policy work. However, when designing policies for people, it is still important to run experiments with real humans and use traditional methods to think through all possible consequences; simulations should only be used as an additional thinking tool, as opposed to being viewed as a standalone representation of ground truth. \color{black}

% Although the simulations in this study were set up and run in a console with no special user interface, in the future there are many ways that people might want to interaction with simulations that would require rich user interfaces. After a simulation has been run, users might want to set through the simulation to better understand what steps lead to a particular outcome. They might want to compare two runs of the simulation with different outcomes to be able to hypothesize which steps led to a particular outcome. These simulations were run in a batch (without user interaction); many users want to run interactive simulations, allowing them to interrupt the simulation and change parameters to interfere to try to create or prevent certain outcomes. Users may also want to fork a simulation at a particular stage to explore two parallel patterns. 

% Since a rich simulation environment with all the necessary mechanisms in place is hard to design and validate, there may be a future where people can use or modify other users' environments rather than building one from scratch. An environment of a large city could be used by many different organizations - city governments can use it to prepare for natural disasters, hospitals can use it to allocate resources during medical emergencies, businesses can use it to explore store locations, and civic planners can use it to mitigate the effects of climate change. Environments can be created collectively and used by everyone like open source code. However, there are many unethical ways a simulation could be used, and there may be reasons to restrict access to simulations of public places or sensitive areas. 

% \color{red}\subsection{Extending the Results of Previous Research}
% % While the results of our studies show several new findings, there is also consistency with past research. Prior work has shown that LLM simulations are able to capture directional effects in published and non-published lab experiments with human subjects \cite{hewitt2024predicting}. Our studies support this finding, specifically studying the PGG as a case study - we replicate published PGG experiments in the first study, while we study "unpublished" experiments in the second study. Our third study finds that generative architectures are able to produce reasonable "emergent" behavior - behavior that LLMs were not explicitly instructed to engage in - in simulation, a finding that has been supported in past research of simulations in other real-world contexts \cite{park2023generativeagentsinteractivesimulacra}. Altogether, this consistency begins to compellingly demonstrate the promise that multi-agent LLM architectures show in being able to simulate human behavior to an acceptable degree and to be used by policymakers as low consequence testing and thinking tools. 

% Past work has shown LLM simulations accurately capture directional effects in both published and unpublished results – but it doesn’t study PPG and doesn’t use an architecture that would allow for "unbounded behaviors" that are necessary for policymaking \cite{hewitt2024predicting}. Past research has shown that generative architectures result in emergent behavior in simulation but do not rigorously evaluate its consistency with observed human behavior \cite{park2023generativeagentsinteractivesimulacra}. Past research has shown that multi-agent architectures perform better than single LLMs in economic games, but do not address the PGG \cite{sreedhar2024simulatinghumanstrategicbehavior}.
% \color{black}

\section{Limitations and future work}
This paper represents an initial exploration of multi-agent LLM systems as a tool for simulating human behavior and has several limitations. While the findings demonstrate that the proposed approach is feasible, there remain many open questions and challenges that need to be addressed.

%Hyperfocus on prosocial cooperative behavior and PGG. 
This paper focused on prosocial cooperative behavior and used the public goods game (PGG) as a vehicle for many of the preliminary studies (Studies 1 and 2). Although the PGG closely mimics real-world scenarios like taxation and charitable donations, it has limitations. First, the outcomes of the PGG depend on its multiplication factor for increasing the public pot. Typically, a factor of 1.6 is used, but if the multiplication factor is lower, the potential benefit is reduced, which could alter the game's dynamics. We lack human data for all possible values of the multiplication factor for comparison. Additionally, there are many variants of the PGG that were not tested: for example, punishment is an important mechanism that was not explored, though it has been shown to replicate in other games like the Ultimatum Game. There are countless mechanisms to replicate, and the more games we replicate, the more confidence we can have that multi-agent LLM systems are consistent with human behavior. At this point, there is a growing body of evidence from AI, HCI, economics, and psychology suggesting that LLM-agents can capture much of human behavior; what remains is to identify and refine the mechanisms that enable successful simulation.
% This paper focused on prosocial cooperative behavior, and used the public goods game as a vehicle for many of the preliminary studies (Studies 1 and 2). Although the PGG closely mimics many important real world scenarios like taxation and charity donation, it is also limited. The first the outcomes of the PPG game depend on its multiplication factor to increase the public pot. Typically 1.6 is used, but if the multiplication factor is lower, then the potential benefit is lower, and that could change the overall dynamics of the game. We don’t have human data for all possible values of the multiplication factor to compare to. Additionally, there are many variants of the PPG that we did not test: punishment is an important mechanism we did not test, but it has been shown to replicate for other games like the Ultimatum Game. There are an unending number of mechanisms to try to replicate. The more games replicate, the more confidence we have that MA-LLMs are consistent with human behavior, the more confidence we can have in AI simulations. At this point, there is a growing body of evidence from AI, HCI, Economics and Psychology that largely conclude that AI can capture much of human behavior; what remains to be done is capture and simplify the mechanisms that allow for successful simulation.

%No guarantees of  generalizability? 
% Our second study, along with other studies replicating multiple experiments not yet published [willer], indicate that LLMS are not simply echoing results of previous papers. Thus, there is potential for LLMs to have simulate human behavior for novel scenarios. It’s unclear how LLMs have these abilities. Possibly LLMs are using knowledge of past experiments and are transferring principles learned from one paper onto new scenarios. An extreme hypothesis is that LLMs are not using any experimental knowledge and have truly understood human nature from training data. It’s unclear how they have these abilities, and it’s also unclear what the limits on it might be. For any novel scenario put in a simulation, we will never know whether the LLM is capable of simulating those abilities or not.  Other work has shown that not all studies replicate [willer], but future work will have to test the bounds on when LLMs are more or less likely to simulate behavior. 

Our second study, along with other studies replicating multiple unpublished psychology experiments ~\cite{hewitt2024predicting}, indicates that LLMs are not simply echoing the results of previous papers - there is potential for LLMs to simulate human behavior in novel scenarios. It is unclear how LLMs possess these abilities since they don't have inherent motivations like humans. Perhaps \color{black} they are using knowledge from past experiments and transferring principles learned from one context to new situations. An extreme hypothesis is that LLMs may not be relying on experimental knowledge at all but have genuinely understood aspects of human nature from their training data. However, the limits of these abilities are also uncertain. For any novel scenario in a simulation, we cannot be certain whether the LLM is capable of simulating the required behaviors. While previous work has shown that not all studies replicate, future research will need to test the boundaries of when LLMs are more or less likely to simulate human behavior accurately.

%complex effects like interactions
Our studies primarily tested single interventions, but real-world scenarios are more complex, often involving multiple policies that can interact in unpredictable ways. For example, adding transparency might increase donations in the PGG, while negative priming might decrease them. If both policies are present, the outcome could vary depending on the specifics of the situation, and there may not be a definitive ground truth to compare against. In the future, more psychological experiments may need to be conducted to inform simulation design.
% Our studies mostly tested a single intervention, but in the real-world more complex things can happen - multiple policies can be present and combine and have a complex interaction. For example, adding transparency should increase donation in the PGG, but negative priming should decrease it. If both policies are present, what will happen? Psychology does not have a clear answer for this - the outcome depends on the specifics of the situation, and there might not be ground truth to compare to. In the future, more psychology experiments might have to be run to inform simulation. 

%POPULATIONS
Much of the experimental evidence from the social sciences is based on Western, Educated, Industrialized, Rich, and Democratic (WEIRD) populations. If LLMs do replicate human behavior, it is uncertain whether they can replicate all human behaviors, or only those represented in training data, such as experiments and online content. Further research is needed to understand to what extent LLMs can simulate behaviors of diverse groups, including children, marginalized communities, and others who are underrepresented in the training data. Past research has demonstrated that people from different types of communities act differently in the same strategic scenarios \cite{oosterbeek2004cultural, henrich2000does, kozitsina2020ethnicity} - it is important to ensure that simulations are representative of the population for which policymakers using them are designing for. \color{black} Additionally, people often behave differently toward their in-group versus an out-group, and it is unclear whether LLMs can capture these nuances.
% Much of the experimental results from the social sciences are based on Western, Educated, Industrialized, Rich, and Democratic (WEIRD) populations. If LLMs do replicate human behavior, it is unclear whether they can replicate all human behavior, or just those seen in training data such as experiments and online content. Further research would require understanding to what degree LLMs replicate WEIRD populations, children, marginalized communities, and other groups that are not well represented in the training data. People also act different to their in-group (or tribe) than they do to an out-group (or competitors). It’s unclear if LLMs capture these nuances of human populations.

% LLMs evolve.
The foundational LLMs used in these simulations continue to evolve. Simulations that replicate human behavior today may not do so in the future. As LLMs are trained on new datasets, their behavior could change for better or worse; high-quality human behavior data (e.g., from video sources) could improve the model, while low-quality or synthetic data could lead to degradation (e.g., mode collapse). Reinforcement Learning from Human Feedback (RLHF) can also cause certain LLMs, such as GPT-4, to display hyper-rational behaviors that exceed typical human responses, especially in emotionally charged situations where humans would behave more irrationally. Experimental results show that LLMs may react to induced emotions (e.g., happiness or anger) in disproportionately rational ways~\cite{mozikov2024good}. Future work may need to track how well simulation results replicate on different models over time.

% The foundational LLMs these simkluations are built on continue to evolve. Simulations that replicate human behavior today might not replicate in the future. LLMs change in many ways: As LLMs train on new datasets agent behavior could change for the better or worse - more data of high quality human behavior data (perhaps from video data) could enhance the model, but low quality, or synthesized data might make it worse (or exhibit mode collapse). Reinforcement Learning from Human Feedback (RLHF) can cause certain LLMs (such as GPT-4) to display hyperrational behaviors that exceed those of humans. This hyperrationality becomes more pronounced in more emotionally charged situations where humans would behave more irrationally. Experimental results show that LLMs might react to induced emotions (such as happiness or anger) in ways that are disproportionately rational ~\cite{mozikov2024good}.

%Actual human cognition.
Lastly, there is a gap between how role-playing tasks are simulated and actual cognitive processes. Naive priming in role-playing situations often leads to caricature-like behaviors instead of genuine cognitive modeling. This is because the underlying RLHF mechanism relies on human crowd workers providing feedback on what ~\emph{they think seems like} plausible behavior for a particular character in a particular situation. However, stereotypical perceptions of behavior can often not match real human behavior in moral dilemmas. For instance, many people may think a Buddhist monk would react to the trolley problem by avoiding action, when in reality surveys have shown the opposite. Moreover, the humans in the loop tend to belong to similar populations characterized as “poorly paid gig workers” ~\cite{casper2023open}, biasing the kinds of perceptions that are represented. Addressing these limitations may involve leveraging techniques like Bayesian induction and internal dialogue to foster more sophisticated representation of agent behaviors.


% 

% \subsection{Mechanisms \& Limitations of LLM-Based Simulations}

% We can predict mismatches between simulation outcomes and human behavior by analyzing the mechanisms underneath the hood in LLM systems. One such mechanism is the bias in the population that produces the content of the training data. Since LLMs are largely trained on content from WEIRD (Western, Educated, Industrialized, Rich, and Democratic) populations, they tend to replicate behaviors typical of these groups ~\cite{atari2023humans}. This bias becomes evident when simulating economic games for which we have experimental evidence of cross-cultural differences in behavior. For instance, the Orma of Kenya have been shown to exhibit the near-total cooperation in public goods games ~\cite{henrich2000does}, which is not captured accurately by out-of-the-box LLMs.

% In terms of reinforcement learning mechanisms, anti-hallucination incentives in Reinforcement Learning from Human Feedback (RLHF) can cause certain LLMs (such as GPT-4) to display hyperrational behaviors that exceed those of humans. This hyperrationality becomes more pronounced in more emotionally charged situations where humans would behave more irrationally. Experimental results show that LLMs might react to induced emotions (such as happiness or anger) in ways that are disproportionately rational ~\cite{mozikov2024good}.

% Beyond hyperrationality, other behaviors and values are also enforced through RLHF to mitigate safety and liability concerns for LLM developers. Most of the popular LLMs (GPT, Gemini, Claude, Llama) are guided by a set of safety guidelines that enforce certain moral values, such as avoiding generating offensive or hurtful content. These guidelines are then given to human evaluators in the RLHF process to enforce. This moral bias deviates from varieties of human behavior that do not reflect morality or follow the same moral paradigm. In our experiments, we found that sometimes LLMs struggle to emulate "bad" behaviors, such as punishing, antagonizing, or reprimanding. For example, in punishment scenarios within the Public Goods Game, GPT-4 models rarely resort to punishment, even when interacting with selfish agents. Moreover, dialogue generated by LLMs in adversarial situations tends to remain polite and sycophantic, consistent with other literature observing sycophantic behavior ~\cite{sharma2023towards}.

% Lastly, there is a gap between how role-playing tasks are simulated and actual cognitive processes. Naive priming in role-playing situations often leads to caricature-like behaviors instead of genuine cognitive modeling. This is because the underlying RLHF mechanism relies on human crowd workers providing feedback on what ~\emph{they think seems like} plausible behavior for a particular character in a particular situation. However, stereotypical perceptions of behavior can often not match real human behavior in moral dilemmas. For instance, many people may think a Buddhist monk would react to the trolley problem by avoiding action, when in reality surveys have shown the opposite. Moreover, the humans in the loop tend to belong to similar populations characterized as “poorly paid gig workers” ~\cite{casper2023open}, biasing the kinds of perceptions that are represented. Addressing these limitations may involve leveraging techniques like Bayesian induction and internal dialogue to foster more sophisticated representation of agent behaviors.

% \subsection{LLMs as simulacra?}
% % Maybe include some discussion on the amplification of human behavioral trends that we notice in experiments. Would it be useful to think of LLMs as simulacra that exaggerate certain features of behavior?

% \subsection{Utility of Simulations Across Contexts}
% % Can we draw any conclusions about the relative utilty of simulations in different scenarios (eg when human behavior is more consistent but we don’t know how things play out at scale or over time, simulation is useful; when cross cultural differences make human behavior difficult to predict, simulation could be difficult to use)?

% \subsection{Additional Cooperation Mechanisms}
% Beyond the validated theories we tested here, experiments have investigated a wide range of factors influencing cooperation in similar games like commons dilemmas, including but not limited to individual differences such as social motives and gender, perceptual factors about the causes and uncertainty of the situation, and social structure of the participants in terms of group size and power differentials. These factors can be used to inform potential policy designs and further evaluate how closely simulations match human behavior across more granular factors.

% \subsection{Ethical Concerns for Policy Designers}
% % It's probably important to explicitly discuss the ethical risks of using simulations for informing policy design, and how we can mitigate those risks. For example, we can explicitly present methods for mitigating stereotype-based biases in agent behaviors.

% Using LLM simulations to inform policy design presents a host of potential ethical risks. For example, when simulations are used to inform policies that impact diverse populations, there is a danger that these biases could reinforce harmful stereotypes or perpetuate systemic inequities. Potential technical and human system mechanisms can be used to mitigate these risks.

% For example, bias detection mechanisms could be implemented to identify and flag stereotypical behaviors exhibited by simulated agents. The tricky part here is accounting for cross-cultural and cross-demographic variations in behavior while not falling into exaggerated stereotypes. While some mitigation can be done, ultimately the tool itself must be used with sensitivity to these biases and avoid over-reliance for design making.

% Transparency and explainability help make possible this kind of appropriate usage. It is important to embed into the tool itself a clear understanding of the limitations and potential biases inherent in the models. Decision-makers should be informed about the mechanisms used to reduce bias, and uncertainties in the models' predictions should be openly communicated. This enables policymakers to make more informed decisions and reduces the risk of over-reliance.

% Ultimately, there is an ethical responsibility to consider the potential societal impact of policies informed by LLM simulations. Policies that influence sensitive domains---such as criminal justice, healthcare, or economic redistribution---should be subject to thorough ethical reviews before being implemented. LLM-based simulations should complement rather than replace human judgment and expertise, especially in contexts where the stakes are high. It is crucial to involve diverse stakeholders in the policy design process to ensure that multiple perspectives are considered, and to validate the fairness and appropriateness of simulated outcomes. Finally, it is important to guard against the misuse of LLM-based simulations for manipulative purposes, such as using simulated human behavior to justify controversial policy decisions or to sway public opinion through synthetic social proof.

% \subsection{Limitations}

% % If we talk about mechanisms and limitations in the discussion, we don't need to go into depth here, we can just mention briefly. I'm not sure how we should split topics between discussion & limitations/future-work/conclusion. @lydia up to you.
% LLMs are good at simulating behavior of experiment participants, but it may turn out they are best at simulating WEIRD people. The experiments we replicate and the knowledge and studies we use to inform the real-world scenarios are likely drawn from WEIRD people, because of the convenience sampling performed in many published experimental studies. An extension of this work might examine the ability of LLMs to simulate behavior in a wider range of demographics. 

% \bigskip

% The system we use is limited by the underlying model (GPT4). There are many other models to chose from. Moreover, as LLMs change, the outputs will change.

% \color{black}



==> source/6_conclusion.tex <==
\section{Conclusion}

This study demonstrates the potential of multi-agent LLM systems to simulate cooperative prosocial behavior, particularly in the context of public goods games. Our findings show that these systems can not only replicate the directional effects observed in human public goods game experiments but also apply priming effects from non-public goods game experiments and incorporate the fading of priming effects over time, as observed in multi-round games. The ability of LLMs to transfer effects across different contexts suggests a deeper understanding of human behavior rather than mere recapitulation of specific experimental results. Our research also highlights the need for additional mechanisms, such as private communication channels and stake-prompting, to accurately capture the nuances of human behavior in real-world scenarios.

While these results are promising, they also underscore the importance of careful implementation and interpretation when using LLM simulations to inform policy decisions. The observed exaggeration of effect magnitudes and the potential for bias inherent in LLM training data necessitate a cautious approach. Future research might focus on refining these simulation techniques, addressing limitations, and developing robust frameworks for validating LLM-based behavioral predictions against real-world outcomes. In sum, these studies suggest that LLM-based simulations, when used judiciously and with an understanding of their limitations, can become a valuable tool for policy designers, offering insights into potential human reactions to policies whose effects may be both difficult to anticipate and crucial to understand.

